Efficient Full-Stack Private Federated Deep Learning with Post-Quantum Security

Federated learning (FL) enables collaborative model training while preserving user data privacy by keeping data local. Despite these advantages, FL remains vulnerable to privacy attacks on user updates and model parameters during training and deployment. Secure aggregation protocols have been proposed to protect user updates by encrypting them, but these methods often incur high computational costs and are not resistant to quantum computers. Additionally, differential privacy (DP) has been used to mitigate privacy leakages, but existing methods focus on secure aggregation or DP, neglecting their potential synergies. To address these gaps, we introduce Beskar, a novel framework that provides post-quantum secure aggregation, optimizes computational overhead for FL settings, and defines a comprehensive threat model that accounts for a wide spectrum of adversaries. We also integrate DP into different stages of FL training to enhance privacy protection in diverse scenarios. Our framework provides a detailed analysis of the trade-offs between security, performance, and model accuracy, representing the first thorough examination of secure aggregation protocols combined with various DP approaches for post-quantum secure FL. Beskar aims to address the pressing privacy and security issues FL while ensuring quantum-safety and robust performance.

==> sections/backup.tex <==










\section{Backup}
The model depends on a third party (i.e., aggregation server) to aggregate (average) the users' gradients in each round. Each user might run multiple epochs locally and report the final update in each round. 
The issue is the intermediate updates can leak information about the users' training data and defeat the data privacy benefit offered by federated learning (i.e., keeping local data private while training a centralized model). 

Existing solutions mainly rely on two approaches: multi-party computation (MPC) and homomorphic encryption (HE). MPC-based approaches often incur significant communication overhead, and HE-based methods require heavy computations.  

Most of the existing frameworks do not offer long-term post-quantum security. 


\section{Our Goal}

Our goal for the journal paper can be summarized in two main contributions: 
The MPC-based design of Bonawitz et al. \cite{bonawitz2017practical} is very communication intensive. Therefore we would want to opt-in for either the design in \cite{flamingo} or \cite{eseafl}. 

The cryptographic primitives used in \cite{eseafl} are efficient and easy to implement. However, the work is still under submission. 

The design in \cite{flamingo} relies on notions such as threshold decryption, which might give us more opportunity. Additionally, it is already published in S\&P Oakland. 

Regardless of which design we choose, we need digital signatures to provide security against malicious adversaries (one that can interfere with communication). We have identified that given in the federated learning setting, the users only communicated in limited training iterations; we can utilize a multiple-time signature scheme.


\subsection{Contribution I}
Design a post-quantum federated learning (PQFL) framework that achieves communication (ideally one round overhead) and computation efficiency. 


For an MPC-based approach, similar to \cite{bonawitz2017practical,Bell2020} we need the following: 

\begin{enumerate}
    \item We will use ASCON as our PRF 
    \item We need to have Kyber as a KEM since key agreement is not considered by NIST PQC
    \item We will use Dilithium with precomputation for signatures
    \item We can also consider that the assisting nodes might not be available, so we might use homomorphic PRF and shamir secret sharing to make up the key for the offline assisting nodes 
    % \item Secret sharing algorithm (e.g., \cite{shamirSecret})to allow $t$ users to reconstruct a share that is divided into $n$ shares, where $n>t$. 
    % \item Key agreement protocol to allow users to agree on a shared key. 
    % \item Authenticated encryption (e.g., ASCON-AE) to allow users to communicate while protecting the integrity and confidentiality of the message. 
\end{enumerate}

We also need a signature scheme \cite{dilithium} to achieve security against a malicious adversary. 

\subsection{Contribution II}

Engineering (multi-core and/or GPU) and optimization (pre-computations) contributions and running on different settings. 

Stress on the powerful server.
Multi-core is available on Apple and Android phones.

\yiwei{
\noindent
\textbf{Contribution.}
\begin{itemize}
\item \textbf{Focusing on stronger adversary models}. Considering the threats posed by quantum computing.
\item \textbf{Exploring the performance and security trade-off through the lens of differential privacy and secure aggregation}. 
For SA, post-quantum algorithms + precomputation
For DP, explore different threat models.
\end{itemize}
}

% \todo{Contribution:
% (1) stronger adversary models (most relax)
% (2) and investigate the performance and security trade-off through the lens of differential privacy and secure aggregation.
% (3) beyond straightforward combination of separate DP and SA and justify the favorable.
% }





\subsection{Adversary}
Consistent with \todo{Flamingo, MicroFedML, PrivateFL}, we consider three types of adversaries, i.e., external attackers, malicious clients, and malicious server.
For all the settings, the adversary is eager to pry on honest users' data.


we define the threat model for launching binary black-box AME attacks against static anti-malware models. Nevertheless, unlike the threat model proposed in (Anderson et al. 2018), which targets feature-based anti-malware engines, our threat model fo- cuses on launching attacks against DL-based anti-malware engines. Three major components of our threat model are:
• Adversary’s Goal: Automatically crafting mal- ware variants that are capable of evading DL-based anti- malware.
• Adversary’s Knowledge: The structure and pa- rameters of the anti-malware model are unknown to the adversary. Furthermore, the adversary does not have ac- cess to the confidence score produced by anti-malware. The only information available to the adversary is whether the generated malware variant can evade the anti-malware or not.
• Adversary’s Capability: Applying functional- ity preserving append modifications on malware binary, while the maximum modification size is limited. We fo- cus on append modifications, since they very often do not interfere with the functionality of the malware.




\yiwei{Compare threat models with Flamingo}

\yiwei{Semi-honest setting.}

Although client data is not directly exposed in the FL process, a large body of research has shown that it is still possible to reveal sensitive client data from individual updates or trained models via data reconstruction or membership inference attacks. 
For example, an adversary can accurately reconstruct a client’s training data from its gradient updates~\cite{geiping2020inverting, wang2022protect, yin2021see, zhao2023secure}; an adversary can also infer from a trained language model whether a client’s private text is in the training set~\cite{carlini2019secret, nasr2019comprehensive, shokri2017membership, song2019auditing}.
% https://dl.acm.org/doi/pdf/10.1145/3627703.3629559

% Three types of roles are involved 
Considering different FL scenarios, in this paper, we target three settings of adversaries, i.e., external attackers, untrusted clients, and untrusted server. For all settings, the adversary is eager to pry on honest users' data.
Specifically, \textit{external attackers} \yiwei{Cryptographic attackers} will be able to intercept the traffics and modify the transmitted packets to perform MITM attacks. 
% They can also act as legimate participants (or compromise the legimate participants) to involve the FL training procedure.
They can achieve the quantum-level computation to crack any cryptographic algorithms.
But \textit{external attackers} are not involved in the FL training procedures. So they can only perform attacks from external or after training.
\textit{Untrusted clients}, including malicious, compromised and impersonated users, can engage in various adversarial behaviors, including injecting false or manipulated data, 
% model poisoning by submitting corrupted updates to compromise the global model's performance, 
and privacy breaches by attempting to infer sensitive information from their local models or gradients. 
Such an assumption is feasible as sometimes the attackers will impersonate as normal users or leverage the existing vulnerabilities to compromise the legitimate users, so that they can involve in the FL procedure to perform further serious attacks like tampering or inferring the sensitive training data.
Additionally, we also consider the \textit{untrusted server} in which the server is \yiwei{honest-but-curious} and attempting to infer sensitive information from global models or client gradients. 



We assume a static, malicious adversary that corrupts the server and up to an $\alpha$ fraction of the total $N$ clients. That is, the adversary compromises $\alpha N$ clients independent of the protocol execution and the corrupted set stays the same throughout the entire execution (i.e., all rounds). Note that malicious clients can obviously choose to drop out during protocol execution, but to make our security definition and analysis clear, we consider the dropout of malicious clients separate from, and in addition to, the dropout of honest clients.

% \yiwei{What if the user is originally malicious? How to protect in such case?}

% can engage in various adversarial behaviors, including data poisoning by injecting false or manipulated data, model poisoning by submitting corrupted updates to compromise the global model's performance, and privacy breaches by attempting to infer sensitive information from their local models or gradients. 

% We aim to control the exposure of honest clients’ data against the above-mentioned attacks. Following the Secure Multi-Party Computation (SMPC) literature [26], we target both the semi-honest setting (where all parties faithfully fol- low the protocol) and the malicious setting (where the adversary can deviate arbitrarily from the protocol). In both settings, the adversary is eager to pry on honest clients’ data, and may collude with the server and a fraction of sampled clients to boost its advantages. We assume mild client collusion because, in real deployments, the number of clients is usually large, making it hard for an adversary to corrupt a large fraction of them. For example, at the scale of the Apple ecosystem (over 2 billion active devices [8]), even com- promising 1% would mean about 20 million nodes. Conse- quently, the chance of having many colluded clients sampled by the server is tiny, if it follows the agreed-upon sampling

\subsection{Threat Models and FL Setups}
Our departure point are FL protocols deployed in real-world applications, such as the one described in~\cite{bonawitz2019towards}. These protocols initially focused on data minimization only.
Based on multiple types of adversaries, we consider four combinations of adversaries in our work. In the following, we illustrate the four types of threat models and the corresponding FL setups to protect the sensitive data from leakage.
\todo{Why do we choose these four threat models? -- applications in real FL systems!}

\begin{itemize}
\item \textbf{TM1: No external attackers, trusted clients and trusted server.} 
We consider such a ``plain'' model as our baseline, where no adversaries are involved. 
In this case, an non-private FL setup can be applied without any secure aggregation and differential privacy protections.

\item \textbf{TM2: External attackers, trusted clients and trusted server.} 
If there are only \textit{external attackers} and they cannot compromise any FL participants, where the FL clients and server can be trusted, we will adopt secure aggregation (SA) and differential privacy (DP) techniques to protect the FL training procedure. Specifically, to prevent the external attackers from inferring the private user training data from the global model, the server can add the DP noise to the final model at the end of the training (i.e., the last round). Then the users can perform the MPC-based protocol to ensure the server can calculate the correct aggregation of all user updates without sending the plain individual updates to the server. This can avoid leaking user private data via the transmission. Moreover, we also adopt digital signatures to guarantee the identity of the participants and the integrity of the transmitted messages.

\item \textbf{TM3: External attackers, untrusted clients and trusted server.} 
Based on \textbf{TM2}, if the clients cannot be trusted, i.e., users are malicious or can be compromised, we will then keep the same SA and digital signature methods and slightly modify the DP procedure. Specifically, instead of adding the DP noise at the end of training, we should apply DP protection on each training round. That is, the server should add the DP noise to the global model after the training of each round. In this way, the untrusted clients will not be able to infer the private individual updates from the DP-protected global models.

\item \textbf{TM4: Exteranl attackers, (un)trusted clients and untrusted server.} 
Based on \textbf{TM3}, if the server cannot be trusted, in which the malicious server tries to infer individual users’ local sensitive data points, we will then apply the DP protection on each client side. That is, each user should add the DP noise to the local model training at each round to prevent the server from inferring sensitive user taining data.
\end{itemize}


% \subsection{FL Setup}
% Our departure point are FL protocols deployed in real-world applications, such as the one described in [9]. These protocols initially focused on data minimization only. We extend them with SA and DDP,
% % https://ieeexplore.ieee.org/abstract/document/10190489


% \subsection{Adversary}
% First adversary is the external attackers. They are able to intercept the traffics but do not involve in the federated learning. 
% quantum computer
% run attacks after the training
% \yiwei{So we need (1) client and node signature for integrity and authenticity; (2) different privacy at least on the last iteration.}

% Second adversary is the server, and their goal is to infer individual users’ local sensitive data points. 
% % Note that the background in Section 2.1 implies that the server can—whenever they choose to—(1) control the weights of the shared model, (2) select which of the N users participate in each round, and (3) provision new users into the pool.
% % (including sybils controlled by the server). We assume that the total fraction of sybils out of the N users is small.
% % https://ieeexplore.ieee.org/abstract/document/10190489

% % We, furthermore, assume the server is malicious, meaning they behave maliciously in any rounds of the protocol. When this happens, they can exert the above capabilities (1-3) adversarially. Do note that the server here does not deviate from the protocol and restricts themselves to only use valid operations (1-3) in the FL protocol. 
% % An OM server ensures the attack remains stealthy, and also allows the server to train a model that has high utility over the non-malicious rounds, which is an expected product of FL.
% \yiwei{So we need (1) differential privacy on each iteration on each iteration on client side.}


% Third adversary is the clients ... \yiwei{Malicious clients can engage in various adversarial behaviors, including data poisoning by injecting false or manipulated data, model poisoning by submitting corrupted updates to compromise the global model's performance, and privacy breaches by attempting to infer sensitive information from their local models or gradients. 
% So we need (1) client signature for authentication; (2) differential privacy on each iteration on server side.}

% We assume a static, malicious adversary that corrupts the server and up to an $\alpha$ fraction of the total $N$ clients. That is, the adversary compromises $\alpha N$ clients independent of the protocol execution and the corrupted set stays the same throughout the entire execution (i.e., all rounds). Note that malicious clients can obviously choose to drop out during protocol execution, but to make our security definition and analysis clear, we consider the dropout of malicious clients separate from, and in addition to, the dropout of honest clients.


% \subsection{Adversarial Model}

% \begin{itemize}
% \item \textbf{Trusted server and trusted client.}

% \item \textbf{Trusted server and untrusted client.}

% \item \textbf{Untrusted server and untrusted client.}

% \end{itemize}




\section{Models}
FL faces significant security threats. 
Consider an FL framework used to enhance the autofill functionality of a mobile keyboard application, as depicted in Figure~\ref{fig:keyboard}. 
In that scenario, users' devices generate typing data, which is used to train local machine learning models. These local models are periodically transmitted to a central server for aggregation into a global model, which is then redistributed to users. This process, however, is vulnerable to several security threats. Attackers could compromise the server or clients, gaining access to transmission channels and potentially injecting or modifying updates to poison the training process, perform membership inference attacks to infer sensitive user data, or manipulate clients to drop out, thereby disrupting the FL process.

In the following of this section, we illustrate the potential adversaries with different abilities, the corresponding threat models, our system model, as well as the security argument.


% \subsection{Motivation Case}
% We first give a motivation example to illustrate the adversary's ability and the potential threats we should consider.
% Figure~\ref{fig:keyboard} depicts an FL framework implemented to enhance the autofill functionality of a mobile keyboard application. 
% In this scenario, multiple users interact with the keyboard application on their respective mobile devices, generating typing data comprising keystrokes, corrections, and frequently used phrases. 
% % To illustrate potential threats in federated learning (FL), we first give a scenario involving a mobile keyboard application aiming to enhance autofill functionality, as depicted in Figure~\ref{fig:keyboard}. 
% % Users interact with the application, generating typing data including keystrokes, corrections, and frequently used phrases. 
% Each user's device maintains a local machine learning model based on their individual typing patterns and vocabulary.
% Periodically, these local models are transmitted to a central server, which orchestrates the FL process. 
% The central server aggregates updates from users' devices to train a global model for autofill prediction. 
% Then it returns the aggregated global model to each user for autofill prediction and further local training.


% Such an FL process faces significant security threats. Attackers could compromise either the server or clients, gaining access to transmission channels, specially if the attacker is internal and has access to and control over these systems.
% As a result, attackers could threaten the transmission for uploading the local updates. For instance, they may deliberately inject or modify these updates to poison the training process, thereby undermining the performance of the overall model.
% % attackers could inject or modify updates to poison the training process, compromising model performance. 
% Moreover, they could also perform membership inference attacks, leveraging access to intermediate or final models to infer sensitive user keyboard input data. Additionally, attackers might manipulate clients to drop out during protocol execution, disrupting the FL process.



% \todo{Add dropout attacks in cryptographic}
% This threat model is relevant to many federated learning applications, such as medical systems, financial fields, and mobile phones, where the curious server or users aims to retrieve user private data.


% \todo{Financial system}
% https://arxiv.org/pdf/1811.03604

\begin{figure}
  \centering
  \includegraphics[width=1\linewidth]{figures/keyboard.pdf}
  \caption{A motivation example of mobile keyboard application.}
  \label{fig:keyboard}
\end{figure}


% In this paper, we consider a more relaxed threat model, involving three types of adversaries, i.e., external cryptographic attackers, honest-but-curious server and users.
% External cryptographic attackers are capable of performing MITM attacks with quantum-computing power to tamper the user updates or infer the local training data via the aggregated global models.
% Honest-but-curious server and users indicate the participants that passively exploit each client’s local models (i.e., honest-but-curious server) or the global models from the server (i.e., honest-but-curious clients) to infer the private user training data.
% Such a threat model can occur in many federated learning applications, like medical system, financial field and mobile phones in our daily life.
% For example, imagine a federated learning framework deployed for improving a mobile keyboard application's autocorrect feature. Users' typing data, including keystrokes and corrections made, are utilized to train a global machine learning model collaboratively. 
% In this case, there may be an external cryptographic attacker intercepts communication between users and the central server.
% By conducting Man-in-the-Middle (MITM) attacks, they can tamper with user updates during transmission, injecting malicious keystrokes or altering training data to degrade model performance. Furthermore, they could infer sensitive user inputs by analyzing the aggregated global models, compromising user privacy.
% A honest-but-curious server or users can also exist. Despite not actively tampering with or compromising the data, they might exploit the information contained within each client's local model or the global model to gain insights into user typing behavior or commonly used phrases.
% Unfortunately to the best of our knowledge, there is no relevant works considering such a threat model and giving corresponding solutions.
% Although some works also mention a malicious setting in which the server and clients can actively inject compromised data to perform data poisoning attack. We are not focusing on this setting as there are already existing studies working on it.

\subsection{Aderveries and Threat Models} 

% \reza{
% \sys incorporates a holistic view of three types of adversary: (1) Malicious client, Malicious server, and Model Inversion (MI) adversary.\\
% \textbf{Malicious Client.} This adversary represents an untrusted malicious entity that impersonates as a trusted client.\\
% \textbf{Malicious Server.} This adversary represents an untrusted  malicious entity that impersonates as the aggregation server.\\
% \textbf{Model Inversion (MI) Adversary.}
% Model inversion adversaries are characterized by machine learning (ML)-enabled attackers that aim to infer any information about or reconstruct the model's training data. In a broad sense, this type of adversary represents both black- and white-box attacks, including gradient-based and attribute/membership inference attacks. This type of adversary can attack both intermediary models during training and the final trained model. }


\begin{figure*}[!ht]
  \centering
  \includegraphics[width=1\linewidth]{figures/threat_model.pdf}
  \caption{Threat Models.}
  \label{fig:threat}
\end{figure*}

% \yiwei{PQ-FL: \\
% - Digital Signature: to defend cryptographic attacker (actively MITM, tamper data)\\
% - SA: to defend 1) malicious server (MI, local updates) and 2) MI attackers (passively MITM)\\
% - ODP: to defend MI attacker (not server or clients, final model)\\
% - CDP: to defend malicious clients (MI, intermediate model)\\
% - LDP: to defend malicious server (MI,  local updates)

% Adversaries:\\
% - Cryptographic attacker: can actively perform MITM to tamper data (local update or intermediate model). We need the digital signature.\\
% - MI attacker: can only access the final model after deployment or monitor the transmission. In this case, we need SA + ODP\\
% - MI clients: can access the intermediate model. We need CDP.\\
% - MI server: can access the clients’ local updates, and intermediate model. Both the local updates and the aggregated model can infer user training data. We need SA + LDP. LDP only is not enough - inference via local updates. SA is not enough - inference via aggregated intermediate model.}


\subsubsection{Adversaries}
% In our threat model, we first consider the quantum adversary, that is, the adversary can crack classical cryptographic algorithms by harnessing the laws of quantum mechanics or leveraging quantum computers to solve problems too complex for classical computers.
% Based on it, we further consider 
\sys incorporates a holistic view of three types of adversary, i.e., \textbf{A1}, \textbf{A2}, \textbf{A3}. Each of them has different abilities to achieve different goals.
\begin{itemize}
\item 


\item \textbf{A1: Final Model Adversary.} We consider an adversary targeting at the final models obtained by FL aggregation to conduct model invention to infer any information about the private training data on clients.
Such adversaries will be able to access the final models, which are usually publicly available.
But they cannot access the internal transmissions or involve in the aggregation procedure to affect FL training.
\item \textbf{A2: Intermediate Model Adversary.} We also consider an adversary targeting at the intermediate models aggregated by the server at the end of each iteration of FL aggregation. 
Such an adversary will be able to compromise or impersonate as a honest client, aiming at perform model inversion via intermediate models to infer any information about private training data of other clients.
\item \textbf{A3: Local Update Adversary.} We consider an adversary aiming at the local updates sent by the clients every iteration, either inferring private training data from client local updates or tampering the local updates to reduce FL model performance.
Such adversaries will be able to access the traffics between clients and the server to intercept and tamper the data transmissions via MITM, such as passively eavesdrop client updates or actively injecting malicious packets to reduce FL model training performance.
, or perform model inversion, such as inferring any information about or reconstructing the user private training data.
Moreover, quantum computation ability will be also considered, that is, the adversary can crack classical cryptographic algorithms by harnessing the laws of quantum mechanics to solve problems too complex for classical computers.
\end{itemize}



\newpage


\rouzbeh{In our threat model, we consider a quantum adversary, i.e., and adversary who has unlimited access to a }
\sys incorporates a holistic view of three types of adversary:

\reza{We should merge the following with adversaries capabilities, goals and knowledge}
\begin{itemize}
\item \textbf{Malicious Client.} This adversary represents an untrusted malicious entity that impersonates as a trusted client.
\item \textbf{Malicious Server.} This adversary represents an untrusted  malicious entity that impersonates as the aggregation server.
\item \textbf{Model Inversion (MI) Adversary.}
Model inversion adversaries are characterized by machine learning (ML)-enabled attackers that aim to infer any information about or reconstruct the model's training data. In a broad sense, this type of adversary represents both black- and white-box attacks, including gradient-based and attribute/membership inference attacks. This type of adversary can attack both intermediary models during training and the final trained model.
\end{itemize}

\subsubsection{Threat Models}
Consistent with existing studies~\cite{flamingo, microfedml, yang2023privatefl}, we consider four settings of threat models, involving the three types adversaries metioned before.

% \todo{external: attacks after deployment}

\yiwei{
A1 - upgrade to - A2 - upgrade to - A3 - upgrade to - A4
who can compromise, then can do what goal}


\vspace{5pt}
\noindent
\elisa{I am not sure why we need TM1. It does not seem to me that we use it in the performance and accuracy performance.}
\textbf{TM1: No external attackers, trusted clients and trusted server.}
We consider such a ``plain'' model as our baseline, where no adversaries are involved. 
That is, the adversary cannot perform MITM via insecure channels and both the server and clients honestly follow the FL aggregation protocol and do not perform inference attacks. 
% In this case, an non-private FL setup can be applied without any secure aggregation and differential privacy protections.

\vspace{5pt}
\noindent
% \textbf{TM2: MI attackers, trusted clients and trusted server.}
\textbf{TM2: MI attackers}
% \todo{data reconstruction}
\elisa{could we use the term "honest" instead of "trusted"? Is there a reason why you used "trusted"?}
The federated learning process can be threatened by external attackers which intercept and tamper with data transmissions between clients and the central server. The trusted clients and server ensure the 
\elisa{how do we ensure the integrity of the updates when being generated/applied by the clients and the server? by using signatures we ensure that the transmitted updates are not tampered with, but we cannot ensure that they are applied correctly once delivered to the server.}
integrity of local updates and the global model.
% We define such a threat model (\textbf{TM2}) as follows:
\begin{itemize}
\item Adversary’s Goal: To intercept and tamper with data transmissions between clients and the server.
\item Adversary’s Knowledge: External attackers can intercept traffic but have no involvement in the federated learning training procedures.
\item Adversary's Ability: Capable of performing MITM attacks and cracking cryptographic algorithms using quantum-level computation. 
% \item FL Setup: To counteract these threats, secure aggregation (SA) and differential privacy (DP) techniques are employed. The server adds DP noise to the final model at the end of training, and a multiparty computation (MPC)-based protocol ensures correct aggregation without plain individual updates being sent to the server. Digital signatures are used to verify participant identity and message integrity.
\end{itemize}

\vspace{5pt}
\noindent
% \textbf{TM3: External attackers, \yiwei{Model MIA} untrusted clients and trusted server.}
\textbf{TM3: Malicious clients.}
% \todo{intermediate model}
% \todo{access model parameters}
Beyond the external attackers, there are also untrusted clients 
\elisa{do you mean that a client can inject false data pretending to be another client? If you mean this, you need to be specific. Digital signatures can protect against this.
However, if you mean that  a client just creates its own false data and then signs and encrypts them and sends them to the server, I'm not sure we can we protect against this.}
who may inject false data or attempt to infer sensitive information. The server remains trusted, ensuring the aggregation of updates and the distribution of the global model.
\begin{itemize}
\item Adversary's Goal: Similar to TM2, with the additional aim of malicious or compromised clients inferring sensitive information.

\item Adversary's Knowledge: External attackers can intercept traffic, and untrusted clients have access to their local models and gradients.

\item Adversary's Ability: In addition to the abilities described in TM2, untrusted clients can inject false or manipulated data and attempt to infer sensitive information from global models. 

% \item FL Setup: To mitigate these risks, SA and digital signatures are maintained, and DP noise is applied at each training round to protect individual updates from being inferred by malicious clients.
\end{itemize}

\vspace{5pt}
\noindent
% \textbf{TM4: External attackers, (un)trusted clients and untrusted server.}
\textbf{TM4: Malicious server.}
In the worst case, the federated learning process faces threats from external attackers, potentially malicious clients, and an untrusted server. The server might attempt to infer sensitive information from client data despite its role in aggregating and distributing the global model.
\begin{itemize}
\item Adversary's Goal: To intercept and tamper with data transmissions, and for the untrusted server to infer sensitive information from client data.

\item Adversary's Knowledge: External attackers can intercept traffic, and untrusted server has access to the global model and client gradients.

\item Adversary's Ability: Beyond the capabilities in TM3, the untrusted server may attempt to infer individual users’ local sensitive data points. 

% \item FL Setup: In this model, each user adds DP noise to their local model training at each round to prevent the server from inferring sensitive user training data. This ensures robust protection against both external attackers and an untrusted server.
\end{itemize}

\vspace{5pt}
\elisa{Is the paragraph below related to specific attacker models among the ones listed above?}
We assume a static, malicious adversary that corrupts the server and up to an $\alpha$ fraction of the total $N$ clients. That is, the adversary compromises $\alpha N$ clients independent of the protocol execution and the corrupted set stays the same throughout the entire execution (i.e., all rounds). Note that malicious clients can obviously choose to drop out during protocol execution, but to make our security definition and analysis clear, we consider the dropout of malicious clients separate from, and in addition to, the dropout of honest clients.

\todo{We do not consider poisoning attacks as existing works have solved it.}


\subsection{System Model}


\begin{figure}
  \centering
  \includegraphics[width=1\linewidth]{figures/system_model.pdf}
  \caption{System Model of \sys.}
  \label{fig:sys_model}
\end{figure}

Figure~\ref{fig:sys_model} illustrate the system model. inspired by~\cite{behnia2023efficient}, our system consists of three types of participants: a server, clients, and assisting nodes.
At a high level, \sys introduces a one time setup and an aggregation step for computing multiple sums, such that the secrets established in the setup can be reused throughout the aggregation step. For each summation in the aggregation step, clients mask their local updates with a random mask derived from those secrets, and then send the masked updates to the server. The server sums up all the masked updates and obtains the aggregated intermediate model (what the server wants) masked with the sum of all masks. \sys then uses a lightweight protocol whereby a small number of additional participants (which we call assisting nodes) interact with the server to remove the masks.
To addresses \sys employs DP techniques to add noise to updates, preventing inference attacks during global model aggregation or local model training or at testing time, after the model is released to be used.







\subsection{Security Model}

\rouzbeh{EU-CMA
PQ
DP definitions }
\rouzbeh{describe the SIS problem }

which we will feed to our hybrid security argument 




\section{Post-Quantum Federated Learning}
Given a secure public key infrastructure, \sys~only requires a single setup round to train a central model (via multiple rounds). 
%
\sys~provides security against quantum adversaries while incurring the least computational overhead compared to its counterparts with conventional (non-quantum) security. 
%
Below, we present the high-level ideas of \sys,  followed by a detailed protocol.  


\begin{figure*}[!ht]
  \centering
  \includegraphics[width=1\linewidth]{figures/pqfl_workflow.pdf}
  \caption{An overview of \sys system architecture and how it fits in the existing FL workflow.}
  \label{fig:workflow}
\end{figure*}


\reza {DP operations can be similar to Algorithm 1 (accountant, clipping, adding noise(Gaussian sampling (offline) + addition(online on the server))) https://dl.acm.org/doi/pdf/10.1145/2976749.2978318}

\subsection{High-level Idea}
The design of \sys~is based on two main observations: (1) Aside from the local training, the main overhead of privacy-preserving FL protocols is due to the underlying cryptographic operation. This is even worse if one considers post-quantum security. (2) the training takes place via a small number of iterations (e.g., 100-200 iterations). 
%
With these insights, we develop a set of precomputation methods aimed at significantly mitigating the cryptographic overhead while attaining post-quantum security. 
%
These methods are mostly targeted for public key operations (e.g., digital signatures) to mitigate their linear impact on protocol performance.
%
Following the recent development in practical secure aggregation protocols (e.g., \cite{flamingo,behnia2023efficient}), \sys~extends the trust on users to a cohort of (potentially rotating) assisting nodes.
%
The 




\subsection{\rouzbeh{Privacy During Training:} Secure Aggregation and Differential privacy}


\subsubsection{Setup Phase}
The setup phase is a one-time process that can be performed, at least partially, offline. 
This phase consists of a single round, namely, \textit{KeyGen and Advertise}. 
During this round, all users ${P_1, ..., P_n}$ and assisting nodes ${A_1, ..., A_k}$ are initialized with the two pairs of public keys, i.e., ($sk_{\kem}$, $pk_{\kem}$) for the key exchange scheme and ($sk_{\Pi}$, $pk_{\Pi}$) for the digital signature scheme. 
Then a public-key exchange procedure is performed in the following ways: 
1) the users receive copies of the key exchanging public keys from each assisting node $pk_{\kem}^{A_j}$;
2) the assisting nodes receive copies of the user signing public keys $pk_{\Pi}^{P_i}$;
and 3) the aggregation server receives copies of the signing public keys from assisting nodes $pk_{\Pi}^{A_j}$ and users $pk_{\Pi}^{P_i}$. 
After that each user can compute a shared secret $x_{P_i}^{A_j}$ for each assisting node $A_j$ with $sk_{\kem}^{P_i}$ and $pk_{\kem}^{A_j}$ via the key exchange scheme $\kem.Encaps(.)$ and securely send it to the corresponding assisting node $A_j$.
The assisting node $A_j$ can recover the shared secret using its private key $sk_{\kem}^{A_j}$ via $\kem.Decaps(.)$.
% Furthermore, all parties ${P_1, ..., P_n}$ and assisting nodes ${A_1, ..., A_k}$ have computed a shared secret $x$.

% At the end of \textit{KeyGen and Advertise} round in the setup phase, all the users ${P_1, ..., P_n}$ will have the signing key pair of itself ($sk_{\Pi}^{P_i}$, $pk_{\Pi}^{P_i}$) and the signing public key of each assisting node $pk_{\Pi}^{A_j}$. The ass

% During the \textit{KeyGen and Advertise} round in Algorithm 1, each assisting node first generates two key pairs, ($sk_{\sum}^{P_i}$, $pk_{\sum}^{P_i}$) by a key exchange scheme and ($sk_{\Pi}^{P_i}$, $pk_{\Pi}^{P_i}$) by a digital signature scheme, and then send ($pk_{\sum}^{P_i}$, $pk_{\Pi}^{P_i}$) to the users and send $pk_{\Pi}^{P_i}$ to the server. computes a shared secret $x_{P_i}^{A_j}$ with the assisting nodes $A_j$. In the malicious setting, users and assisting nodes are also initialized with signature key pairs to sign outgoing communications in the Aggregation phase (Algorithm 2).

% The setup phase is a one-time process that could potentially be carried out (at least in part) offline. This phase takes place in one round only, namely, \textit{KeyGen and Advertise}.
% At the end of this phase, all the parties $\{P_1, ..., P_n\}$ and assisting nodes $\{A_1, ..., A_k\}$ are initialized with the key exchange scheme (plus a digital signature scheme in the malicious setting) public keys. The assisting nodes and the aggregation server receive a copy of the user public keys. Additionally, all parties $\{P_1, ..., P_n\}$ and assisting nodes $\{A_1, ..., A_k\}$ have a computed a shared secret $x$.

% In the KeyGen and Advertise round in Algorithm 1, for the semi-honest setting, each user generates a key pair ($sk_{\sum}^{P_i}$, $pk_{\sum}^{P_i}$) for the key exchange protocol to computes a shared secret $x_{P_i}^{A_j}$ with assisting nodes $A_j$. 
% For the malicious setting, users and assisting nodes are also initialized with signature key pairs. This will be used to sign outgoing communications in the Aggregation phase (Algorithm 2). 


% Efficient Secure Aggregation for Privacy-Preserving Federated Machine Learning
% reference from Flamingo

\input{algos/sa_algo}

\subsubsection{Aggregation Phase}
The aggregation phase (Algorithm 2) comprises two rounds: \textit{Masking Updates} and \textit{Aggregate Updates}.

In the first round (\textit{Masking Updates}), each user computes a masking vector $a_t^{P_i}$ using the shared secrets $x_{P_i}^{A_j}$ for $j = {1, ..., k}$ to mask its local gradient vector $w_t^{P_i}$. The user then sends the masked gradient $y_t^{P_i}$ and a participation message (e.g., the iteration number) to the aggregation server and the $k$ assisting nodes, respectively. All the messages are signed using $\Pi.\sgnsign(.)$.

In the second round (\textit{Aggregate Updates}), upon receiving (and verifying) the participation message (and signature), each $A_j$ adds the user to the list $\mathcal{L}{j,t}$. For all users in $\mathcal{L}{j,t}$, $A_j$ computes the aggregation of their masking vectors $a_t^{A_j}$ using the shared keys $x_{P_i}^{A_j}$ and sends $a_t^{A_j}$ to the aggregation server, in which the messages are signed by assisting nodes using $\Pi.\sgnsign(.)$.
Next, when receiving (and verifying) the participation message (and signature), the aggregation server $\mathcal{S}$ adds the user to the list $\mathcal{L}{s,t}$ and then verifies that all user lists from the assisting nodes and the aggregation server are identical. 
For all users in $\mathcal{L}{s,t}$, the server uses the masked updates ($y_t^{P_i}$ and the aggregated masking terms $a_t^{A_j}$) provided by the assisting nodes to efficiently compute the final global model.

% The aggregation phase consists of two rounds: \textit{Masking Updates} and \textit{Aggregate Updates}.

% The first round of the aggregation phase (Algorithm 2) starts by the user computing a masking vector $a_t^{P_i}$ (using the shared secrets $x_{P_i}^{A_j}$ for $j = \{1, ..., k\}$) to mask its local gradient vector $w_t^{P_i}$. 
% Next, the masked gradient $y_t^{P_i}$ and a participation message (e.g., the iteration number) are sent to the aggregation server and the $k$ assisting nodes, respectively. 
% In the malicious setting, the outgoing messages are signed using $\Pi.\sgnsign(.)$.

% In the second round of the aggregation phase (Algorithm 2), for the semi-honest (malicious setting), upon receiving (and verifying) the participating message (and signature), each $A_j$ adds the user to the list $\mathcal{L}_{j,t}$.
% Then for all users in $\mathcal{L}_{j,t}$, it computes the aggregation of all their masking terms $a_t^{A_j}$ (using the shared keys $x_{P_i}^{A_j}$) and sends $a_t^{A_j}$ to the aggregation server. 
% In the malicious setting, the assisting nodes sign all their outgoing messages using $\Pi.\sgnsign(.)$.
% Next, for the semi-honest (malicious) setting, upon receiving (and verifying) the participating message (and signature), $\mathcal{S}$ adds the user to the list $\mathcal{L}_{s,t}$. Then it checks if all the user lists (assisting node's and the aggregation server's) are equal.
% Then, for all the users in $\mathcal{L}_{s,t}$, the server uses the masked updates (i.e., $y_t^{P_i}$ and the aggregated masking terms $a_t^{A_j}$), supplied by the assisting nodes, to efficiently compute the final model.

\subsubsection{Training Phase}
As mentioned before, sensitive data can be exposed through message exchanges in different iterations during FL training~\cite{}. 
% It is also possible to infer a client’s data from the trained models~\cite{} by exploiting their ability to memorize information~\cite{}. 
That is, if the users (i.e., \textbf{TM3}) or the aggregation server (i.e., \textbf{TM4}) are malicious, they can infer the private training data from the intermediate updates or global models.
Thus, it is not enough for secure aggregation to protect user training data from leakage.

To tackle that issue, \sys adds noises to the intermediate results by applying differential privacy techniques during the training.
Specifically, we consider two cases to protect the privacy during training:
\begin{itemize}
\item \textbf{Central Differential Privacy (CDP).} 
% If untrusted clients exist, \sys requires the aggregation server to add DP noise to the global models at each training iteration to protect individual data from being inferred by malicious clients via the aggregated updates.
For the \textbf{TM3} where the server can be trusted but the clients may be malicious, \sys adopts the Central Differential Privacy (CDP) setting to defend untrusted clients. In this case, \sys requires the aggregation server to add DP noise to the global models at each training iteration to protect individual data from being inferred by malicious clients via the aggregated updates.

\item \textbf{Local Differential Privacy (LDP).} 
For the \textbf{TM4} where both the server and the clients can be malicious, Local Differential Privacy (LDP) will be applied. 
\sys forces each LDP client to add the DP noise when training its local model at each iteration.
In this way, the intermediate local updates as well as the aggregated global models are defendable against both untrusted server and untrusted clients.
Note that the clients may use different privacy budgets $\varepsilon$, and the overall privacy guarantee depends on the largest $\varepsilon$ among all the clients.
 
\end{itemize}

% Dordis-Efficient Federated Learning with Dropout-Resilient Differential Privacy.pdf


\subsection{\rouzbeh{Post Training Privacy:} Differential Privacy}
After finishing the training procedure, the final global model may be accessible to everyone, including the malicious external attackers (i.e. \textbf{TM2}).
It is possible for these external attackers to infer a client’s data from the trained models~\cite{}.
To avoid inference attacks and the leakage of private training data in this case, \sys protects the post-training privacy by introducing the \textbf{One-time Differential Privacy (ODP)} strategy.
Specifically, the ODP server will add the noise to the final global model, i.e., add the noise at the last iteration of the training procedure.
In this way, \sys can achieve DP protections for the global model from external attackers. But ODP cannot defend the internal malicious parties like the untrusted server and clients. 

% \yiwei{In this paper, we tend to explore the best practice to integrate the secure aggregation and differential privacy under various threat models with different security requirements.}
% % Inspired by~\cite{yang2023privatefl}, w
% In the following, we introduce four DP settings, corresponding to the four threat models illustrated in Section xx:
% \begin{itemize}
% \item \textbf{Non Differential Privacy (NDP)}: For the \textbf{TM1} where no malicious adversaries are involved, we adopt the setting without differential privacy (NDP) as the baseline.
% \item \textbf{One-time Differential Privacy (ODP)}: For the \textbf{TM2} where only external attackers are considered and both the server and the clients can be trusted, we adopt the One-time Differential Privacy (ODP). The ODP server will add the noise after the end training step to achieve DP protections for the global model from external attackers. But ODP cannot defend the internal malicious parties like the server and clients. 
% \item \textbf{Central Differential Privacy (CDP)}: For the \textbf{TM3} where the server can be trusted but the clients may be malicious, we adopt the Central Differential Privacy (CDP) setting to defend untrusted clients. In this case, the CDP server adds calibrated noise during aggregation to achieve DP for the global model. Specially, CDP cannot protect data from untrusted server as the server can access the clients' noise-free local models.
% \item \textbf{Local Differential Privacy (LDP)}: For the \textbf{TM4} where both the server and the clients can be malicious, Local Differential Privacy (LDP) will be applied. LDP is the strongest variant, which defends against both untrusted server and untrusted clients. Each LDP client adds noise in each training step when training its local model in each FL round. Note that the clients may use different privacy budgets $\varepsilon$, and the overall privacy guarantee depends on the largest $\varepsilon$ among all the clients.
% \end{itemize}

% https://www.usenix.org/system/files/usenixsecurity23-yang-yuchen.pdf

\subsection{Efficient Post-Quantum Signature}

% dilithium has a type in the verify, we should not repeat it
% if conditions met, return 1 otherwise 0

% also, can you please make each algorithm interface like ours
% like (pk,sk)<-Gen(1^\kappa)

\input{algos/dili_algo}
\input{algos/precompute_algo}

Digital signatures are essential for ensuring the authenticity and integrity of transmitted messages. While post-quantum signatures promise long-term security against quantum adversaries, they are often more resource-intensive than their classical counterparts. This overhead becomes significant when these schemes are deployed on resource and battery-constrained devices like cellular phones. 
Following NIST post-quantum standards, we select and modify the Dilithium signature scheme \cite{dilithium} for use in \sys. In the following, we describe Dilithium and introduce a precomputation method to improve its computational overhead in the FL settings significantly. 

Dilithium is based on Fiat-Shamir with abort paradigm, and its security relies on the hardness of the modulo-SIS and modulo-LWE problems. We present the plain Dilithium signature (without any optimization) in Algorithm \ref{alg:dilithium}.   The key generation involves selecting matrix $\textbf{A}$ of dismission $k\times l$ and computing an MLWE public key $\textbf{t}=\textbf{A}s_1+s_2$ where $s_1$ and $s_2$ are sampled from the key space  $\mathcal{S}_\eta$ with small coefficient of size at most $\eta$. The $\mathsf{HighBits}(\cdot)$ and 
$\mathsf{LowBits}(\cdot)$ methods simply select the high-order and low-order bits of the coefficients in their vector, respectively. 

%
Given the Fiat-Shamir paradigm, in lattice-base settings, since we are solving for a variant of the SIS problem, the signature $\mathbf{z}$ should be small. To ensure this, an eligible signature should meet two conditions: (i) For security, it is crucial that the masking term $\mathbf{y}$ is completely hiding $c\mathbf{s}_1$,  the first rejection condition (Step 7) addresses this concerns. (ii) The second rejection condition is required for both the scheme's correctness and security \cite{behnia2021removing} and ensures that the same $c$ is recovered in the verification algorithm. 
In practice, this could require repeating the signing algorithm $~7$ times before finding an eligible signature \cite{dilithium,behnia2021removing}. This can have significant resource and computation overhead for constrained devices.  
 

To address this, by levering the fact that FL takes place in a small number of training iterations (in order of hundreds), we propose a precomputation algorithm for Dilithium. The high-level idea of the precomputation algorithm, presented in Algorithm \ref{algo:dili}, is to store a list of masking values $\mathbf{y}$ and their corresponding commitment values $\mathbf{Ay}$. Therefore, if during the signing algorithm if the selected masking term does not pass the rejection conditions, another value and its corresponding commitment can be selected from the list. Following the one-time nature of the masking term, once an eligible masking term is selected, it will be removed from the list. Algorithm \ref{alg:dilithiumfull} presents the incorporation of the precomputation algorithm in Dilithium signing algorithm. 
 
% To mitigate this overhead, we utilize the fact that federated learning often takes place in a small number of iterations (in order of hundreds) and revise a NIST post-quantum signature scheme \cite{dilithium}, to improve its signing overhead significantly. 

% However, the computation of these signatures, especially with post-quantum algorithms like \texttt{Dilithium}, can be resource-intensive and time-consuming. 
% Moreover, the pseudo-random number generation operation used for mask generation in every iteration is also time-consuming.

\subsection{Precomputation}
Digital signatures are essential for ensuring the authenticity and integrity of transmitted messages. However, the computation of these signatures, especially with post-quantum algorithms like \texttt{Dilithium}, can be resource-intensive and time-consuming. 
Moreover, the pseudo-random number generation operation used for mask generation in every iteration is also time-consuming.
To mitigate this, we get insights from~\cite{} to conduct an additional precomputation step, including precomputing post-quantum signing parameters and precomputing masks at the following iterations.

\subsubsection{Dilithium Signing Parameters}
Specifically, we identify several parameters within the \texttt{Dilithium} algorithm that can be precomputed offline.
The precomputed parameters must meet two criteria:
\begin{itemize}
\item They should be dependent on the specific message.
\item They should be dependent on the private key.
\end{itemize}

Based on these criteria, we precompute five parameters involved in the \texttt{Dilithium} signing algorithm, that is, a masking vector $y$ to introduce randomness and security properties into the signature generation, as well as the parameters derived from $y$. 
These parameters, not derived from the input messages or private keys that may change at runtime, can be calculated in advance. 
Consequently, our system (\sys) can perform these computations offline, prior to the runtime aggregation phase, and directly use the precomputed values during runtime signing. This approach significantly reduces the computational cost associated with generating digital signatures.

% As every transmitted message needs a digital signature to guarantee the sender's authenticity and the message's integrity, the calculation of signature can cause significant cost, especially for post-quantum algorithm (i.e., \texttt{Dilithium}). 
% Thus, to speed up the signing computation, we first select several parameters in \texttt{Dilithium} that can be computed offline. 
% Typically, the precomputed parameters should satisfy two requirements:
% 1) the parameters should message dependent; 
% 2) the parameters should private key dependent.
% As a result, \todo{xxx} parameters involving in \texttt{Dilithium} signing algorithm are select to be precomputed.
% These precomputed parameters are generated from the input messages or private keys which may change runtime.
% In this way, \sys can then compute them offline, i.e., before the runtime aggregation phase, and directly use them for runtime signing, which will greatly save the computation cost.



\subsubsection{Masks of Each Iteration}
To avoid local updates being leaked to external MIA attackers and the server, \sys generates a mask for each user model update and only transmit the masked update.
On the user side, a mask is generated with the shared secret of the user and each assisting node $x_{P_i}^{A_j}$ and the iteration number $t$.
As the shared secrets are calculated in setup phase and the iteration number is iterated in order, there is no any runtime information (i.e., local updates) involved.
Therefore, we can precompute $T$ masks for $T$ iterations before the runtime aggregation.




\subsection{Security Analysis}

\begin{theorem}\label{thm:malicious}
    The \sys~protocol presented in Algorithms \ref{alg:sysSetup} and \ref{alg:sysAgg}, running with $n$ parties $\{ \user_1,\dots, \user_n\}$, $k$ assisting nodes $\{\node_1,\dots,\node_k\}$,  and an aggregation server \agg~provides  post-quantum privacy against  a malicious adversary $A$~which controls \agg~and  $1-\alpha$ fraction of  users and $k-1$  assisting nodes with the offline rate $(1-\delta)\geq\alpha$.   
\end{theorem}

    


\begin{proof} \rouzbeh{in the proof below mention PQ security }

Following \cite{behnia2023efficient}, we prove the above theorem by the standard hybrid argument. The proof relies on the assumption of the simulator \Sim~that controls the environment. $\ppp_h$ and $\ppp_C$ define the set of honest and corrupt users, respectively.   

 

\smallskip
\noindent

\emph{Setup phase:}
\begin{enumerate}
    \item Each honest user $\user_i$ and assisting node $\node_j$ follows the protocol in Algorithm \ref{alg:sysSetup}.
    % by running $(\sk^{\user_i}_{\Sigma},\pk^{\user_i}_{\Sigma})\gets \Sigma.\kakeygen(1^\kappa)$ and $(\sk^{\node_i}_{\Sigma},\pk^{\node_i}_{\Sigma})\gets \Sigma.\kakeygen(1^\kappa)$, respectively. 
    \item For each  corrupt user $\user_{i'}\in\ppp_{C}$ and honest assisting node  $\node_j\in\aaa_H$,  compute  and store  $(\x_{\node_j}^{\user_{i'}}, c_{\node_j}^{\user_{i'}})\gets\kem.\kemenc(\pk_\kem^{\node_j})$.

    \item For each  honest user $\user_{i}\in\ppp_H$ and corrupt assisting node  $\node_{j'}\in\aaa_C$,  compute and store   $(\x_{\node_{j'}}^{\user_{i}}, c_{\node_{j'}}^{\user_{i}})\gets\kem.\kemenc(\pk_\kem^{\node_{j'}})$.
    \item For each honest pair of user $\user_i$ and honest assisting node $\node_j$, \Sim~ picks $\x_r\Ra\mathcal{K}_\Sigma$ and sets $   \x^{\user_i}_{\node_j}= \x_r$.
\end{enumerate}

\smallskip
\noindent
\emph{Aggregation phase:}
  
\begin{enumerate}
    \item In each iteration $t$ of the protocol, each honest user picks a random $\Vec{y'}_t^{\user_i}$. It then computes two signatures  $\sigma^{\user_i}_{\agg} \gets \Pi.\sgnsign(\sk^{\user_i}_\Pi,m)$ and $\sigma^{\user_i}_{\node_j} \gets \Pi.\sgnsign(\sk^{\user_i}_\Pi,m')$  and sends $(m{,\sigma^{\user_i}_{\agg}})$ and $(m'{,\sigma^{\user_i}_{\node_j}})$ to the aggregation server and the assisting node $\node_j $ (for $j\in[1,\dots,k]$), respectively. 
    \item The aggregation server  \agg~first adds the user $\user_i$ to the list $\Ulist_{\agg,t}$ and then calls the $\alpha$-summation ideal functionality $\mathcal{F}_{\Vec{x},\alpha}(\Ulist_{\agg,t}\backslash \mathcal{P}_{C})$ (where $\mathcal{P}_{C}$ is the set of corrupt users) to get $\Vec{w}_t$.

\item Next, the simulator samples $\Vec{w'}_t^{\user_i} \Ra \mathcal{M}^d$ for all $\user_i \in \Ulist_{\agg,t}\backslash \mathcal{P}_{C} $ such that $\Vec{w}_t=\sum_{i\in\mathcal{P}_{C}}\Vec{w'}_t^{\user_i} $ and computes $\Vec{a'}_{t}^{\user_i}=\Vec{y'}_t^{\user_i} - \Vec{w'}_t^{\user_i}$.
\Sim sets $\{\Vec{a'}_{\node_j,t}^{\user_i}\}_{\node_j \in \aaa_H} = \{\RO(\x_{\node_j}^{\user_i},t)\}_{\node_j\in\aaa_H}$ such that $\Vec{a'}_{t}^{\user_i}=\sum_{\node_j \in \aaa_H} \{\Vec{a'}_{\node_j,t}^{\user_i}\}$, and for each $\node_j\in\aaa_H$, it computes  $ \Vec{a'}_{\user_i,t}^{\node_j}=\sum_{\user_i\in\ppp_H}\Vec{a'}_{j,t}^{\user_i}$. 

\end{enumerate}

The hybrids are provided below. We note that each hybrid represents a view of the system seen by the adversary. The proof relies on the indistinguishability of each hybrid.  The hybrids are constructed by the simulator \Sim. 
% We present our hybrids below. The hybrids represent different views of the system as seen by corrupted entities e.g., aggregation server, assisting nodes, and/or users), and the proof is based on the assumption that these views are computationally indistinguishable from each other. The simulator \Sim~is used to construct these hybrids, and the adversary \adv~controls the corrupted entities.


 
\begin{description} 

\item [$\mathtt{Hyb0}$] The random variable is identical to the real execution of the protocol (i.e., \real). 
% \item [$\mathtt{Hyb0}$]  This random variable is distributed identically to \real, i.e., the real execution of the protocol where \adv~interacts with the honest entities.  
\item [$\mathtt{Hyb1}$] Now, \Sim~that knows the secrets of all honest entities is introduced in this hybrid. The distribution of this hybrid remains identical to the one above. 

% \item [$\mathtt{Hyb1}$] In this hybrid, a simulator \Sim~that has knowledge of all the secrets of the honest parties (in each iteration) is introduced. 

% The distribution of this hybrid is identical to the previous one. 
\item [$\mathtt{Hyb2}$] This hybrid replaces the shared keys between the users and assisting nodes with a random shared secret key sampled from  $\mathcal{K}_\mathtt{\Sigma}$.  The \indist of this hybrid is delivered by the security of the key encapsulation mechanism (Definition \ref{def:INDCCA}). Our protocol delivers this by the security of the CRYSTALS-Kyber algorithm  \cite{bos2018crystals}, which is based on the Module-LWE problem. 

% \item [$\mathtt{Hyb2}$] In this hybrid, we change the behavior of the simulated honest parties $\user_i \in \ppp_H$ and assisting nodes $\node_j \in \aaa_H$ by selecting a random shared secret key from the key space $\mathcal{K}_\mathtt{\Sigma}$ instead of instantiating the $\Sigma.keyagree(\cdot)$ algorithm. 

% The \indist of this hybrid with the one before is guaranteed by the security of the instantiated key exchange protocol. For instance with the Diffie-Hellman key exchange protocol, this is guaranteed by the 2ODH assumption \cite{bonawitz2017practical}. 
\item [$\mathtt{Hyb3}$] This hybrid starts with each honest user picking a random vector $\Vec{y'}^{\user_i}_t$. The user then computes a signature $\sigma^{\user_i}_{\agg} \gets \Pi.\sgnsign(\sk^{\user_i}_\Pi,<\Vec{y'}^{\user_i}_t,t>)$ and sends $(\Vec{y'}^{\user_i}_t,\sigma^{\user_i}_{\agg})$ to the server.  The \indist of this hybrid is due to the following. 1) Given we need at least one assisting node to remain honest, and since $A$ does not have the secret of honest entities, in \real, the masked gradient vector will have the same distribution as $\Vec{y'}^{\user_i}_t$ and therefore indistinguishable. 2) The  \indist of $\sigma^{\user_i}_{\agg}$ is delivered via the security requirement (Definition \ref{def:EUCMA}) of the underlying signature scheme. 

% \item [$\mathtt{Hyb3}$] In this hybrid, each honest user $\user_i\in\ppp_H$ samples a random vector $\Vec{y'}^{\user_i}_t$ for the update domain. It also computes a signature $\sigma^{\user_i}_{\agg} \gets \Pi.\sgnsign(\sk^{\user_i}_\Pi,<\Vec{y'}^{\user_i}_t,t>)$ and sends $(\Vec{y'}^{\user_i}_t,\sigma^{\user_i}_{\agg})$ to the server. Firstly, the \indist of $\sigma^{\user_i}_{\agg}$ is guaranteed by the underlying signature scheme. Secondly,  as aforementioned, we require at least one of the assisting nodes in our protocol to be honest. Therefore, the \indist of this hybrid is guaranteed since \adv~does not have knowledge on the honest entity's secret and hence in \real~the masked update will have the same distribution as $\Vec{y'}^{\user_i}_t$ in \simul.    

\item [$\mathtt{Hyb4}$] The ideal functionality $\mathcal{F}_{\Vec{x},\alpha}(\Ulist_{\agg,t}\backslash \mathcal{P}_{C})$ and random oracles are used to substitute the aggregated mask outputted by the honest assisting nodes  $\node_i\in\aaa_H$ with  $ \Vec{a'}_{\user_i,t}^{\node_j}$ (computed in Step 3 of the simulated Aggregation phase presented above). This hybrid outputs $( \Vec{a'}_{\user_i,t}^{\node_j},\sigma^{\node_i}_{\agg})$ where $\sigma^{\node_i}_{\agg} \gets \sgnsign(\sk^{\node_j}_\Pi,m'')$. Given the ideal functionality, random oracles, digital signatures, and since $A$ does not have the secret of honest entities, the view of this hybrid is \indist with the previous hybrid. 

% \item [$\mathtt{Hyb4}$] In this hybrid we call  the idea functionality $\mathcal{F}_{\Vec{x},\alpha}(\Ulist_{\agg,t}\backslash \mathcal{P}_{C})$ and utilize random oracles to  replace the aggregated masking  term outputted by the honest assisting nodes  $\node_i\in\aaa_H$ with  $ \Vec{a'}_{\user_i,t}^{\node_j}$ (computed in Step 3 of the simulated Aggregation phase presented above). The output of this hybrid is $( \Vec{a'}_{\user_i,t}^{\node_j},\sigma^{\node_i}_{\agg})$ where $\sigma^{\node_i}_{\agg} \gets \sgnsign(\sk^{\node_j}_\Pi,m'')$. The \indist of   $\sigma^{\node_i}_{\agg}$ is  provided via the security of the underlying signature scheme.  Hence, the view of this hybrid is \indist with the previous hybrid since \adv~does not have any knowledge on the honest entities shared secret and the distribution of the aggregate masking term in \simul~is identical to the one in \real. 


\item [$\mathtt{Hyb5}$] In the final hybrid, \Sim~outputs the output of the ideal functionality  (Step 2 in the simulated Aggregation phase)  as the global update $\vec{w}_t$. Given the assumption of the fraction of honest users/nodes, the ideal functionality will not output $\bot$ with an overwhelming probability. Thus, this hybrid is \indist from the previous one. 
% \item [$\mathtt{Hyb5}$]  In this hybrid, \Sim~sends the output of the ideal functionality  (as in Step 2 in the simulated Aggregation phase above)  as the universal model update $\vec{w}_t$ for iteration $t$. Note that the ideal functionality will not return $\bot$ based on the condition of the fraction of the honest users. Hence, this hybrid is \indist from the previous one given the local updates are not known by \adv~in \real. 



 


\end{description}
In the above, we have shown that the view of all the corrupted parties controlled by $A$~is computationally indistinguishable. 
 
\end{proof}
\rouzbeh{provide corollary for each TM, incorporation of DP}



\section{Evaluation}

We answer the following Research Questions (RQs).
\begin{itemize}
\item \textbf{RQ1}: What is the performance of post-quantum enhanced secure aggregation on FL?
% \item \textbf{RQ2}: How does \sys improve it by introducing pre-computation method?
% \item \textbf{RQ2}: How does differential number of clients affect the performance of \sys?
\item \textbf{RQ2}: How does the differential privacy module in \sys work under different threat models?
\item \textbf{RQ3}: What is the performance of the DP-enhanced method on FL among different training datasets?
\end{itemize}

\subsection{RQ1: Post-quantum Enhanced SA+FL Performance}


\subsubsection{Computation}
We discuss the computation cost of \sys in the Setup phase and Aggregation phase separately.

\input{tables/sa_time}

\noindent
\textbf{Setup Phase.}
Figure~\ref{fig:sa_setup_time} depicts the computation cost of our protocol in the Setup phase compared with the one in \flamingo and the one in \micro.
The results show that \sys generally has a better performance than \flamingo and \micro in terms of the computation cost in Setup phase, as the computation time of \sys on server and assisting node sides is greatly lower than that of \flamingo and \micro though the computation time of \sys is slightly higher than \microsecond on the client side.

\begin{itemize}
\item Server and Assisting Node: \sys takes less time than \flamingo and \micro during Setup phase. 
This is because during the setup phase, the server and assisting nodes of \sys only generate their key pair and send their public key to the users. 
Except generating and sending the public key, the server and decryptors of \flamingo have to perform the distributed key generation (DKG) protocol to generates and distribute secret key shares for the asymmetric encryption scheme among the decryptors, without revealing the key to any single entity. 
For \micro, the server have to, on the hand, receive the encryption keys of users and verified the signatures, and on the other hand, involve in user mask sharing and check if the online users are enough.

\item User: \sys takes less time than \flamingo and \microfirst but more time than \microsecond. This is because the users of \sys perform key generation, key exchange to generate shared secret with each assisting node, and send the public key to the server.
The users involved in \flamingo have to receive public keys from decryptors and verify their signatures.
The user computation time of both \sys and \flamingo is proportional to the number of assisting nodes/decryptors but constant to the number of users. 
For \microfirst, the user has to perform mask sharing among other users, the computation of which is larger than secret sharing between the users and assisting nodes in \sys.
For \microsecond, the user only distributes shares among the other users in the same group.
\end{itemize}


% Specifically, the server in \sys takes 0.07 ms to setup (generate a \texttt{Kyber} key pair and a \texttt{Dilithium} key pair), compared to 26.74 ms for \flamingo.
% \todo{In \flamingo protocol, given their design, xxxx (why).}
% For \micro protocol, both \microfirst and \microsecond take linear computation time with the number of clients. 
% That is, the more clients are involved in FL, the worse performance \microfirst and \microsecond will have than \sys.
% \todo{This is resulted from xxx}
% The client in \sys takes 9.66 ms to generate the key pairs and shared secret with each assisting node, which is better than \flamingo and \microfirst but worse than \microsecond.
% \todo{In \flamingo protocol, given their design, xxxx (why).}
% \todo{\microfirst xxx \microsecond xxx.}
% Additionally, when comparing the computation cost of assisting nodes in \sys and that of decryptors in \flamingo, \sys is better than \flamingo for the tested number of users. But it will exceed \flamingo when xxx as the time cost is linear of the number of users.
% \todo{This is because \sys xxx while \flamingo xxxx}

% Thus, our protocol is xxx - xxxx (for the defined number of users range) faster than \flamingo and xxx - xxx faster than \micro.

\noindent
\textbf{Aggregation Phase.}
Figure~\ref{fig:sa_agg_time} depicts the computation cost of \sys in aggregation phase compared with the one in \flamingo and the ones in \micro.
The results show that all entities in our protocol incur a small computation overhead and all the computation time in our protocol is faster than \flamingo and \micro regarding users, assisting nodes, and the server.

\begin{itemize}
\item The reason why \micro take the most cost is because each user has to calculate $H(k)^{X_i}$ and $H(k)^{R_i}$ and the server recover the vector by calculating the discrete log of $H(k)^{X_i} - H(k)^{R_i}$. Such a calculation of the discrete log is extremely expensive, which takes even more time as the dimensions of vector are very large.
\item The reason why \flamingo takes more time than \sys is \todo{because \flamingo will remove the masks for those dropout users. Thus the users and decryptors have to provide additional materials (e.g., secret shares) for server to recover the local vector. \sys adopts a straightforward strategy, that is, it just removes and ignores the masked vectors of dropout users, which may lower message utilization, but remove unnecessary calculations, greatly reducing time overhead.}
\end{itemize}

% The results show that \sys generally has a better performance than \flamingo and \micro in terms of the computation cost in Setup phase, as the computation time of \sys on server and assisting node sides is greatly lower than that of \flamingo and \micro though the computation time of \sys is slightly higher than \micro on the client side.
% \todo{This is because \micro does not generate a signature for its masked input.
% Although it generates a signature for the online set, but the signing algorithm is simple without taking too much time but achieving low security.}




% \begin{figure*}[htbp]
%     \centering
%     \begin{minipage}{0.32\textwidth}
%         \centering
%         \includegraphics[width=\textwidth]{figures/sa_setup_time/sa_time_setup_server_nopre.pdf}
%         \caption*{(a) Server}
%     \end{minipage}
%     \hfill
%     \begin{minipage}{0.32\textwidth}
%         \centering
%         \includegraphics[width=\textwidth]{figures/sa_setup_time/sa_time_setup_client_nopre.pdf}
%         \caption*{(b) User}
%     \end{minipage}
%     \hfill
%     \begin{minipage}{0.32\textwidth}
%         \centering
%         \includegraphics[width=\textwidth]{figures/sa_setup_time/sa_time_setup_node_nopre.pdf}
%         \caption*{(c) Assisting node}
%     \end{minipage}
%     \caption{Computation in the Setup phase (The dimension of the weight list is set to 16K.)}
%     \label{fig:sa_setup_time}
% \end{figure*}


% \begin{figure*}[htbp]
%     \centering
%     \begin{minipage}{0.32\textwidth}
%         \centering
%         \includegraphics[width=\textwidth]{figures/sa_agg_time/sa_time_agg_server.pdf}
%         \caption*{(a) Server}
%     \end{minipage}
%     \hfill
%     \begin{minipage}{0.32\textwidth}
%         \centering
%         \includegraphics[width=\textwidth]{figures/sa_agg_time/sa_time_agg_client.pdf}
%         \caption*{(b) User}
%     \end{minipage}
%     \hfill
%     \begin{minipage}{0.32\textwidth}
%         \centering
%         \includegraphics[width=\textwidth]{figures/sa_agg_time/sa_time_agg_node.pdf}
%         \caption*{(c) Assisting node}
%     \end{minipage}
%     \caption{Computation in the Aggregation phase (The dimension of the weight list is set to 16K.)}
%     \label{fig:sa_agg_time}
% \end{figure*}

\subsubsection{Outbound bandwidth}
We discuss the outbound bandwidth cost of \sys in the Setup phase and Aggregation phase separately.

\input{tables/sa_size}

\noindent
\textbf{Setup Phase.}
We present the outbound bandwidth cost of all entities in \sys during the Setup phase in Figure~\ref{fig:sa_setup_bw}. 
The outbound bandwidth cost of \sys is less than that of \micro and \flamingo.

\begin{itemize}
\item Server: the server of \sys broadcasts its public key to the user, thus its bandwidth depends on the size of public key. The server of \flamingo gets involved in the DKG protocols, in which the bandwidth depends on the messages of DKG protocols and is proportional to the number of decryptors but constant to the number of clients. The server of \micro forwards the public keys and secret shares of one user to the other users, thus its bandwidth is proportional to the number of clients.
\item User: We do not consider \flamingo here as the user in \flamingo does not send any messages. The user of \sys should send its public key and the encrypted secret to each assisting node, thus its bandwidth is constant to the number of users. The user of \micro should send its public key and (N-1) mask shares to the other users separately, so its bandwidth is proportional to the number of clients, more than that of \sys.
\item Assisting Node: During the setup phase, each assisting node of \sys should send its public key to each user, thus its bandwidth is proportional to the number of users. The decryptor of \flamingo gets involved in the DKG protocols, in which the bandwidth depends on the messages of DKG protocols and is proportional to the number of decryptors but constant to the number of clients.
\end{itemize}



\noindent
\textbf{Aggregation Phase.}
We present the outbound bandwidth cost of all entities in \sys during the Setup phase in Figure~\ref{fig:sa_agg_bw}. 
The outbound bandwidth cost of \sys on all entities is less than that of \micro and \flamingo.

\begin{itemize}
\item Server: The server of \sys has to only broadcast the final update during the aggregation phase, thus its outbound bandwidth is the size of final length and constant to the number of users. The server of \flamingo should get involved in forwarding the user message to the decryptors to recover the masks of dropout clients, as well as broadcast the final update, thus its bandwidth is more than that of \sys and roughly proportional to the number of users. The server of \micro has to report the online user set to each user and forwards the signature of each user to other users, as well as distribute the final update, thus its bandwidth is more than \sys and \flamingo and proportional to the number of users.
\item User: The user of \sys sends the masked update and the iteration number to the server and assisting nodes separately, thus its bandwidth depends on the size of the update vector and is proportional to the number of assisting nodes, but constant to the number of users.
The user of \flamingo sends the masked update to sever and the secret shares of the decryptors and its neighbors to decryptors, thus its bandwidth is proportional to the number of decryptors and the number of users (i.e., neighbors).
The user of \micro sends its masked update, the signature of online set and the masks of online users to the server, thus its bandwidth is constant to the number of users, smaller than \flamingo but higher than \sys.
\item Assisting Node: The assisting node of \sys should send the sum of masks of online users to the server, thus its bandwidth is the size of update and constant to the number of users.
The decryptor of \flamingo has to send the decrypted secret shares (i.e., same size with the update) of each users to the server, thus its bandwidth is proportional to the number of users and larger than \sys.
\end{itemize}


% For 1000 users, the server transmits ~x-x orders of magnitude less than \flamingo and ~x-x orders of magnitude less than \micro.
% The server bandwidth in \sys protocol grows linearly as the number of users increases because xxx.
% In \flamingo, however, due to the design, xxxx
% In \micro, xxxx
% Thus, user bandwidth in \sys is xxx - xxx less than \flamingo and xxx - xxx less than \micro, respectively.
% The bandwidth cost of assisting nodes in \sys is negligible where each xxx.
% As the overhead is due to xxx, its bandwidth cost grows linearly xxx

% In Figure xxx, we compare the outbound bandwidth costs of the Aggregation phase for all the entities in our protocol with the one in \flamingo and the one in \micro.
% We have observed that the outbound bandwidth cost for the server and the user in our protocol is considerably lower than those in the \flamingo and \micro protocols.
% xxxx

% \begin{figure*}[htbp]
%     \centering
%     \begin{minipage}{0.32\textwidth}
%         \centering
%         \includegraphics[width=\textwidth]{figures/sa_setup_size/sa_size_setup_server.pdf}
%         \caption*{(a) Server}
%     \end{minipage}
%     \hfill
%     \begin{minipage}{0.32\textwidth}
%         \centering
%         \includegraphics[width=\textwidth]{figures/sa_setup_size/sa_size_setup_client.pdf}
%         \caption*{(b) User}
%     \end{minipage}
%     \hfill
%     \begin{minipage}{0.32\textwidth}
%         \centering
%         \includegraphics[width=\textwidth]{figures/sa_setup_size/sa_size_setup_node.pdf}
%         \caption*{(c) Assisting node}
%     \end{minipage}
%     \caption{Bandwidth in the Setup phase (The dimension of the weight list is set to 16K.)}
%     \label{fig:sa_setup_bw}
% \end{figure*}

% \begin{figure*}[htbp]
%     \centering
%     \begin{minipage}{0.32\textwidth}
%         \centering
%         \includegraphics[width=\textwidth]{figures/sa_agg_size/sa_size_agg_server.pdf}
%         \caption*{(a) Server}
%     \end{minipage}
%     \hfill
%     \begin{minipage}{0.32\textwidth}
%         \centering
%         \includegraphics[width=\textwidth]{figures/sa_agg_size/sa_size_agg_client.pdf}
%         \caption*{(b) User}
%     \end{minipage}
%     \hfill
%     \begin{minipage}{0.32\textwidth}
%         \centering
%         \includegraphics[width=\textwidth]{figures/sa_agg_size/sa_size_agg_node.pdf}
%         \caption*{(c) Assisting node}
%     \end{minipage}
%     \caption{Bandwidth in the Aggregation phase (The dimension of the weight list is set to 16K.)}
%     \label{fig:sa_agg_bw}
% \end{figure*}


\subsubsection{Precomputation Improvement}


\input{tables/precomputed}

\yiwei{Precomputation could greatly improve the efficiency on assisting nodes with the increasing number of clients.}

% \subsubsection{Number of Clients}
% We explore how different number of clients (ranging from 200 to 1000) affects the performance of secure aggregation in \sys.
% xxx and xxx show the computation time and outbound bandwidth of \sys when the number of clients varies.
% We observe that \sys consistently outperforms xxx and xxx in both time and bandwidth, especially when the system has more clients.
% For instance, the xxx gap between \sys and xxx increases from xxx\% with 200 clients to xxx\% with 1000 clients.




\subsection{RQ2: DP+FL Performance under different threat models}


\input{tables/dp_acc}

% To evaluate the performance of our DP methods in FL, we conducted experiments using two benchmark datasets: MNIST and CIFAR-10. 
% The goal was to assess the impact of different DP methods on the accuracy of the models while preserving privacy, under different threat models. 

We assessed the accuracy of models trained using the MNIST and CIFAR-10 datasets across three differential privacy (DP) methods, i.e., ODP, CDP, LDP, and the Non-Differential Privacy (NDP) method as a baseline. Table~\ref{tab:dp_acc} presents the testing accuracies (i.e., the best accuracy) for FL models under these DP methods, varying by privacy budget $\epsilon$.

Generally, the NDP method, which does not add noise, achieved the highest accuracy. On average, ODP, CDP, and LDP methods resulted in accuracy reductions of approximately 5\%, 13\%, and 20\%, respectively. Notably, ODP exhibited superior accuracy compared to CDP and LDP. This is attributed to the fact that ODP only adds one-time noise at the final iteration, whereas CDP and LDP introduce noise at each iteration.
% on the aggregated model, and LDP applies noise to individual client data transformations at every iteration.
The reason why CDP generally achieves higher accuracy than LDP, particularly at larger $\epsilon$ values is CDP adds noise to the aggregated results, allowing the model to learn global patterns despite the presence of noise, whereas LDP applies noise to individual client data transformations, diminishing the model's ability to utilize data correlations and global information effectively.

Furthermore, we observed that accuracy improves with increasing $\epsilon$ across all three DP methods. This trend occurs because smaller $\epsilon$ values introduce more noise, increasing data heterogeneity. The accuracy improvement in CDP with larger $\epsilon$ values surpasses that of ODP and LDP, as CDP's noise addition during intermediate model aggregation allows for more effective training. In contrast, either the one-iteration noise in ODP or the dispersed impact of noise in LDP results in a smaller overall influence on the model. 



\begin{tcolorbox}[colback=gray!10,colframe=black,boxrule=1pt]
\textbf{Takeaway:} Although applying differential privacy does introduce a trade-off between privacy and accuracy, our DP methods managed to maintain a high level of accuracy close to that of the NDP baseline while ensuring data privacy. 
\end{tcolorbox}

% Consequently, CDP generally achieves higher accuracy than LDP, particularly at larger $\epsilon$ values, as CDP allows the model to learn global patterns despite the presence of noise, whereas LDP's per-data-point noise diminishes the model's ability to utilize data correlations and global information effectively.



% We measured the accuracy of the models trained using the MNIST and datasets for four DP methods, i.e., ODP, CDP, LDP, as well as Non-DP (NDP) as the baseline. 
% Table~\ref{tab:dp_acc} shows the testing accuracy of FL model training using different DP methods when the privacy budget $\epsilon$ varies.
% Generally, the NDP method had the best accuracy as no additional noise was added.
% For ODP, CDP and LDP, there were 5\%, 13\% and 20\% deduction of accuracy on average, respectively.
% % Such deductions are tolerable in pracice~\cite{}.
% Moreover, we found that the accuracy of ODP is better than that of CDP, which is better than that of LDP.
% The reason is that ODP only requires one-time adding noise at the last iteration while CDP requires adding noise at each iteration on the aggregated model, both of them are more efficient in mitigating the heterogeneity compared with LDP which adds noise to the individual data transformation on the client.
% Additionally, we observed that for all three DP methods, the accuracy becomes higher when $\epsilon$ is larger. 
% This is because DP introduces more heterogeneity among the clients when $\epsilon$ is smaller as the noise is large.
% The reason why the increase in accuracy of CDP is greater than that of LDP as $\epsilon$ increases is the noise in CDP is added during the intermediate model aggregation on the server, in which the training performance can be more significantly improved with the decreasing of noise, while the noise in LDP works separately on each data point, in which the impact of noise is relatively dispersed, resulting in a smaller overall impact on the model.
% Furthermore, the overall accuracy of CDP is better than that of LDP, especially when $\epsilon$ is larger. This is because the noise in LDP works on separate data points, resulting in the model being unable to fully utilize the correlation and global information between data and leading to a lower overall accuracy of the model.
% In CDP, noise is added based on the aggregated intermediate model, which enables the model to effectively learn global patterns in the data even after adding noise. 



% In centralized differential privacy, noise is usually added during the global model update or data aggregation process. In this way, the influence range of noise is relatively large, which can more significantly change the training results of the global model. Therefore, as ϵ increases, the added noise decreases and the impact on the model gradually decreases, resulting in a significant improvement in accuracy.
% LDP (Local Differential Privacy): In local differential privacy, noise is added separately on each data point. This means that the impact of noise is relatively dispersed, and the amount of noise added to each data point is small, resulting in a smaller overall impact on the model. In addition, as noise is local, increasing ϵ does not significantly reduce the impact of noise, especially within a specific range of each data point. This may result in less significant improvement in accuracy as ϵ increases.



% Our results show that the introduction of differential privacy does introduce a trade-off between privacy and accuracy. However, our DP methods, particularly the ODP and CDP, managed to maintain a high level of accuracy close to that of the NDP baseline, with only a slight degradation. 
% This indicates that our approach effectively balances privacy preservation with model performance.
% The slight reduction in accuracy can be attributed to the noise added to ensure differential privacy, which can obscure important features of the data. 


% Table~\ref{tab:dp_acc} shows the accuracy of FL training using MNIST and CIFAR10 datasets under different threat models.
% In addition to the three DP strategies mentioned in Section~\ref{sec:pqfl:dp} (i.e., ODP, CDP, and LDP), we also add the Non-DP FL training as the baseline.
% Generally, 

% With the increasing of iterations, the difference among the accuracy of DP strategies are becoming smaller.


% \yiwei{To illustrate there is no significant loss in accuracy}


% \begin{figure}[!ht]
%   \centering
%   \includegraphics[width=1\linewidth]{figures/dp_acc.pdf}
%   \caption{The Accuracy of Different Privacy Module (MNIST)}
%   \label{fig:dp_acc}
% \end{figure}

\subsection{RQ3: DP+FL Performance under different parameters}

\input{tables/dp_params}

To further understand the trade-offs involved, we investigated the impact of varying noise parameters on our DP methods. 
Based on our investigations~\cite{opacus}, the accuracy of FL model training is mainly affected by the number of involved FL clients and the added noise, which depends on three parameters: $\epsilon$, the number of iterations, and the sample rate.
The results are listed in Table~\ref{tab:dp_param}.

\noindent
\textbf{Number of Clients.}
With the increasing number of clients, the accuracy of CDP is increasing, up to x1.43, as having more data from more clients or training with more iterations can help in better generalization, improving the model's performance, while keeping the same noise.
But LDP, the more clients there are, the worse the accuracy is.
This could be due to the fact that adding more noise at the local level for a larger number of clients aggregates to a higher total noise, degrading the overall model accuracy.

\noindent
\textbf{$\epsilon$.}
As $\epsilon$ increases, the accuracy of CDP and LDP generally improves, up to x1.09 and x1.03.
This is because a higher $\epsilon$, which corresponds to weaker privacy guarantees, allows for less added noise to reduce the distortion in the aggregated results, thus improving model performance.

\noindent
\textbf{Number of Iterations.}
With the increasing number of iterations, the accuracy of CDP and LDP is increasing, even though the added noise is becoming larger.
This may result from the basic principle of FL training, that is, the more clients are involved and the more iterations are conducted, the better performance will be achieved.

\noindent
\textbf{Sample Rate.}
Our results show that the accuracy of CDP and LDP is slightly increasing when the sample rate is becoming larger, due to its double side impact.
The sample rate of clients, on the one hand, affects the number of involved clients, and a larger sample rate will lead to better accuracy as more client data is used for training.
On the other hand, it can also decide the added noise for privacy protection.
With the increase of the sample rate, its two impacts are offset.


\begin{tcolorbox}[colback=gray!10,colframe=black,boxrule=1pt]
\textbf{Takeaway:} 
% While higher noise levels provide stronger privacy guarantees, they also reduce model accuracy. 
A careful balance is necessary based on the specific privacy requirements of the applications, where the noise parameters are optimized to provide adequate privacy without unduly compromising the model's performance. 
\end{tcolorbox}

% In summary, our results indicate that while higher noise levels provide stronger privacy guarantees, they also reduce model accuracy. This necessitates a careful balance, where the noise parameters are optimized to provide adequate privacy without unduly compromising the model's performance. The choice of noise parameters can also be influenced by the sensitivity of the training data and the specific privacy requirements of the application.

% Moreover, the accuracy improves with the increasing number of iterations and client sample rate, even though the added noise is becoming larger.
% This may result from the basic principle of FL training, that is, the more clients are involved and the more iterations are conducted, the better performance will be achieved.
% In addition, with the increasing number of clients and same noise, the best accuracy is increasing, up to x1.43, as having more data from more clients or training with more iterations can help in better generalization, improving the model's performance.


% Things are similar for $\epsilon$, the number of iterations and the sample rate in LDP settings, as the more $\epsilon$ and the less iterations and sample rate are, the less noise will be added to the model training to protect privacy.
% But for the number of clients, the more clients there are, the worse the accuracy is.
% This could be due to the fact that adding more noise at the local level for a larger number of clients aggregates to a higher total noise, degrading the overall model accuracy.
% the more noise will be added in total, as LDP adopts DP (i.e., adding noise) at each client side.





% This a higher ε, which corresponds to weaker privacy guarantees, allows for better accuracy. The noise added to the data decreases with increasing ε (from 9.04 to 5.21), reducing the distortion in the aggregated results and thus improving model performance.
% LDP: Accuracy remains relatively flat at 0.68 regardless of ε. This suggests that LDP might be more resistant to changes in ε in terms of performance, potentially due to more noise being added at the local level, which might not reduce as significantly with increasing ε.

% Our analysis revealed that increasing the noise parameter generally leads to a decrease in accuracy, as the injected noise becomes more significant relative to the signal in the data. However, different DP methods responded differently to changes in noise levels. For instance, LDP, which applies noise at the local client level, showed a more pronounced decrease in accuracy compared to CDP, which aggregates the noise at the central server.

% The results indicate that while higher noise levels provide stronger privacy guarantees, they also reduce model accuracy. This necessitates a careful balance, where the noise parameters are optimized to provide adequate privacy without unduly compromising the model's performance. The choice of noise parameters can also be influenced by the sensitivity of the training data and the specific privacy requirements of the application.

% \yiwei{The performance of DP mainly depends on three parameters: epsilon, the number of iterations, and sample rate.
% The larger epsilon is, the less noise is added, the higher accuracy is.
% The less iterations are, the less noise is added, the higher accuracy is.
% The less sample rate is, the less noise is added, the higher accuracy is.}


% MNIST and CiFAR-10



\section{Performance Evaluation }
\subsection{Analytical Performance}
\begin{table*}[!t]
	\centering
 \footnotesize
	 \caption{Analytical performance of the secure aggregation of \sys~and its counterparts}
	\label{tab:analytical}\vspace{-1em}
 	 \resizebox{1\textwidth}{!}{
	\begin{threeparttable}
	\begin{tabular}{|c|c|c|c||c|c|c|}
			\hline
		\multirow{2}{*}{\textbf{Scheme}} & \multicolumn{3}{c||}{\textbf{Setup Phase}} & \multicolumn{3}{c|}{\textbf{Aggregate Phase} }	\\	 \cline{2-7}
		 & \textbf{User} &
		 \begin{tabular}{@{}c@{}c@{}}
		 \textbf{Assisting/Helper} \\ \textbf{Nodes} \end{tabular}& \textbf{Server} &
		 \textbf{User} &
		 \begin{tabular}{@{}c@{}c@{}}
		 \textbf{Assisting/Helper} \\ \textbf{Nodes} \end{tabular} & \textbf{Server}	\\	\hline
% 		  \cite{Bell2020} & N/A & N/A & N/A
% &\begin{tabular}{@{}c@{}c@{}}
% $2_\Kg+2_{\sshl} +\log n (1_\SEnc+1_\SDec + $ \\
% ${1_\Ka + 2_\Sgn+2_\Vfy})+(2\log n)_\Su$ \end{tabular}& N/A &$1_\Rssh + 2\log n_\Su$\\\hline


MicroFedML \cite{microfedml} &
		\begin{tabular}{@{}c@{}c@{}} $1_\Kg + 1_\Sgn+|U'-1|(1_\Vfy+$
		\\
		$1_\Ka + 1_{\sshl} + 1_\AEnc+1_\ADec)$
		\end{tabular} & N/A
		& ${|U|_\Vfy }$
		&\begin{tabular}{@{}c@{}c@{}} $(|w|+1)_\Ex+1_\Sgn+$\\$|U-1|(1_\Su+1_\Vfy)+1_\Su$ \end{tabular}& N/A & \begin{tabular}{@{}c@{}c@{}} $1_{\Rsshe} +|w|_\Ex + $\\
		$1_\Mu$\end{tabular}	\\	\hline

  
	Flamingo	\cite{flamingo} &
		$|D'|_\Vfy$
		& \begin{tabular}{@{}c@{}c@{}}$2_{\PIL} + 3_\Sgn+2_{\sshl} +$	\\ $	|D|(3|D'|+1)_\Vfy + $\\
		$(|D'|\cdot|D|)_\Mu$\end{tabular}
		& $(|D'|\cdot|D|)_\Vfy$ & \begin{tabular}{@{}c@{}c@{}} $2_\PRG+|D'|(1_\Ex+1_\Hash+1_\PRF+$\\$1_\Su+1_\AEnc+1_\Sgn+1_\SEnc)+1_{\sshl}$ \end{tabular}&\begin{tabular}{@{}c@{}c@{}}$1_\Sgn+|U'|_\SDec +$ \\ $(|D|+|U'|)_\Vfy
		$\end{tabular}
		&
		\begin{tabular}{@{}c@{}c@{}} $|D|_{\PIL}+|U'|(1_\Su + $ \\ $1_\Mu +1_\Rssh)+2_\PRG+ $ \\ $ (|U'|+1)_\Su $ \end{tabular}
		\\	\hline
		
		


		 \sys &
		 $2_\Kg + k_\Ka$
		 & $2_\Kg + k_\Ka$
		 & $1_\Kg$
		 & $k_\PRF+|k+1|_\Su+2_\Sgn$ &\begin{tabular}{@{}c@{}c@{}} $|U'| (1_\Vfy+1_\Su+ $\\
		 $1_\PRF)+ {1_\Sgn}$\end{tabular}
		 & \begin{tabular}{@{}c@{}c@{}}$(|U'|+|k|)(1_\Vfy + $ \\ $1_\Su)$
		 \end{tabular}\\
		 \hline
		 		 
	\end{tabular}
\begin{tablenotes}[para, flushleft]
	 
	$\Kg$, $\Sgn$, $\Vfy$, and $\Hash$ denote key generation, signature generation, verification, and hash function, respectively.
	$\Ka$ denotes the shared key computation in the key agreement protocol.
	$|D|$ and $|D'|$ denote the number of all decryptors and the threshold of participating decryptors~\cite{sp/MaWAPR23}, respectively.
	$\PIL$ denotes polynomial interpolation of length $L$.
	$\sshl$, $\Rssh$, and $\Rsshe$ denote secret sharing operation to $l$ shares, share reconstruction, and share reconstruction in the exponent, respectively.
	$\Mu$, $\Su$ and $\Ex$ denote multiplication, summation and exponentiation operations, respectively.
	$\PRG$ and $\PRF$ denote pseudorandom generators and pseudorandom functions, respectively.
	$\AEnc$, $\ADec$, $\SEnc$, and $\SDec$ denote asymmetric encryption, decryption, symmetric encryption, and decryption, respectively.
	$|w|$ denotes the number of model parameters.
	$k$ is the set of assisting nodes in \sys.
 
	\end{tablenotes}
	\end{threeparttable}
		 }
   
\end{table*}

\subsection{Implementation}



% \vspace{5pt}
% \noindent
% \textbf{Implementation.}
We implement \sys in 2.5k lines, involving two components the secure aggregation for local updates and the model training with DP protection.
Our code is available at \url{https://github.com}.

\noindent
\textbf{Secure Aggregation.}
The end-to-end FL implementations of \sys are based on ABIDES~\cite{byrd2019abides}, a discrete event simulation framework with modifications to enable the simulation of multi-iterative aggregation protocols.
We adopt two post-quantum algorithms, i.e., \texttt{Kyber} key encapsulation algorithm~\cite{bos2018crystals} and users and \texttt{Dilithium}~\cite{ducas2018crystals}, to negotiate shared secrets between clients and assisting nodes and generate digital signatures for each message during aggregation phase, respectively.
Both of the two algorithms are implemented based on existing libraries~\cite{}, with several modifications to support signing with precomputation, which is implemented in the C language.
For the Pseudo-Random Function (PRF) used to generate the masks, we use \texttt{ASCON}~\cite{dobraunig2021ascon} which implements lightweight and efficient cryptography, suitable for limited-resource client devices.

\noindent
\textbf{Model Training with DP Protections.}
We follow the previous work~\cite{yang2023privatefl} to instantiate FL model training.
The DP privacy protection is incorporated via \texttt{PyTorch Opacus}\cite{opacus}.
We implement three DP methods under different threat models, as described in Section~\ref{sec:pqfl:dp}, as well as the one without DP protections as the baseline.

\subsection{Experimental Environment}
All experiments are conducted on an x86\_64 Linux machine with AMD Ryzen Threadripper PRO 5965WX 24-Cores and 256 GB RAM. 
The model training is performed using three GeForce RTX 3090 graphics cards (NVIDIA).
We use multiple benchmark datasets following previous FL works~\cite{}, i.e., MNIST~\cite{xiao2017fashion} and CIFAR-10~\cite{krizhevsky2009learning}, with model choices of Fully-connected and ResNet-18 respectively. 



\subsection{Experimental Setup and Evaluation Metrics}
To evaluate the performance of \sys, we adopt three metrics: computation time, communication cost, and the accuracy of the final model.

\noindent
\textbf{Computation Time.}
We record the time taken by computational operations, such as key encapsulation, mask generation, signing and verifying, to evaluate the efficiency of our secure aggregation method with post-quantum protections.
Specifically, we vary the user count from 200 to 1000 with three assisting nodes and one aggregation server. 
We also adopt $w$ with 16,000 gradients to test the performance under high-dimensional gradient vectors. 
Moreover, \flamingo～\cite{flamingo} and \micro～\cite{microfedml} are chosen for comparative analysis. 
To have a similar environment for the comparative analysis, we employ an identical setup for \micro and \falmingo. 
We select three decryptors for \flamingo.

\noindent
\textbf{Communication Cost.}
We record the total size of messages transmitted between each entity, i.e., clients, assisting nodes and the server, to evaluate the communication cost.
% The reason why we use message size instead of transmission time is because message transmission time highly depends on current network conditions. Variations in hardware and network quality can greatly affect latency.

\noindent
\textbf{Accuracy.}
We use the accuracy of the final models to evaluate the efficient of our DP methods.
Training data assignment to clients follows established protocols~\cite{yang2023privatefl}. 



We separately evaluate the components of \sys. 
Generally, evaluation metrics include the computation time and outbound bandwidth for secure aggregation, and the accuracy for training with differential privacy. 

For secure aggregation, we vary the user count from 200 to 1000, utilizing three assisting nodes and one aggregation server. 
Performance with high-dimensional gradient vectors, specifically $w$ with 100,000 gradients, is reported. 
\flamingo\cite{flamingo} and \micro\cite{microfedml} are chosen for comparative analysis. 
\todo{To have a similar environment for the comparative analysis, we employ an identical setup for \micro. 
We select a range of 200 to 1000 users, three decryptors, and one aggregation server as the setting of \flamingo.}

The differential privacy module is assessed on two real-world datasets, i.e., MNIST~\cite{xiao2017fashion} and CIFAR-10~\cite{krizhevsky2009learning} datasets, with model choices of Fully-connected and ResNet-18 respectively. 
\todo{Training data assignment to clients follows established protocols~\cite{yang2023privatefl}. 
Default parameter settings are detailed in Table xxx, adhered to unless stated otherwise.}



% We implement \sys with 205+250+336+330+335+322+404 lines of Python code and 322 lines of C code. 
% \sys is based on the existing federated learning framework~\cite{}. 
We follow the previous work~\cite{yang2023privatefl} to instantiate FL applications.
We use \texttt{ASCON}~\cite{dobraunig2021ascon} as the Pseudo-Random Function (PRF), \texttt{Kyber} key encapsulation algorithm~\cite{bos2018crystals} to generate shared secrets between assisting nodes and users, and \texttt{Dilithium}~\cite{ducas2018crystals} to generate digital signatures.
Differential privacy is incorporated via \texttt{PyTorch Opacus}\cite{opacus}.
Our codebase is publicly available at (xxx).

\yiwei{ABIDES: Towards High-Fidelity Market Simulation for AI Research~\cite{byrd2019abides}}

$\text{latency} = \text{min\_latency} + \left(\frac{a}{x^3}\right) \times \left(\frac{\text{min\_latency}}{\text{unit}}\right) \times \left(\frac{\text{message\_size}}{10000}\right)$

\yiwei{
To generate latency in the LatencyModel class using the cubic model, several parameters are involved. The latency is calculated based on the minimum latency between the sender and recipient, combined with a random $jitter$ component. The jitter component is influenced by the $jitter$, $jitter\_clip$, and $jitter\_unit$ parameters, which control the shape and extent of the random noise added to the latency. Additionally, the final latency is scaled by the size of the message being sent. The process involves drawing a random value x from a uniform distribution within the $range (jitter\_clip, 1.0]$, and using this value in the cubic equation to compute the additional $jitter$. The formula ensures that larger messages incur higher latency, reflecting real-world network behavior where message size impacts transmission time.

x is a random variable drawn from a uniform distribution in the $range (jitter\_clip, 1.0]$, introducing randomness into the latency calculation.

$jitter$ (denoted as $a$) is a parameter that controls the shape of the cubic curve for the additive latency noise, determining the magnitude of the $jitter$ in the cubic equation. A higher $jitter$ value will result in greater variability in the latency.

$jitter\_clip$ is a parameter that sets the minimum value of the uniform range from which $x$ is drawn. By setting a minimum value for $x$, $jitter\_clip$ effectively clips the cubic curve, limiting the maximum possible value of the $jitter$ term. 

$jitter\_unit$ is a parameter that scales the unit of measurement for $jitter$ relative to the $min\_latency$, adjusting the influence of $min\_latency$ on the $jitter$ calculation. It normalizes the $jitter$ term so that the impact of $jitter$ is proportional to the minimum latency between the sender and recipient.
}

\yiwei{ns3}

\vspace{5pt}
\noindent
\textbf{Experimental Setup and Metrics}
Experiments are conducted on an \todo{x86\_64 Linux machine with AMD Ryzen Threadripper PRO 5965WX 24-Cores and 256 GB RAM}. 
We separately evaluate the components of \sys. 
Generally, evaluation metrics include the computation time and outbound bandwidth for secure aggregation, and the accuracy for training with differential privacy. 

For secure aggregation, we vary the user count from 200 to 1000, utilizing three assisting nodes and one aggregation server. 
Performance with high-dimensional gradient vectors, specifically $w$ with 100,000 gradients, is reported. 
\flamingo\cite{flamingo} and \micro\cite{microfedml} are chosen for comparative analysis. 
\todo{To have a similar environment for the comparative analysis, we employ an identical setup for \micro. 
We select a range of 200 to 1000 users, three decryptors, and one aggregation server as the setting of \flamingo.}

The differential privacy module is assessed on two real-world datasets, i.e., MNIST~\cite{xiao2017fashion} and CIFAR-10~\cite{krizhevsky2009learning} datasets, with model choices of Fully-connected and ResNet-18 respectively. 
\todo{Training data assignment to clients follows established protocols~\cite{yang2023privatefl}. 
Default parameter settings are detailed in Table xxx, adhered to unless stated otherwise.}



% All experiments are performed on a \todo{x86\_64 Linux machine with AMD Ryzen Threadripper PRO 5965WX 24-Cores and 256 GB RAM}. 
% We evaluated the two components of \sys separately.
% Generally, our evaluation adopts two metrics: the used time of the secure aggregation module and the accuracy of the training procedure with the differential privacy module.

% For secure aggregation, we consider a range of 200 to 1000 users, three assisting nodes, and one aggregation server. 
% We measure \todo{the computation time and the outbound bandwidth cost} of the server, the users, and the assisting nodes in both the Setup and Aggregation phases.
% To demonstrate the performance of \sys with high-dimensional gradient vectors, we report the performance when the weight vector $w$ consists of 100,000 gradients. 
% % In fact, compared to the existing works (e.g., ~\cite{}), our protocol offers a much higher efficiency for weight vectors with high dimensions since it does not require any expensive operations (e.g., solving for the discrete logarithm) to compute the final model from local updates.
% We consider \flamingo~\cite{flamingo} and \micro~\cite{microfedml} as our counterparts to evaluate the performance of the secure aggregation module of \sys.
% % \flamingo reduces the number of interactions between clients and the server to achieve significant communication and computation efficiency.
% % Similarly, 
% To launch a similar environment setup, we use the same setup for \micro. We select a range of 200 to 1000 users, three decryptors, and one aggregation server as the setting of \flamingo.

% For the differential privacy module, we follow previous DP work~\cite{} and use two real-world datasets of different scales, i.e., MNIST and CIFAR-10.
% \begin{itemize}
% \item The MNIST dataset~\cite{} contains 60,000 28x28 grayscale hand-written digits images in 10 different classes. We use 50,000 for training and 10,000 for texting. We select the Fully-connected~\cite{} as our training model.
% \item The CIFAR-10 dataset~\cite{} contains 60,000 32x32 color images in 1- different classes. We use 50,000 for training and 10,000 for testing. We select the ResNet-18~\cite{} as our training model. 
% \end{itemize}
% We follow the existing work~\cite{} to assign training data to clients. Table xxx shows the default parameter settings, which we adopt in experiments unless otherwise mentioned.

% https://www.usenix.org/system/files/usenixsecurity23-yang-yuchen.pdf
% https://arxiv.org/pdf/2304.03841


\section{Evaluation 0821}


\reza {We systematically evaluate our proposed \sys in two dimensions: efficiency  and performance. Our efficiency evaluation experiments include empirical time complexity of Setup phase and Aggregation phase and their corresponding bandwidths, respectively. Our performance evaluation assesses \sys's accuracy on two widely-used machine learning benchmark, MNIST and CIFAR10.}\\
\yiwei{Can this be moved to previous subsection?}

\reza{Dear Yiwei, please consider removing "RQ1" and "RQ2" and have each section as a numbered section instead.}\\
\yiwei{Done.}

\reza {We need to include Figures 3, 4, 5, and 6 in their corresponding numbered subsection provided in the paragraph above.}\\

\reza{Yiwei, once these structural changes are done, I can do another pass and revise the writing. Thanks!}

\begin{itemize}

\item \textbf{Section~\ref{sec:eval:eff} (Efficiency Measurement)}: What is the efficiency of post-quantum enhanced secure aggregation in FL? How does the efficiency of \sys improve by the introduction of pre-computation?
% \item \textbf{RQ2}: How does \sys improve it by introducing pre-computation method?
% \item \textbf{RQ2}: How does differential number of clients affect the performance of \sys?
\item \textbf{Section~\ref{sec:eval:perf} (Performance Measurement)}: How does the differential privacy module in \sys perform under different threat models? What is the performance of the DP-enhanced method in FL across different training datasets?
% \item \textbf{RQ3}: What is the performance of the DP-enhanced method in FL across different training datasets?
\end{itemize}

\subsection{Post-quantum Enhanced SA+FL Efficiency}


\subsubsection{Computation}~\label{sec:eval:eff}
We compare the computation cost of \sys in the Setup phase and Aggregation phase with the three other approaches, i.e., \flamingo, \pqsa, and \micro.
The results are listed in Table~\ref{table:sa_time}.

\input{tables/sa_time}


\begin{figure*}[htbp]
    \centering
    \begin{minipage}{0.32\textwidth}
        \centering
        \includegraphics[width=\textwidth]{figures/sa_setup_time/sa_time_setup_server.pdf}
        \caption*{(a) Server}
    \end{minipage}
    \hfill
    \begin{minipage}{0.32\textwidth}
        \centering
        \includegraphics[width=\textwidth]{figures/sa_setup_time/sa_time_setup_client.pdf}
        \caption*{(b) User}
    \end{minipage}
    \hfill
    \begin{minipage}{0.32\textwidth}
        \centering
        \includegraphics[width=\textwidth]{figures/sa_setup_time/sa_time_setup_node.pdf}
        \caption*{(c) Assisting node}
    \end{minipage}
    \caption{Computation in the Setup phase (The dimension of the weight list is set to 16K.)}
    \label{fig:sa_setup_time}
\end{figure*}



\noindent
\textbf{Setup Phase.}
\todo{replace "computational time" with "computation time"}
Figure~\ref{fig:sa_setup_time} shows the computation cost of our protocol in the Setup phase, compared to \flamingo and \micro.
\pqsa is excluded from this comparison as it only distributes several public parameters without performing significant computations.
% \elisa{can you please check again Figure 3 again? It seems that Beskar has the highest computation time. Perhaps I miss something. Also in the figure I would replace "computational time" with "computation time", also because in the text below you use "computation time"; make sure that the same term is used everywhere.}
Our results indicate that \sys has a higher computation time than \flamingo and \micro at all the entities.
% Our results indicate that \sys generally outperforms \flamingo and \micro in terms of the computation cost in the Setup phase. Specifically, \sys exhibits significantly lower computation time on the server and assisting node sides although it shows a slightly higher computation time than \microsecond on the client side.
The reason is that \sys implements an additional precomputation step in the setup phase, where several digital signature parameters are pre-computed for further runtime signing.

% \begin{itemize}
% \item Server and Assisting Node: \sys takes less time than \flamingo and \micro during the Setup phase. 
% The reason is that during the setup phase, the server and assisting nodes of \sys only need to generate their key pair and send their public key to the clients. 
% In contrast, 
% % Except generating and sending the public key, 
% the server and decryptors of \flamingo have to perform a distributed key generation (DKG) protocol to generate and distribute secret key shares for the asymmetric encryption scheme among the decryptors, without revealing the key to any single entity. 
% For \micro, the server must receive the client encryption keys, verify the signatures, manage client mask sharing, and ensure an adequate number of online clients.
%  % if the online users are enough.
% \elisa{In figure 3, I would change "User" with "Client" as in the text here we use "client".}
% \item Client: \sys takes less time than \flamingo and \microfirst but more time than \microsecond. The reason is that the clients of \sys perform key generation and key exchange to generate shared secret with each assisting node, and then send the public key to the server.
% The clients involved in \flamingo have to receive public keys from decryptors and verify their signatures.
% The client computation time for both \sys and \flamingo is proportional to the number of assisting nodes/decryptors but constant to the number of users. 
% For \microfirst, clients have to perform mask sharing with other clients, which is more computationally intensive than the secret sharing between users and assisting nodes in \sys.
% % the computation of which is larger than secret sharing between the users and assisting nodes in \sys.
% For \microsecond, clients only distribute shares among other users within the same group.
% \end{itemize}



\begin{figure*}[htbp]
    \centering
    \begin{minipage}{0.32\textwidth}
        \centering
        \includegraphics[width=\textwidth]{figures/sa_agg_time/sa_time_agg_server.pdf}
        \caption*{(a) Server}
    \end{minipage}
    \hfill
    \begin{minipage}{0.32\textwidth}
        \centering
        \includegraphics[width=\textwidth]{figures/sa_agg_time/sa_time_agg_client.pdf}
        \caption*{(b) User}
    \end{minipage}
    \hfill
    \begin{minipage}{0.32\textwidth}
        \centering
        \includegraphics[width=\textwidth]{figures/sa_agg_time/sa_time_agg_node.pdf}
        \caption*{(c) Assisting node}
    \end{minipage}
    \caption{Computation Times of the Aggregation phase (The dimension of the weight list is set to 16K.)}
    \label{fig:sa_agg_time}
\end{figure*}



\noindent
\textbf{Aggregation Phase.}
Figure~\ref{fig:sa_agg_time} shows the computation time of \sys in the aggregation phase compared with that in \flamingo, \pqsa, and \micro.
The results demonstrate that all entities in \sys incur a minimal computational overhead, with all the computation times significantly lower than those of \flamingo, \pqsa, and \micro regarding users, assisting nodes, and the server.

\begin{itemize}
\item \micro incurs the highest cost because each client has to calculate $H(k)^{X_i}$ and $H(k)^{R_i}$ and the server must recover the vector by calculating the discrete logarithm of $H(k)^{X_i} - H(k)^{R_i}$. This discrete logarithm calculation is computationally very intensive, especially as the vector dimensions increase.
\item \flamingo takes more time than \sys because it involves removing the masks for those dropout clients. Consequently, the clients and decryptors have to provide additional materials (e.g., secret shares) for the server to recover the local vector. 
\sys, however, employs a straightforward strategy that simply removes and ignores the masked vectors of dropout clients.
% \elisa{The wording "message utilization" is not very good. Do you mean that "it requires a smaller number of messages"?}
% While \sys may reduce message utilization, it eliminates unnecessary calculations, significantly reducing time overhead.
Thus it requires a smaller number of messages, eliminating unnecessary calculations and significantly reducing time overhead.
\end{itemize}

% The results show that \sys generally has a better performance than \flamingo and \micro in terms of the computation cost in Setup phase, as the computation time of \sys on server and assisting node sides is greatly lower than that of \flamingo and \micro though the computation time of \sys is slightly higher than \micro on the client side.
% \todo{This is because \micro does not generate a signature for its masked input.
% Although it generates a signature for the online set, but the signing algorithm is simple without taking too much time but achieving low security.}




\subsubsection{Outbound bandwidth}
We discuss the outbound bandwidth cost of \sys in the Setup phase and Aggregation phase separately. The results are reported in Table~\ref{table:sa_size}.

\input{tables/sa_size}


\begin{figure*}[htbp]
    \centering
    \begin{minipage}{0.4\textwidth}
        \centering
        \includegraphics[width=\textwidth]{figures/sa_setup_size/sa_size_setup_server.pdf}
        \caption*{(a) Server}
    \end{minipage}
    % \hfill
    \begin{minipage}{0.4\textwidth}
        \centering
        \includegraphics[width=\textwidth]{figures/sa_setup_size/sa_size_setup_client.pdf}
        \caption*{(b) User}
    \end{minipage}
    % \hfill
    % \begin{minipage}{0.32\textwidth}
    %     \centering
    %     \includegraphics[width=\textwidth]{figures/sa_setup_size/sa_size_setup_node.pdf}
    %     \caption*{(c) Assisting node}
    % \end{minipage}
    \caption{Bandwidth in the Setup Phase (The dimension of the weight list is set to 16K.)}
    \label{fig:sa_setup_bw}
\end{figure*}


\noindent
\textbf{Setup Phase.}
We present the outbound bandwidth cost of all entities in \sys during the Setup phase in Figure~\ref{fig:sa_setup_bw}. 
The outbound bandwidth cost of \sys is less than that of \micro and \flamingo on both client and server side.

\begin{itemize}
\item Server: The server in \sys broadcasts its public key to clients, thus its bandwidth depends on the public key size. The server in \flamingo participates in the DKG protocols, where the bandwidth depends
%\elisa{do you mean depends on "the number of messages" or on the "size of the messages" or on both?} \yiwei{both}
on the number and size of
the messages of DKG protocols and is proportional to the number of decryptors, but constant relative to the number of clients. 
In \micro, the server forwards all the communications, i.e., the public keys and secret shares, from one client to the others, making its bandwidth proportional to the number of clients.
% all the communications such as the distribution of the DH keys and encrypted shares need to be communicated via the aggregation server, which incurs a significant communication overhead.
\item Client: In \sys, each client should send its public key and the encrypted secret to each assisting node, thus its bandwidth is constant relative to the number of clients. In \micro, each client should send its public key and (N-1) mask shares to all the other clients, making its bandwidth proportional to the number of clients, thus higher than that of \sys. \flamingo is excluded here as its clients do not send any messages during this phase.
\item Assisting Node: During the setup phase, each assisting node in \sys sends its public key to each client, thus its bandwidth is proportional to the number of clients. 
In \flamingo, the decryptors involved in DKG protocols have a bandwidth dependent on DKG messages and proportional to the number of decryptors but constant relative to the number of clients.
\end{itemize}


\begin{figure*}[htbp]
    \centering
    \begin{minipage}{0.32\textwidth}
        \centering
        \includegraphics[width=\textwidth]{figures/sa_agg_size/sa_size_agg_server.pdf}
        \caption*{(a) Server}
    \end{minipage}
    \hfill
    \begin{minipage}{0.32\textwidth}
        \centering
        \includegraphics[width=\textwidth]{figures/sa_agg_size/sa_size_agg_client.pdf}
        \caption*{(b) User}
    \end{minipage}
    \hfill
    \begin{minipage}{0.32\textwidth}
        \centering
        \includegraphics[width=\textwidth]{figures/sa_agg_size/sa_size_agg_node.pdf}
        \caption*{(c) Assisting node}
    \end{minipage}
    \caption{Bandwidth in the Aggregation phase (The dimension of the weight list is set to 16K.)}
    \label{fig:sa_agg_bw}
\end{figure*}


\noindent
\textbf{Aggregation Phase.}
We present the outbound bandwidth cost of all entities in \sys during the Aggregation phase in Figure~\ref{fig:sa_agg_bw}. 
The outbound bandwidth cost of \sys on all entities is less than that of \micro and \flamingo.

\begin{itemize}
\item Server: In \sys, the server only broadcasts the final update during the aggregation phase, thus its outbound bandwidth is the size of the final update and constant to the number of clients. Servers in \flamingo, \pqsa and \micro have to get involved in forwarding the client message to the decryptors or other clients to assist in recovering the masks of dropout clients and managing secret sharing among clients, thus their bandwidth is higher than that of \sys and roughly proportional to the number of clients. 
% The server of \micro has to report the online client set to each client and forwards the signature of each client to other clients, as well as distribute the final update, thus its bandwidth is more than \sys and \flamingo and proportional to the number of clients.
\item Client: Clients in \sys send masked updates and iteration numbers to the server and assisting nodes separately, with the bandwidth being dependent on the update vector size and proportional to the number of assisting nodes but constant relative to the number of clients.
In \flamingo, clients send masked updates to the server and secret shares to decryptors and neighbors, making their bandwidth proportional to the number of decryptors and clients (i.e., neighbors).
Clients in \micro send masked updates and masks of online clients to the server, resulting in bandwidth higher than \sys but lower than \flamingo. 
Clients in \pqsa have to additionally send the split secrets of each other client, except to the masked update, leading to the highest bandwidth proportional to the number of clients.
\item Assisting Node: Each assisting node in \sys should send the sum of masks of online clients to the server, thus its bandwidth is the size of the update and constant to the number of clients.
In \flamingo, decryptors send decrypted secret shares of each client to the server, resulting in higher bandwidth proportional to the number of clients compared to \sys.
\end{itemize}

% Each assisting node in \sys sends the sum of masks of online clients to the server, with bandwidth constant relative to the number of clients. In \flamingo, decryptors send decrypted secret shares (equivalent in size to the update) of each client to the server, resulting in higher bandwidth proportional to the number of clients compared to \sys.

% For 1000 users, the server transmits ~x-x orders of magnitude less than \flamingo and ~x-x orders of magnitude less than \micro.
% The server bandwidth in \sys protocol grows linearly as the number of users increases because xxx.
% In \flamingo, however, due to the design, xxxx
% In \micro, xxxx
% Thus, user bandwidth in \sys is xxx - xxx less than \flamingo and xxx - xxx less than \micro, respectively.
% The bandwidth cost of assisting nodes in \sys is negligible where each xxx.
% As the overhead is due to xxx, its bandwidth cost grows linearly xxx

% In Figure xxx, we compare the outbound bandwidth costs of the Aggregation phase for all the entities in our protocol with the one in \flamingo and the one in \micro.
% We have observed that the outbound bandwidth cost for the server and the user in our protocol is considerably lower than those in the \flamingo and \micro protocols.
% xxxx

% \begin{figure*}[htbp]
%     \centering
%     \begin{minipage}{0.32\textwidth}
%         \centering
%         \includegraphics[width=\textwidth]{figures/sa_setup_size/sa_size_setup_server.pdf}
%         \caption*{(a) Server}
%     \end{minipage}
%     \hfill
%     \begin{minipage}{0.32\textwidth}
%         \centering
%         \includegraphics[width=\textwidth]{figures/sa_setup_size/sa_size_setup_client.pdf}
%         \caption*{(b) User}
%     \end{minipage}
%     \hfill
%     \begin{minipage}{0.32\textwidth}
%         \centering
%         \includegraphics[width=\textwidth]{figures/sa_setup_size/sa_size_setup_node.pdf}
%         \caption*{(c) Assisting node}
%     \end{minipage}
%     \caption{Bandwidth in the Setup phase (The dimension of the weight list is set to 16K.)}
%     \label{fig:sa_setup_bw}
% \end{figure*}

% \begin{figure*}[htbp]
%     \centering
%     \begin{minipage}{0.32\textwidth}
%         \centering
%         \includegraphics[width=\textwidth]{figures/sa_agg_size/sa_size_agg_server.pdf}
%         \caption*{(a) Server}
%     \end{minipage}
%     \hfill
%     \begin{minipage}{0.32\textwidth}
%         \centering
%         \includegraphics[width=\textwidth]{figures/sa_agg_size/sa_size_agg_client.pdf}
%         \caption*{(b) User}
%     \end{minipage}
%     \hfill
%     \begin{minipage}{0.32\textwidth}
%         \centering
%         \includegraphics[width=\textwidth]{figures/sa_agg_size/sa_size_agg_node.pdf}
%         \caption*{(c) Assisting node}
%     \end{minipage}
%     \caption{Bandwidth in the Aggregation phase (The dimension of the weight list is set to 16K.)}
%     \label{fig:sa_agg_bw}
% \end{figure*}


\subsubsection{Precomputation Improvement}


\input{tables/precomputed}

To assess the impact of precomputation strategies on \sys, we conducted a comparative experiment implementing \sys without precomputation in the Dilithium signing algorithms and mask generation. The results, shown in Table~\ref{table:precomputed}, indicate that precomputation significantly enhances efficiency for both assisting nodes and clients as the number of clients increases.

Without precomputation, an assisting node must perform additional mask generation operations for N clients and one signing operation, while a client must perform additional mask generation for M assisting nodes and M+1 signing operations. Consequently, precomputation notably reduces the computational burden on these entities.

On the server side, the benefits of precomputation are less pronounced. The reason is that the server performs relatively fewer computational operations, limited to only one signing operation, compared to the assisting nodes and clients.


% To evaluate how precomputation strategies enhance \sys, e conducted a comparative experiment, in which we implemented \sys without precomputations, i.e., in Dilithium signing algorithms and mask generation.
% The results are listed in Table~\ref{table:precomputed}.
% We can see that precomputation could greatly improve the efficiency on assisting nodes and clients with the increasing number of clients.
% This is because without precomputation, one assisting node has to perform additional N mask generation for N clients and one signing operation, and one client has to perform additional M mask generation and M+1 signing operations. 
% Moreover, precomputations did not improve a lot on the server side, as the server perform much less computational operations (i.e., only one signing operation) than the assisting nodes and clients.

% \yiwei{Precomputation could greatly improve the efficiency on assisting nodes with the increasing number of clients.}


% \subsubsection{Number of Clients}
% We explore how different number of clients (ranging from 200 to 1000) affects the performance of secure aggregation in \sys.
% xxx and xxx show the computation time and outbound bandwidth of \sys when the number of clients varies.
% We observe that \sys consistently outperforms xxx and xxx in both time and bandwidth, especially when the system has more clients.
% For instance, the xxx gap between \sys and xxx increases from xxx\% with 200 clients to xxx\% with 1000 clients.




\subsection{DP+FL Performance}~\label{sec:eval:perf}


% \subsubsection{DP Performance with MNIST and CIFAR-10}

\input{tables/dp_acc}

We evaluated the accuracy of models trained on the MNIST and CIFAR-10 datasets using three differential privacy (DP) methods—ODP, CDP, LDP—and compared them to a Non-Differential Privacy (NDP) baseline. 
Table~\ref{tab:dp_acc} presents the best testing accuracy for federated learning (FL) models under these DP methods, with varying privacy budgets ($\epsilon$).

As expected, the NDP method, which does not introduce noise, achieved the highest accuracy. On average, the accuracy reductions for ODP, CDP, and LDP were approximately 5\%, 13\%, and 20\%, respectively. 
Notably, ODP demonstrated superior accuracy compared to CDP and LDP. This can be attributed to ODP's addition of noise only at the final iteration, unlike CDP and LDP, which introduce noise at every iteration. 
CDP generally outperformed LDP, particularly at larger $\epsilon$ values, consistent with findings in~\cite{yang2023privatefl}. This is because CDP adds noise to aggregated results, allowing the model to better capture global patterns despite the noise. In contrast, LDP's noise application to individual client data at each iteration diminishes the model's ability to leverage data correlations and global information effectively.
% \elisa{I think that the above results is consistent with previous work as it is well known that LDP results in much less accuracy as one has to add a lot of noise to the data. Could we perhaps mention some references here?}
% \yiwei{Done.}


% \reza {I think we need to only keep the first 8 rows of Table VII. The relationship between the noise and accuracy becomes questionable when we change many other parameters at the same time. Please consider removing all the rows other than the first 8 numbers to make the table simple and accurate. Please also adjust the description of the table to match this change. Also, column such as sample rate that are always 1 in our case, can be removed from the table and mentioned in the text.}
% \yiwei{Done.}

Additionally, we observed that accuracy improved with increasing $\epsilon$ across all DP methods. This trend is due to smaller $\epsilon$ values—corresponding to stronger privacy protection—introducing more noise, thus increasing data heterogeneity. CDP's accuracy gains with larger $\epsilon$ values were more pronounced than those of ODP and LDP. The noise addition during intermediate model aggregation in CDP allows for more effective training, whereas ODP's one-time noise or LDP's dispersed noise results in less impact on overall model performance.

In conclusion, while there is a trade-off between privacy and accuracy, our DP methods effectively maintain high accuracy levels, closely approximating that of the NDP baseline, while ensuring robust data privacy.


% % To evaluate the performance of our DP methods in FL, we conducted experiments using two benchmark datasets: MNIST and CIFAR-10. 
% % The goal was to assess the impact of different DP methods on the accuracy of the models while preserving privacy, under different threat models. 

% We assessed the accuracy of models trained using the MNIST and CIFAR-10 datasets across three differential privacy (DP) methods, i.e., ODP, CDP, LDP, and the Non-Differential Privacy (NDP) method as a baseline. Table~\ref{tab:dp_acc} presents the testing accuracy results (i.e., the best accuracy) for FL models under these DP methods, for varying privacy budget $\epsilon$.

% Generally, the NDP method, which does not add noise, achieves the highest accuracy. On average, ODP, CDP, and LDP methods result in accuracy reductions of approximately 5\%, 13\%, and 20\%, respectively. Notably, ODP exhibits superior accuracy compared to CDP and LDP. This is attributed to the fact that ODP only adds one-time noise at the final iteration, whereas CDP and LDP introduce noise at each iteration.
% % on the aggregated model, and LDP applies noise to individual client data transformations at every iteration.
% The reason why CDP generally achieves higher accuracy than LDP, particularly at larger $\epsilon$ values, is that CDP adds noise to the aggregated results, allowing the model to learn global patterns despite the presence of noise, whereas LDP applies noise to individual client data transformations, diminishing the model's ability to utilize data correlations and global information effectively.


% Furthermore, we observed that the accuracy improves with increasing $\epsilon$ across all three DP methods. This trend occurs because smaller $\epsilon$ values, which corresponds to stronger privacy protection, introduce more noise, increasing data heterogeneity. The accuracy improvement in CDP with larger $\epsilon$ values surpasses that of ODP and LDP, as CDP's noise addition during intermediate model aggregation allows for more effective training. In contrast, either the one-iteration noise in ODP or the dispersed impact of noise in LDP results in a smaller overall influence on the model. 

% % A higher $\epsilon$ value, which corresponds to weaker privacy protection, generally enhances the accuracy of both CDP and LDP, with improvements up to 1.09 and 1.03 times, respectively. This occurs because less noise is required for privacy preservation, leading to less distortion in the aggregated results and better model performance.


% In summary, although applying differential privacy does introduce a trade-off between privacy and accuracy, our DP methods effectively maintain a high level of accuracy, closely approximating that of the NDP baseline, while still ensuring data privacy.




% \begin{tcolorbox}[colback=gray!10,colframe=black,boxrule=1pt]
% \textbf{Takeaway:} Although applying differential privacy does introduce a trade-off between privacy and accuracy, our DP methods effectively maintained a high level of accuracy, closely approximating that of the NDP baseline, while still ensuring data privacy.
% \end{tcolorbox}

% Consequently, CDP generally achieves higher accuracy than LDP, particularly at larger $\epsilon$ values, as CDP allows the model to learn global patterns despite the presence of noise, whereas LDP's per-data-point noise diminishes the model's ability to utilize data correlations and global information effectively.



% \begin{figure}[!ht]
%   \centering
%   \includegraphics[width=1\linewidth]{figures/dp_acc.pdf}
%   \caption{The Accuracy of Different Privacy Module (MNIST)}
%   \label{fig:dp_acc}
% \end{figure}

% \subsection{RQ3: DP+FL Performance under different parameters}

% \subsubsection{DP Performance with different DP guarantees}
% \input{tables/dp_params}

% % overlap, one data in one client but not in another client


% To understand the trade-offs in our DP methods, we examined the effects of varying parameters. Our investigation, based on previous findings~\cite{opacus}, focused on how these parameters impact the accuracy of FL models. The four key parameters considered were 
% % the number of clients and
% three noise parameters, i.e., the privacy budget $\epsilon$, the number of training iterations, and the sample rate of clients. 
% The results are listed in Table~\ref{tab:dp_param}.


% % \noindent
% % \textbf{Number of Clients.}
% % % With the increasing number of clients, the accuracy of CDP is increasing, up to x1.43, as having more data from more clients or training with more iterations can help in better generalization, improving the model's performance, while keeping the same noise.
% % % But LDP, the more clients there are, the worse the accuracy is.
% % % This could be due to the fact that adding more noise at the local level for a larger number of clients aggregates to a higher total noise, degrading the overall model accuracy.
% % Increasing the number of clients generally improves the accuracy of CDP, with a reported increase of up to 1.43 times. 
% % This improvement is likely due to the greater data diversity and better generalization achieved with more clients, even when noise levels remain constant. In contrast, LDP shows a decrease in accuracy with more clients. This reduction is attributed to the cumulative effect of adding more noise at the local level, which deteriorates the overall model accuracy.


% \noindent
% \textbf{$\epsilon$.}
% % As $\epsilon$ increases, the accuracy of CDP and LDP generally improves, up to x1.09 and x1.03.
% % This is because a higher $\epsilon$, which corresponds to weaker privacy guarantees, allows for less added noise to reduce the distortion in the aggregated results, thus improving model performance.
% A higher $\epsilon$ value, which corresponds to weaker privacy protection, generally enhances the accuracy of both CDP and LDP, with improvements up to 1.09 and 1.03 times, respectively. This occurs because less noise is required for privacy preservation, leading to less distortion in the aggregated results and better model performance.


% \noindent
% \textbf{Number of Iterations.}
% % With the increasing number of iterations, the accuracy of CDP and LDP is increasing, even though the added noise is becoming larger.
% % This may result from the basic principle of FL training, that is, the more clients are involved and the more iterations are conducted, the better performance will be achieved.
% The accuracy of both CDP and LDP models improves with more training iterations, despite an increase in added noise. Because longer training with more iterations of computation, generally leads to better performance, as models have more opportunity to converge~\cite{yang2019federated}.
% % This result can be explained by the common observations of FL: more iterations and greater client involvement generally lead to better model performance.

% \noindent
% \textbf{Sample Rate.}
% An increase in sample rate leads to a slight improvement in the accuracy of both CDP and LDP. The sample rate impacts both the number of clients involved in the training and the amount of noise added for privacy. A larger sample rate allows for more client data to be used, which generally enhances model accuracy. However, it also necessitates more noise addition to preserve privacy, which can negatively impact accuracy. As a result, the opposing effects of increased data and added noise tend to balance each other out, leading to a marginal net gain in accuracy.

% \vspace{5pt}
% To achieve the best performance, a careful balance between model accuracy and noise levels for privacy protection is essential. The noise parameters should be optimized to meet specific privacy requirements while minimizing the impact on model performance.













% Our results show that the accuracy of CDP and LDP is slightly increasing when the sample rate is becoming larger, due to its double side impact.
% The sample rate of clients, on the one hand, affects the number of involved clients, and a larger sample rate will lead to better accuracy as more client data is used for training.
% On the other hand, it can also decide the added noise for privacy protection.
% With the increase of the sample rate, its two impacts are offset.


% \begin{tcolorbox}[colback=gray!10,colframe=black,boxrule=1pt]
% \textbf{Takeaway:} 
% % While higher noise levels provide stronger privacy guarantees, they also reduce model accuracy. 
% A careful balance between model accuracy and noise levels for privacy protection is essential. The noise parameters should be optimized to meet specific privacy requirements while minimizing the impact on model performance.
% \end{tcolorbox}

% In summary, our results indicate that while higher noise levels provide stronger privacy guarantees, they also reduce model accuracy. This necessitates a careful balance, where the noise parameters are optimized to provide adequate privacy without unduly compromising the model's performance. The choice of noise parameters can also be influenced by the sensitivity of the training data and the specific privacy requirements of the application.

% Moreover, the accuracy improves with the increasing number of iterations and client sample rate, even though the added noise is becoming larger.
% This may result from the basic principle of FL training, that is, the more clients are involved and the more iterations are conducted, the better performance will be achieved.
% In addition, with the increasing number of clients and same noise, the best accuracy is increasing, up to x1.43, as having more data from more clients or training with more iterations can help in better generalization, improving the model's performance.


% Things are similar for $\epsilon$, the number of iterations and the sample rate in LDP settings, as the more $\epsilon$ and the less iterations and sample rate are, the less noise will be added to the model training to protect privacy.
% But for the number of clients, the more clients there are, the worse the accuracy is.
% This could be due to the fact that adding more noise at the local level for a larger number of clients aggregates to a higher total noise, degrading the overall model accuracy.
% the more noise will be added in total, as LDP adopts DP (i.e., adding noise) at each client side.





% This a higher ε, which corresponds to weaker privacy guarantees, allows for better accuracy. The noise added to the data decreases with increasing ε (from 9.04 to 5.21), reducing the distortion in the aggregated results and thus improving model performance.
% LDP: Accuracy remains relatively flat at 0.68 regardless of ε. This suggests that LDP might be more resistant to changes in ε in terms of performance, potentially due to more noise being added at the local level, which might not reduce as significantly with increasing ε.

% Our analysis revealed that increasing the noise parameter generally leads to a decrease in accuracy, as the injected noise becomes more significant relative to the signal in the data. However, different DP methods responded differently to changes in noise levels. For instance, LDP, which applies noise at the local client level, showed a more pronounced decrease in accuracy compared to CDP, which aggregates the noise at the central server.

% The results indicate that while higher noise levels provide stronger privacy guarantees, they also reduce model accuracy. This necessitates a careful balance, where the noise parameters are optimized to provide adequate privacy without unduly compromising the model's performance. The choice of noise parameters can also be influenced by the sensitivity of the training data and the specific privacy requirements of the application.

% \yiwei{The performance of DP mainly depends on three parameters: epsilon, the number of iterations, and sample rate.
% The larger epsilon is, the less noise is added, the higher accuracy is.
% The less iterations are, the less noise is added, the higher accuracy is.
% The less sample rate is, the less noise is added, the higher accuracy is.}


% MNIST and CiFAR-10



\section{Evaluation 0822}

In this section, we present the experimental results evaluating the efficiency and performance of \sys. Our findings address the following key research questions:

% \reza {We systematically evaluate our proposed \sys in two dimensions: efficiency  and performance. Our efficiency evaluation experiments include empirical time complexity of Setup phase and Aggregation phase and their corresponding bandwidths, respectively. Our performance evaluation assesses \sys's accuracy on two widely-used machine learning benchmark, MNIST and CIFAR10.}\\
% \yiwei{Can this be moved to previous subsection?}

% \reza{Dear Yiwei, please consider removing "RQ1" and "RQ2" and have each section as a numbered section instead.}\\
% \yiwei{Done.}

% \reza {We need to include Figures 3, 4, 5, and 6 in their corresponding numbered subsection provided in the paragraph above.}\\

% \reza{Yiwei, once these structural changes are done, I can do another pass and revise the writing. Thanks!}

\begin{itemize}

\item \textbf{Section~\ref{sec:eval:eff} (Efficiency Measurement)}: How efficient is post-quantum enhanced secure aggregation in FL? What gains in efficiency does \sys achieve through the use of pre-computation?
% How does the efficiency of \sys improve by the introduction of pre-computation?
\item \textbf{Section~\ref{sec:eval:perf} (Performance Measurement)}: How does \sys’s differential privacy module perform under different threat models? What is the impact of DP-enhanced methods on FL performance across different training datasets?
% How does the differential privacy module in \sys perform under different threat models? What is the performance of the DP-enhanced method in FL across different training datasets?
\end{itemize}

\subsection{Post-quantum Enhanced SA+FL Efficiency}~\label{sec:eval:eff}


\subsubsection{Computation}
We compare the computational cost of \sys in the Setup phase and Aggregation phase with the four other approaches, i.e., \flamingo, \pqsa, \eseafl, and \micro.
% The results are listed in Table~\ref{table:sa_time}.

% \input{tables/sa_time}


\begin{figure*}[htbp]
    \centering
    \begin{minipage}{0.32\textwidth}
        \centering
        \includegraphics[width=\textwidth]{figures/sa_setup_time/sa_time_setup_server.pdf}
        \caption*{(a) Server}
    \end{minipage}
    \hfill
    \begin{minipage}{0.32\textwidth}
        \centering
        \includegraphics[width=\textwidth]{figures/sa_setup_time/sa_time_setup_client.pdf}
        \caption*{(b) Client}
    \end{minipage}
    \hfill
    \begin{minipage}{0.32\textwidth}
        \centering
        \includegraphics[width=\textwidth]{figures/sa_setup_time/sa_time_setup_node.pdf}
        \caption*{(c) Assisting node}
    \end{minipage}
    \caption{Computation Time of the Setup phase (The dimension of the weight list is set to 16K.)}
    \label{fig:sa_setup_time}
\end{figure*}



\noindent
\textbf{Setup Phase.}
Figure~\ref{fig:sa_setup_time} shows the computation cost of each works in the Setup phase.
\pqsa is excluded from this comparison as it only distributes several public parameters without performing significant computations.
Our results indicate that \sys has a higher computation time than \flamingo and \micro at all the entities.
% Our results indicate that \sys generally outperforms \flamingo and \micro in terms of the computation cost in the Setup phase. Specifically, \sys exhibits significantly lower computation time on the server and assisting node sides although it shows a slightly higher computation time than \microsecond on the client side.
The reason is that \sys implements an additional precomputation step in the setup phase, where several digital signature parameters are pre-computed for further runtime signing.

% \begin{itemize}
% \item Server and Assisting Node: \sys takes less time than \flamingo and \micro during the Setup phase. 
% The reason is that during the setup phase, the server and assisting nodes of \sys only need to generate their key pair and send their public key to the clients. 
% In contrast, 
% % Except generating and sending the public key, 
% the server and decryptors of \flamingo have to perform a distributed key generation (DKG) protocol to generate and distribute secret key shares for the asymmetric encryption scheme among the decryptors, without revealing the key to any single entity. 
% For \micro, the server must receive the client encryption keys, verify the signatures, manage client mask sharing, and ensure an adequate number of online clients.
%  % if the online users are enough.
% \elisa{In figure 3, I would change "User" with "Client" as in the text here we use "client".}
% \item Client: \sys takes less time than \flamingo and \microfirst but more time than \microsecond. The reason is that the clients of \sys perform key generation and key exchange to generate shared secret with each assisting node, and then send the public key to the server.
% The clients involved in \flamingo have to receive public keys from decryptors and verify their signatures.
% The client computation time for both \sys and \flamingo is proportional to the number of assisting nodes/decryptors but constant to the number of users. 
% For \microfirst, clients have to perform mask sharing with other clients, which is more computationally intensive than the secret sharing between users and assisting nodes in \sys.
% % the computation of which is larger than secret sharing between the users and assisting nodes in \sys.
% For \microsecond, clients only distribute shares among other users within the same group.
% \end{itemize}



\begin{figure*}[htbp]
    \centering
    \begin{minipage}{0.32\textwidth}
        \centering
        \includegraphics[width=\textwidth]{figures/sa_agg_time/sa_time_agg_server.pdf}
        \caption*{(a) Server}
    \end{minipage}
    \hfill
    \begin{minipage}{0.32\textwidth}
        \centering
        \includegraphics[width=\textwidth]{figures/sa_agg_time/sa_time_agg_client.pdf}
        \caption*{(b) User}
    \end{minipage}
    \hfill
    \begin{minipage}{0.32\textwidth}
        \centering
        \includegraphics[width=\textwidth]{figures/sa_agg_time/sa_time_agg_node.pdf}
        \caption*{(c) Assisting node}
    \end{minipage}
    \caption{Computation Time of the Aggregation phase (The dimension of the weight list is set to 16K.)}
    \label{fig:sa_agg_time}
\end{figure*}



\noindent
\textbf{Aggregation Phase.}
Figure~\ref{fig:sa_agg_time} shows the computation time of \sys in the aggregation phase compared with that in \flamingo, \pqsa, and \micro.
The results demonstrate that all entities in \sys incur a minimal computational overhead, with all the computation times significantly lower than those of \flamingo, \pqsa, and \micro regarding users, assisting nodes, and the server.

\begin{itemize}
\item \micro incurs the highest cost because each client has to calculate $H(k)^{X_i}$ and $H(k)^{R_i}$ and the server must recover the vector by calculating the discrete logarithm of $H(k)^{X_i} - H(k)^{R_i}$. This discrete logarithm calculation is computationally very intensive, especially as the vector dimensions increase.
\item \flamingo takes more time than \sys because it involves removing the masks for those dropout clients. Consequently, the clients and decryptors have to provide additional materials (e.g., secret shares) for the server to recover the local vector. 
\sys, however, employs a straightforward strategy that simply removes and ignores the masked vectors of dropout clients.
% \elisa{The wording "message utilization" is not very good. Do you mean that "it requires a smaller number of messages"?}
% While \sys may reduce message utilization, it eliminates unnecessary calculations, significantly reducing time overhead.
Thus it requires a smaller number of messages, eliminating unnecessary calculations and significantly reducing time overhead.
\end{itemize}

% The results show that \sys generally has a better performance than \flamingo and \micro in terms of the computation cost in Setup phase, as the computation time of \sys on server and assisting node sides is greatly lower than that of \flamingo and \micro though the computation time of \sys is slightly higher than \micro on the client side.
% \todo{This is because \micro does not generate a signature for its masked input.
% Although it generates a signature for the online set, but the signing algorithm is simple without taking too much time but achieving low security.}




\subsubsection{Outbound bandwidth}
We discuss the outbound bandwidth cost of \sys in the Setup phase and Aggregation phase separately. The results are reported in Table~\ref{table:sa_size}.

% \input{tables/sa_size}


\begin{figure*}[htbp]
    \centering
    \begin{minipage}{0.32\textwidth}
        \centering
        \includegraphics[width=\textwidth]{figures/sa_setup_size/sa_size_setup_server.pdf}
        \caption*{(a) Server}
    \end{minipage}
    \hfill
    \begin{minipage}{0.32\textwidth}
        \centering
        \includegraphics[width=\textwidth]{figures/sa_setup_size/sa_size_setup_client.pdf}
        \caption*{(b) Client}
    \end{minipage}
    \hfill
    \begin{minipage}{0.32\textwidth}
        \centering
        \includegraphics[width=\textwidth]{figures/sa_setup_size/sa_size_setup_node.pdf}
        \caption*{(c) Assisting node}
    \end{minipage}
    \caption{Bandwidth in the Setup Phase (The dimension of the weight list is set to 16K.)}
    \label{fig:sa_setup_bw}
\end{figure*}


\noindent
\textbf{Setup Phase.}
We present the outbound bandwidth cost of all entities in \sys during the Setup phase in Figure~\ref{fig:sa_setup_bw}. 
The outbound bandwidth cost of \sys is less than that of \micro and \flamingo on both client and server side.

\begin{itemize}
\item Server: The server in \sys broadcasts its public key to clients, thus its bandwidth depends on the public key size. The server in \flamingo participates in the DKG protocols, where the bandwidth depends
%\elisa{do you mean depends on "the number of messages" or on the "size of the messages" or on both?} \yiwei{both}
on the number and size of
the messages of DKG protocols and is proportional to the number of decryptors, but constant relative to the number of clients. 
In \micro, the server forwards all the communications, i.e., the public keys and secret shares, from one client to the others, making its bandwidth proportional to the number of clients.
% all the communications such as the distribution of the DH keys and encrypted shares need to be communicated via the aggregation server, which incurs a significant communication overhead.
\item Client: In \sys, each client should send its public key and the encrypted secret to each assisting node, thus its bandwidth is constant relative to the number of clients. In \micro, each client should send its public key and (N-1) mask shares to all the other clients, making its bandwidth proportional to the number of clients, thus higher than that of \sys. \flamingo is excluded here as its clients do not send any messages during this phase.
\item Assisting Node: During the setup phase, each assisting node in \sys sends its public key to each client, thus its bandwidth is proportional to the number of clients. 
In \flamingo, the decryptors involved in DKG protocols have a bandwidth dependent on DKG messages and proportional to the number of decryptors but constant relative to the number of clients.
\end{itemize}


\begin{figure*}[htbp]
    \centering
    \begin{minipage}{0.32\textwidth}
        \centering
        \includegraphics[width=\textwidth]{figures/sa_agg_size/sa_size_agg_server.pdf}
        \caption*{(a) Server}
    \end{minipage}
    \hfill
    \begin{minipage}{0.32\textwidth}
        \centering
        \includegraphics[width=\textwidth]{figures/sa_agg_size/sa_size_agg_client.pdf}
        \caption*{(b) User}
    \end{minipage}
    \hfill
    \begin{minipage}{0.32\textwidth}
        \centering
        \includegraphics[width=\textwidth]{figures/sa_agg_size/sa_size_agg_node.pdf}
        \caption*{(c) Assisting node}
    \end{minipage}
    \caption{Bandwidth in the Aggregation phase (The dimension of the weight list is set to 16K.)}
    \label{fig:sa_agg_bw}
\end{figure*}


\noindent
\textbf{Aggregation Phase.}
We present the outbound bandwidth cost of all entities in \sys during the Aggregation phase in Figure~\ref{fig:sa_agg_bw}. 
The outbound bandwidth cost of \sys on all entities is less than that of \micro and \flamingo.

\begin{itemize}
\item Server: In \sys, the server only broadcasts the final update during the aggregation phase, thus its outbound bandwidth is the size of the final update and constant to the number of clients. Servers in \flamingo, \pqsa and \micro have to get involved in forwarding the client message to the decryptors or other clients to assist in recovering the masks of dropout clients and managing secret sharing among clients, thus their bandwidth is higher than that of \sys and roughly proportional to the number of clients. 
% The server of \micro has to report the online client set to each client and forwards the signature of each client to other clients, as well as distribute the final update, thus its bandwidth is more than \sys and \flamingo and proportional to the number of clients.
\item Client: Clients in \sys send masked updates and iteration numbers to the server and assisting nodes separately, with the bandwidth being dependent on the update vector size and proportional to the number of assisting nodes but constant relative to the number of clients.
In \flamingo, clients send masked updates to the server and secret shares to decryptors and neighbors, making their bandwidth proportional to the number of decryptors and clients (i.e., neighbors).
Clients in \micro send masked updates and masks of online clients to the server, resulting in bandwidth higher than \sys but lower than \flamingo. 
Clients in \pqsa have to additionally send the split secrets of each other client, except to the masked update, leading to the highest bandwidth proportional to the number of clients.
\item Assisting Node: Each assisting node in \sys should send the sum of masks of online clients to the server, thus its bandwidth is the size of the update and constant to the number of clients.
In \flamingo, decryptors send decrypted secret shares of each client to the server, resulting in higher bandwidth proportional to the number of clients compared to \sys.
\end{itemize}



\subsubsection{Precomputation Improvement}


\input{tables/precomputed}

To assess the impact of precomputation strategies on \sys, we conducted a comparative experiment implementing \sys without precomputation in the Dilithium signing algorithms and mask generation. The results, shown in Table~\ref{table:precomputed}, indicate that precomputation significantly enhances efficiency for both assisting nodes and clients as the number of clients increases.

Without precomputation, an assisting node must perform additional mask generation operations for N clients and one signing operation, while a client must perform additional mask generation for M assisting nodes and M+1 signing operations. Consequently, precomputation notably reduces the computational burden on these entities.

On the server side, the benefits of precomputation are less pronounced. The reason is that the server performs relatively fewer computational operations, limited to only one signing operation, compared to the assisting nodes and clients.


% To evaluate how precomputation strategies enhance \sys, e conducted a comparative experiment, in which we implemented \sys without precomputations, i.e., in Dilithium signing algorithms and mask generation.
% The results are listed in Table~\ref{table:precomputed}.
% We can see that precomputation could greatly improve the efficiency on assisting nodes and clients with the increasing number of clients.
% This is because without precomputation, one assisting node has to perform additional N mask generation for N clients and one signing operation, and one client has to perform additional M mask generation and M+1 signing operations. 
% Moreover, precomputations did not improve a lot on the server side, as the server perform much less computational operations (i.e., only one signing operation) than the assisting nodes and clients.

% \yiwei{Precomputation could greatly improve the efficiency on assisting nodes with the increasing number of clients.}


% \subsubsection{Number of Clients}
% We explore how different number of clients (ranging from 200 to 1000) affects the performance of secure aggregation in \sys.
% xxx and xxx show the computation time and outbound bandwidth of \sys when the number of clients varies.
% We observe that \sys consistently outperforms xxx and xxx in both time and bandwidth, especially when the system has more clients.
% For instance, the xxx gap between \sys and xxx increases from xxx\% with 200 clients to xxx\% with 1000 clients.




\subsection{DP+FL Performance}~\label{sec:eval:perf}


% \subsubsection{DP Performance with MNIST and CIFAR-10}

\input{tables/dp_acc}

We evaluated the accuracy of models trained on the MNIST and CIFAR-10 datasets using three differential privacy (DP) methods—ODP, CDP, LDP—and compared them to a Non-Differential Privacy (NDP) baseline. 
Table~\ref{tab:dp_acc} presents the best testing accuracy for federated learning (FL) models under these DP methods, with varying privacy budgets ($\epsilon$).

As expected, the NDP method, which does not introduce noise, achieved the highest accuracy. On average, the accuracy reductions for ODP, CDP, and LDP were approximately 5\%, 13\%, and 20\%, respectively. 
Notably, ODP demonstrated superior accuracy compared to CDP and LDP. This can be attributed to ODP's addition of noise only at the final iteration, unlike CDP and LDP, which introduce noise at every iteration. 
CDP generally outperformed LDP, particularly at larger $\epsilon$ values, consistent with findings in~\cite{yang2023privatefl}. This is because CDP adds noise to aggregated results, allowing the model to better capture global patterns despite the noise. In contrast, LDP's noise application to individual client data at each iteration diminishes the model's ability to leverage data correlations and global information effectively.
% \elisa{I think that the above results is consistent with previous work as it is well known that LDP results in much less accuracy as one has to add a lot of noise to the data. Could we perhaps mention some references here?}
% \yiwei{Done.}


% \reza {I think we need to only keep the first 8 rows of Table VII. The relationship between the noise and accuracy becomes questionable when we change many other parameters at the same time. Please consider removing all the rows other than the first 8 numbers to make the table simple and accurate. Please also adjust the description of the table to match this change. Also, column such as sample rate that are always 1 in our case, can be removed from the table and mentioned in the text.}
% \yiwei{Done.}

Additionally, we observed that accuracy improved with increasing $\epsilon$ across all DP methods. This trend is due to smaller $\epsilon$ values—corresponding to stronger privacy protection—introducing more noise, thus increasing data heterogeneity. CDP's accuracy gains with larger $\epsilon$ values were more pronounced than those of ODP and LDP. The noise addition during intermediate model aggregation in CDP allows for more effective training, whereas ODP's one-time noise or LDP's dispersed noise results in less impact on overall model performance.

In conclusion, while there is a trade-off between privacy and accuracy, our DP methods effectively maintain high accuracy levels, closely approximating that of the NDP baseline, while ensuring robust data privacy.


% % To evaluate the performance of our DP methods in FL, we conducted experiments using two benchmark datasets: MNIST and CIFAR-10. 
% % The goal was to assess the impact of different DP methods on the accuracy of the models while preserving privacy, under different threat models. 

% We assessed the accuracy of models trained using the MNIST and CIFAR-10 datasets across three differential privacy (DP) methods, i.e., ODP, CDP, LDP, and the Non-Differential Privacy (NDP) method as a baseline. Table~\ref{tab:dp_acc} presents the testing accuracy results (i.e., the best accuracy) for FL models under these DP methods, for varying privacy budget $\epsilon$.

% Generally, the NDP method, which does not add noise, achieves the highest accuracy. On average, ODP, CDP, and LDP methods result in accuracy reductions of approximately 5\%, 13\%, and 20\%, respectively. Notably, ODP exhibits superior accuracy compared to CDP and LDP. This is attributed to the fact that ODP only adds one-time noise at the final iteration, whereas CDP and LDP introduce noise at each iteration.
% % on the aggregated model, and LDP applies noise to individual client data transformations at every iteration.
% The reason why CDP generally achieves higher accuracy than LDP, particularly at larger $\epsilon$ values, is that CDP adds noise to the aggregated results, allowing the model to learn global patterns despite the presence of noise, whereas LDP applies noise to individual client data transformations, diminishing the model's ability to utilize data correlations and global information effectively.


% Furthermore, we observed that the accuracy improves with increasing $\epsilon$ across all three DP methods. This trend occurs because smaller $\epsilon$ values, which corresponds to stronger privacy protection, introduce more noise, increasing data heterogeneity. The accuracy improvement in CDP with larger $\epsilon$ values surpasses that of ODP and LDP, as CDP's noise addition during intermediate model aggregation allows for more effective training. In contrast, either the one-iteration noise in ODP or the dispersed impact of noise in LDP results in a smaller overall influence on the model. 

% % A higher $\epsilon$ value, which corresponds to weaker privacy protection, generally enhances the accuracy of both CDP and LDP, with improvements up to 1.09 and 1.03 times, respectively. This occurs because less noise is required for privacy preservation, leading to less distortion in the aggregated results and better model performance.


% In summary, although applying differential privacy does introduce a trade-off between privacy and accuracy, our DP methods effectively maintain a high level of accuracy, closely approximating that of the NDP baseline, while still ensuring data privacy.




% \begin{tcolorbox}[colback=gray!10,colframe=black,boxrule=1pt]
% \textbf{Takeaway:} Although applying differential privacy does introduce a trade-off between privacy and accuracy, our DP methods effectively maintained a high level of accuracy, closely approximating that of the NDP baseline, while still ensuring data privacy.
% \end{tcolorbox}

% Consequently, CDP generally achieves higher accuracy than LDP, particularly at larger $\epsilon$ values, as CDP allows the model to learn global patterns despite the presence of noise, whereas LDP's per-data-point noise diminishes the model's ability to utilize data correlations and global information effectively.



% \begin{figure}[!ht]
%   \centering
%   \includegraphics[width=1\linewidth]{figures/dp_acc.pdf}
%   \caption{The Accuracy of Different Privacy Module (MNIST)}
%   \label{fig:dp_acc}
% \end{figure}

% \subsection{RQ3: DP+FL Performance under different parameters}

% \subsubsection{DP Performance with different DP guarantees}
% \input{tables/dp_params}

% % overlap, one data in one client but not in another client


% To understand the trade-offs in our DP methods, we examined the effects of varying parameters. Our investigation, based on previous findings~\cite{opacus}, focused on how these parameters impact the accuracy of FL models. The four key parameters considered were 
% % the number of clients and
% three noise parameters, i.e., the privacy budget $\epsilon$, the number of training iterations, and the sample rate of clients. 
% The results are listed in Table~\ref{tab:dp_param}.


% % \noindent
% % \textbf{Number of Clients.}
% % % With the increasing number of clients, the accuracy of CDP is increasing, up to x1.43, as having more data from more clients or training with more iterations can help in better generalization, improving the model's performance, while keeping the same noise.
% % % But LDP, the more clients there are, the worse the accuracy is.
% % % This could be due to the fact that adding more noise at the local level for a larger number of clients aggregates to a higher total noise, degrading the overall model accuracy.
% % Increasing the number of clients generally improves the accuracy of CDP, with a reported increase of up to 1.43 times. 
% % This improvement is likely due to the greater data diversity and better generalization achieved with more clients, even when noise levels remain constant. In contrast, LDP shows a decrease in accuracy with more clients. This reduction is attributed to the cumulative effect of adding more noise at the local level, which deteriorates the overall model accuracy.


% \noindent
% \textbf{$\epsilon$.}
% % As $\epsilon$ increases, the accuracy of CDP and LDP generally improves, up to x1.09 and x1.03.
% % This is because a higher $\epsilon$, which corresponds to weaker privacy guarantees, allows for less added noise to reduce the distortion in the aggregated results, thus improving model performance.
% A higher $\epsilon$ value, which corresponds to weaker privacy protection, generally enhances the accuracy of both CDP and LDP, with improvements up to 1.09 and 1.03 times, respectively. This occurs because less noise is required for privacy preservation, leading to less distortion in the aggregated results and better model performance.


% \noindent
% \textbf{Number of Iterations.}
% % With the increasing number of iterations, the accuracy of CDP and LDP is increasing, even though the added noise is becoming larger.
% % This may result from the basic principle of FL training, that is, the more clients are involved and the more iterations are conducted, the better performance will be achieved.
% The accuracy of both CDP and LDP models improves with more training iterations, despite an increase in added noise. Because longer training with more iterations of computation, generally leads to better performance, as models have more opportunity to converge~\cite{yang2019federated}.
% % This result can be explained by the common observations of FL: more iterations and greater client involvement generally lead to better model performance.

% \noindent
% \textbf{Sample Rate.}
% An increase in sample rate leads to a slight improvement in the accuracy of both CDP and LDP. The sample rate impacts both the number of clients involved in the training and the amount of noise added for privacy. A larger sample rate allows for more client data to be used, which generally enhances model accuracy. However, it also necessitates more noise addition to preserve privacy, which can negatively impact accuracy. As a result, the opposing effects of increased data and added noise tend to balance each other out, leading to a marginal net gain in accuracy.

% \vspace{5pt}
% To achieve the best performance, a careful balance between model accuracy and noise levels for privacy protection is essential. The noise parameters should be optimized to meet specific privacy requirements while minimizing the impact on model performance.













% Our results show that the accuracy of CDP and LDP is slightly increasing when the sample rate is becoming larger, due to its double side impact.
% The sample rate of clients, on the one hand, affects the number of involved clients, and a larger sample rate will lead to better accuracy as more client data is used for training.
% On the other hand, it can also decide the added noise for privacy protection.
% With the increase of the sample rate, its two impacts are offset.


% \begin{tcolorbox}[colback=gray!10,colframe=black,boxrule=1pt]
% \textbf{Takeaway:} 
% % While higher noise levels provide stronger privacy guarantees, they also reduce model accuracy. 
% A careful balance between model accuracy and noise levels for privacy protection is essential. The noise parameters should be optimized to meet specific privacy requirements while minimizing the impact on model performance.
% \end{tcolorbox}

% In summary, our results indicate that while higher noise levels provide stronger privacy guarantees, they also reduce model accuracy. This necessitates a careful balance, where the noise parameters are optimized to provide adequate privacy without unduly compromising the model's performance. The choice of noise parameters can also be influenced by the sensitivity of the training data and the specific privacy requirements of the application.

% Moreover, the accuracy improves with the increasing number of iterations and client sample rate, even though the added noise is becoming larger.
% This may result from the basic principle of FL training, that is, the more clients are involved and the more iterations are conducted, the better performance will be achieved.
% In addition, with the increasing number of clients and same noise, the best accuracy is increasing, up to x1.43, as having more data from more clients or training with more iterations can help in better generalization, improving the model's performance.


% Things are similar for $\epsilon$, the number of iterations and the sample rate in LDP settings, as the more $\epsilon$ and the less iterations and sample rate are, the less noise will be added to the model training to protect privacy.
% But for the number of clients, the more clients there are, the worse the accuracy is.
% This could be due to the fact that adding more noise at the local level for a larger number of clients aggregates to a higher total noise, degrading the overall model accuracy.
% the more noise will be added in total, as LDP adopts DP (i.e., adding noise) at each client side.





% This a higher ε, which corresponds to weaker privacy guarantees, allows for better accuracy. The noise added to the data decreases with increasing ε (from 9.04 to 5.21), reducing the distortion in the aggregated results and thus improving model performance.
% LDP: Accuracy remains relatively flat at 0.68 regardless of ε. This suggests that LDP might be more resistant to changes in ε in terms of performance, potentially due to more noise being added at the local level, which might not reduce as significantly with increasing ε.

% Our analysis revealed that increasing the noise parameter generally leads to a decrease in accuracy, as the injected noise becomes more significant relative to the signal in the data. However, different DP methods responded differently to changes in noise levels. For instance, LDP, which applies noise at the local client level, showed a more pronounced decrease in accuracy compared to CDP, which aggregates the noise at the central server.

% The results indicate that while higher noise levels provide stronger privacy guarantees, they also reduce model accuracy. This necessitates a careful balance, where the noise parameters are optimized to provide adequate privacy without unduly compromising the model's performance. The choice of noise parameters can also be influenced by the sensitivity of the training data and the specific privacy requirements of the application.

% \yiwei{The performance of DP mainly depends on three parameters: epsilon, the number of iterations, and sample rate.
% The larger epsilon is, the less noise is added, the higher accuracy is.
% The less iterations are, the less noise is added, the higher accuracy is.
% The less sample rate is, the less noise is added, the higher accuracy is.}


% MNIST and CiFAR-10





\begin{algorithm}
\caption{Dilithium with Precomputation}\label{alg:dilifull}
% \small

\textbf{Precomputing} 

\raggedright{\textbf{Input:} Dilithium private key $sk$ and the number of groups for Dilithium parameters to be precomputed $N$.}

\textbf{Output:} $N$ groups of precomputed Dilithium parameters for $sk$

\begin{algorithmic}[1]
\Function{Precomputing}{$sk$, $N$}
    \While{\text{len(PreList[$sk$])} $<$ $N$}
        \State $y \gets \mathcal{S}^l_{\eta_1 - 1}$
        \State $w \gets \text{HighBits}(Ay, 2\eta_2)$
        \State Add ($y, w, sm$) into \text{PreList[$sk$]}
    \EndWhile
\EndFunction

\end{algorithmic}
\vspace{-1mm}
\hrulefill

\textbf{Signing} 

\raggedright{\textbf{Input:} Dilithium private key $sk$, message to be signed $M$, and the list of precomputed Dilithium parameters $PreList$.}

\textbf{Output:} the signature $\sigma$.

\begin{algorithmic}[1]

\Function{Sign}{$sk$, $M$, $PreList$}
    \For{$(y,w,sm) \text{ in } PreList$}
        \State $c \in \mathcal{B}^{60} := H(M \parallel sm)$
        \State $z := y + cs_1$
        \If{$\lVert z\rVert_{\infty} \leq \gamma_1 - \beta \text{ and } \lVert \text{LowBits}(Ay - cs_2, 2\eta_2) \rVert_{\infty} \leq \gamma_2 - \beta$}
            \State Remove $(y,w,sm)$ from $PreList$
            \State \Return{$\sigma = (z, c)$}
        \EndIf
    \EndFor
    \State $z := \bot$
    \While{$z = \bot$}
        \State $y \gets \mathcal{S}^l_{\eta_1 - 1}$
        \State $w \gets \text{HighBits}(Ay, 2\eta_2)$
        \State $c \in \mathcal{B}^{60} := H(M \parallel w_1)$
        \State $z := y + cs_1$
        \If{$\lVert z\rVert_{\infty} > \gamma_1 - \beta \text{ or } \lVert \text{LowBits}(Ay - cs_2, 2\eta_2) \rVert_{\infty} > \gamma_2 - \beta$}
            \State $z := \bot$
        \EndIf
    \EndWhile
    \State \Return{$\sigma = (z, c)$}
\EndFunction


\end{algorithmic}
\vspace{-1mm}
\hrulefill

\textbf{Verifying} 

\raggedright{\textbf{Input:} Dilithium public key $pk$, message $M$, and the signature $\sigma$.}

\textbf{Output:} the signature verification result.

\begin{algorithmic}[1]

\Function{Verify}{$pk$, $\sigma = (z, c)$}
    
    \State $w \gets \text{HighBits}(Az - ct, 2\eta_2)$
    \State \Return{$[\lVert z\rVert_{\infty} < \gamma_1 - \beta] \text{ and } \sigma = (z, c)$}
\EndFunction


\end{algorithmic}
\end{algorithm}




\section{Performance Evaluation }
% \subsection{Analytical Performance}

\subsection{Analytical Evaluation}\label{sec:analytical}


% We compare the analytical performance of \sys and the state-of-the-art in Table~\ref{tab:analytical}.
% Setting up \sys incurs two runs of key generation protocol and $k$ runs of key agreement protocol.
% Additionally, the user and assisting node perform $T*k$ and $T*|U|$ $\PRF$ invocations to pre-compute $T$ groups of masks, respectively， as well as $N$ $\precomputesgn$ operations to pre-compute the $N$ groups of signing parameters.
% \sys improves the computational cost over \flamingo as $k$ can be as small as~$2$, while the number of participating decryptors $|D'|$ is at least $64$ in Flamingo~\cite{flamingo}.
% Moreover, we also compare \sys with the maliciously-secure version of MicroSecAgg~\cite{guo2022microsecagg}.
% MicroSecAgg incurs a linear number of signature verification, key agreement, secret sharing, and symmetric encryption and decryption algorithms, which make it more costly than \sys.
% The key material of the protocol of Bell~et al.~\cite{bell2020secure} cannot be reused across multiple rounds; therefore, the setup phase should be repeated in each aggregation phase.
% Additionally, when compared with \eseafl, \sys incurs an additional cost for precomputing signing parameters and masks. Fortunately, such precomputation will be used to optimize the subsequent aggregation and will not affect the offline setup phase too much.


% In the Aggregation phase of \sys, the user only performs $k + 1$ summation, and two signature generations to achieve malicious security.
% Specially, the user does not have to perform $\PRF$ as the masks are precomputed in Setup phase.
% Given that $k$ is significantly smaller than the number of participating users/decryptors, this results in higher efficiency than its counterparts.



We compare the analytical performance of \sys and the state-of-the-art in Table~\ref{tab:analytical}.
Setting up \sys incurs two runs of key generation protocol and $k$ runs of key agreement protocol.
Additionally, the user and assisting node perform $T*k$ and $T*|U|$ $\PRF$ invocations to pre-compute $T$ groups of masks, respectively， as well as $N$ $\precomputesgn$ operations to pre-compute the $N$ groups of signing parameters.
\sys improves the computational cost over \flamingo as $k$ can be as small as~$2$, while the number of participating decryptors $|D'|$ is at least $64$ in Flamingo~\cite{flamingo}.
% Note that $k$ can be as small as~$2$, while the number of participating decryptors $|D'|$ is at least $64$ in Flamingo~\cite{flamingo}.
We also compare \sys with the maliciously-secure version of MicroSecAgg~\cite{guo2022microsecagg}.
MicroSecAgg incurs a linear number of signature verification, key agreement, secret sharing, and symmetric encryption and decryption algorithms, which make it more costly than \sys.
The key material of the protocol of Bell~et al.~\cite{bell2020secure} cannot be reused across multiple rounds; therefore, the setup phase should be repeated in each aggregation phase.


In the Aggregation phase of \sys, the user only performs $k + 1$ summation, and two signature generations to achieve malicious security.
Given that $k$ is significantly smaller than the number of participating users/decryptors, this results in higher efficiency than its counterparts.

\begin{table*}[!t]
	\centering
 \footnotesize
	 \caption{Analytical performance of the secure aggregation of \sys~and its counterparts}
	\label{tab:analytical}
 % \vspace{-1em}
 	 \resizebox{1\textwidth}{!}{
	\begin{threeparttable}
	\begin{tabular}{|c|c|c|c||c|c|c|}
			\hline
		\multirow{2}{*}{\textbf{Scheme}} & \multicolumn{3}{c||}{\textbf{Setup Phase}} & \multicolumn{3}{c|}{\textbf{Aggregate Phase} }	\\	 \cline{2-7}
		 & \textbf{User} &
		 \begin{tabular}{@{}c@{}c@{}}
		 \textbf{Assisting/Helper} \\ \textbf{Nodes} \end{tabular}& \textbf{Server} &
		 \textbf{User} &
		 \begin{tabular}{@{}c@{}c@{}}
		 \textbf{Assisting/Helper} \\ \textbf{Nodes} \end{tabular} & \textbf{Server}	\\	\hline
% 		  \cite{Bell2020} & N/A & N/A & N/A
% &\begin{tabular}{@{}c@{}c@{}}
% $2_\Kg+2_{\sshl} +\log n (1_\SEnc+1_\SDec + $ \\
% ${1_\Ka + 2_\Sgn+2_\Vfy})+(2\log n)_\Su$ \end{tabular}& N/A &$1_\Rssh + 2\log n_\Su$\\\hline


MicroFedML \cite{microfedml} &
		\begin{tabular}{@{}c@{}c@{}} $1_\Kg + 1_\Sgn+|U'-1|(1_\Vfy+$
		\\
		$1_\Ka + 1_{\sshl} + 1_\AEnc+1_\ADec)$
		\end{tabular} & N/A
		& ${|U|_\Vfy }$
		&\begin{tabular}{@{}c@{}c@{}} $(|w|+1)_\Ex+1_\Sgn+$\\$|U-1|(1_\Su+1_\Vfy)+1_\Su$ \end{tabular}& N/A & \begin{tabular}{@{}c@{}c@{}} $1_{\Rsshe} +|w|_\Ex + $\\
		$1_\Mu$\end{tabular}	\\	\hline

  
	Flamingo	\cite{flamingo} &
		$|D'|_\Vfy$
		& \begin{tabular}{@{}c@{}c@{}}$2_{\PIL} + 3_\Sgn+2_{\sshl} +$	\\ $	|D|(3|D'|+1)_\Vfy + $\\
		$(|D'|\cdot|D|)_\Mu$\end{tabular}
		& $(|D'|\cdot|D|)_\Vfy$ & \begin{tabular}{@{}c@{}c@{}} $2_\PRG+|D'|(1_\Ex+1_\Hash+1_\PRF+$\\$1_\Su+1_\AEnc+1_\Sgn+1_\SEnc)+1_{\sshl}$ \end{tabular}&\begin{tabular}{@{}c@{}c@{}}$1_\Sgn+|U'|_\SDec +$ \\ $(|D|+|U'|)_\Vfy
		$\end{tabular}
		&
		\begin{tabular}{@{}c@{}c@{}} $|D|_{\PIL}+|U'|(1_\Su + $ \\ $1_\Mu +1_\Rssh)+2_\PRG+ $ \\ $ (|U'|+1)_\Su $ \end{tabular}
		\\	\hline
		
		


		 \eseafl \cite{behnia2023efficient}&
		 $2_\Kg + k_\Ka$
		 & $2_\Kg + k_\Ka$
		 & $1_\Kg$
		 & $k_\PRF+|k+1|_\Su+2_\Sgn$ &\begin{tabular}{@{}c@{}c@{}} $|U'| (1_\Vfy+1_\Su+ $\\
		 $1_\PRF)+ {1_\Sgn}$\end{tabular}
		 & \begin{tabular}{@{}c@{}c@{}}$(|U'|+|k|)(1_\Vfy + $ \\ $1_\Su)$
		 \end{tabular}\\
		 \hline


   
		 \sys &
		 $2_\Kg + k_\encap + N_\precomputesgn+(T\times k)_\PRF$
		 & $2_\Kg + |U|_\decap + (T\times|U|)_\PRF$
		 & $1_\Kg$
		 & $|k+1|_\Su+2_\PSgn$ &\begin{tabular}{@{}c@{}c@{}} $|U'| (1_\Vfy+1_\Su) $\\
		 $+ {1_\Sgn}$\end{tabular}
		 & \begin{tabular}{@{}c@{}c@{}}$(|U'|+|k|)(1_\Vfy + $ \\ $1_\Su)$
		 \end{tabular}\\
		 \hline
		 		 
	\end{tabular}
\begin{tablenotes}[para, flushleft]
	 
	$\Kg$, $\Sgn$, $\Vfy$, and $\Hash$ denote key generation, signature generation, verification, and hash function, respectively.
	$\Ka$ denotes the shared key computation in the key agreement protocol.
	$|D|$ and $|D'|$ denote the number of all decryptors and the threshold of participating decryptors~\cite{sp/MaWAPR23}, respectively.
	$\PIL$ denotes polynomial interpolation of length $L$.
	$\sshl$, $\Rssh$, and $\Rsshe$ denote secret sharing operation to $l$ shares, share reconstruction, and share reconstruction in the exponent, respectively.
	$\Mu$, $\Su$ and $\Ex$ denote multiplication, summation and exponentiation operations, respectively.
	$\PRG$ and $\PRF$ denote pseudorandom generators and pseudorandom functions, respectively.
	$\AEnc$, $\ADec$, $\SEnc$, and $\SDec$ denote asymmetric encryption, decryption, symmetric encryption, and decryption, respectively.
	$|w|$ denotes the number of model parameters.
	$k$ is the set of assisting nodes in \sys.
 \rouzbeh{we use pSGN to refer to dilithium with precompute, can you please make sure the naming matches throughout the text and with algo 5.}
	\end{tablenotes}
	\end{threeparttable}
		 }
   
\end{table*}

\subsection{Implementation}
We implement \sys with 2.5k lines of code, involving two components, namely the secure aggregation for gradient updates and the model training with multiple DP protections.
Our code is available at \todo{\url{https://github.com}}.

\noindent
\textbf{Secure Aggregation.}
\sys builds on the  ABIDES~\cite{byrd2019abides}, a discrete event simulation framework commonly used in FL researches~\cite{flamingo,microfedml}, enabling the simulation of multi-iterative aggregation protocols.
We incorporated two post-quantum algorithms, i.e., the \texttt{Kyber} key encapsulation algorithm for negotiating shared secrets between clients and assisting nodes, and \texttt{Dilithium} signing algorithm for generating and verifying digital signatures during aggregation phase.
These algorithms are implemented based on existing libraries~\cite{kyberpy, dilic}, with \texttt{Dilithium} modified to support signing with precomputation in C. 
For the Pseudo-Random Function (PRF) used in mask generation, we employed \texttt{ASCON}~\cite{dobraunig2021ascon}, known for its lightweight and efficient cryptography, making it suitable for resource-constrained client devices.

% The end-to-end FL implementations of \sys are based on ABIDES~\cite{byrd2019abides}, a discrete event simulation framework with modifications to enable the simulation of multi-iterative aggregation protocols, widely used by existing FL works~\cite{flamingo,microfedml}.
% \sys adopts two post-quantum algorithms, i.e., the \texttt{Kyber} key encapsulation algorithm
% %and users 
% and \texttt{Dilithium} signing algorithm, to negotiate shared secrets between clients and assisting nodes, and generate and verify digital signatures for each message during aggregation phase, respectively.
% Both those algorithms are implemented based on existing libraries~\cite{kyberpy, dilic}, which we modified the \texttt{Dilithium} %several modifications 
% to support signing with precomputation implemented in the C language.
% For the Pseudo-Random Function (PRF) used to generate the masks, we use \texttt{ASCON}~\cite{dobraunig2021ascon}, which implements lightweight and efficient cryptography, suitable for limited-resource client devices.

\noindent
\textbf{Model Training with Multiple DP Protections.}
We follow the approach by Yang \textit{et al.}~\cite{yang2023privatefl} for FL model training, to instantiate the FL model training, incorporating DP protections using \texttt{PyTorch Opacus}~\cite{opacus}.
Specifically, we implemented two DP methods to handle different threat models, as detailed in Section~\ref{sec:pqfl:dp}, along with a baseline FL model without DP protection.


% Based on that, the DP privacy protection is incorporated via \texttt{PyTorch Opacus}~\cite{opacus}.
% Specifically, we implement two DP methods under different threat models, as described in Section~\ref{sec:pqfl:dp}, as well as the one without DP protection as baseline.

\subsection{Experimental Environment}
All experiments were conducted on an x86\_64 Linux machine with AMD Ryzen Threadripper PRO 5965WX 24-Cores and 256 GB RAM. 
The models were trained using three GeForce RTX 3090 graphics cards (NVIDIA).
We used benchmark datasets MNIST~\cite{xiao2017fashion} and CIFAR-10~\cite{krizhevsky2009learning}, employing Fully-connected and ResNet-18 models, respectively, as in previous FL study~\cite{yang2023privatefl}.

% We used multiple benchmark datasets following previous FL works~\cite{yang2023privatefl}, i.e., MNIST~\cite{xiao2017fashion} and CIFAR-10~\cite{krizhevsky2009learning}, using as models Fully-connected and ResNet-18, respectively. 



\subsection{Experimental Setup and Evaluation Metrics}
% We conducted two types of experiments to evaluate \sys, i.e., efficiency and performance. 
% For efficiency, we compute both computational complexity and empirical assessment of time, while for performance, we measured the accuracy and DP guarantees. 
We systematically evaluated \sys with respect to two key dimensions: efficiency  and performance.
Efficiency was measured by empirical time complexity during the Setup and Aggregation phases, along with corresponding bandwidth usage. 
Performance was assessed based on accuracy using two widely recognized machine learning benchmarks: MNIST and CIFAR-10. 
In the following, we describe the three empirical metrics employed in our experiments.

% We systematically evaluated \sys with respect to two key dimensions: efficiency  and performance. The efficiency evaluation encompasses empirical time complexity during the Setup and Aggregation phases, alongside their corresponding bandwidth usage. Performance evaluation, on the other hand, measures \sys's accuracy using two widely recognized machine learning benchmarks: MNIST and CIFAR10. In the following, we describe the three empirical metrics employed in our experiments.

\noindent
\textbf{Metrics for Efficiency:} We use two metrics, i.e., computation time and communication bandwidth, for efficiency measurement.
Comparative analysis was conducted using \flamingo\cite{flamingo}, \pqsa\cite{yang2022post}, \eseafl\cite{behnia2023efficient}, and \micro\cite{microfedml}.
% \noindent
% \textbf{Computation Time.}
\begin{itemize}
\item \textit{Computation Time.} To assess the efficiency of our secure aggregation method with post-quantum protection, we measured the time required for computational operations such as key encapsulation, mask generation, signing, and verification. The number of clients (N) was varied from 200 to 1000, with three assisting nodes (M=3) and one aggregation server. 
We also tested performance with a gradient vector size of 16,000 to simulate high-dimensional data. 
% Comparative analysis was conducted using \flamingo\cite{flamingo}, \pqsa\cite{yang2022post}, \eseafl\cite{behnia2023efficient}, and \micro\cite{microfedml}, 
Besides, consistent experimental setups were adopted in the compared works, specifically three assisting nodes/decryptors are used for \flamingo and \eseafl.

\item \textit{Communication Bandwidth.} We recorded the bandwidth, i.e., total message size exchanged between clients, assisting nodes, and the server, to evaluate communication costs.
% The bandwidth, i.e., the total size of messages exchanged between clients, (assisting nodes,) and the server, is recorded to evaluate communication cost. 
% Message size is prioritized over transmission time due to the latter's susceptibility to variations in network conditions and hardware performance.
The reason why we use message size instead of transmission time is because message transmission time highly depends on current network conditions. Variations in hardware and network quality can greatly affect latency.
\end{itemize}


% We record the time taken by computational operations, such as key encapsulation, mask generation, signing and verifying, to evaluate the efficiency of our secure aggregation method with post-quantum protections.
% Specifically, we vary the client number (N) from 200 to 1000 with M (with M=3 as default) assisting nodes and one aggregation server. 
% We also use $w$ with 16,000 gradients to test the performance under high-dimensional gradient vectors. 
% Moreover, we use \pqsa\cite{yang2022post}, \eseafl\cite{behnia2023efficient}, \flamingo\cite{flamingo} and \micro\cite{microfedml} for the comparative analysis. 
% To have a similar environment for the comparative analysis, we employ an identical setup for \pqsa, \eseafl, \micro and \flamingo. 
% We select three assisting nodes/decryptors for \eseafl and \flamingo.

% \noindent
% \textbf{Communication Cost.}
% We record the total size of messages transmitted between each entity, i.e., clients, assisting nodes, and the server, to evaluate the communication cost.
% % The reason why we use message size instead of transmission time is because message transmission time highly depends on current network conditions. Variations in hardware and network quality can greatly affect latency.

\noindent
\textbf{Metric for Performance:}
We accessed the performance of our differential privacy (DP) methods by evaluating the \textit{accuracy} of the final models. Client data allocation adheres to standard protocols~\cite{yang2023privatefl}. Unless stated otherwise, experiments were conducted with 100 clients (N=100), 100 iterations, and a sample rate of 1.



% \todo{Training data assignment to clients follows established protocols~\cite{yang2023privatefl}. 
% Default parameter settings are detailed in Table xxx, adhered to unless stated otherwise.}



% https://www.usenix.org/system/files/usenixsecurity23-yang-yuchen.pdf
% https://arxiv.org/pdf/2304.03841



\renewcommand{\arraystretch}{1.2}
\begin{table}[ht]
\centering
\caption{Results of Differential Privacy Accuracy: Iterations = 100, Sample Rate = 1.}
\label{tab:dp_acc}
% \resizebox{1\columnwidth}{!}{
\begin{tabular}{|c|c|c|c||c|c|c|}
% \toprule[1.5pt]
% \textbf{Dataset} & \textbf{$\epsilon$} & \textbf{DP} & \textbf{Noise} & \textbf{Best Acc} \\
% \midrule
% \multirow{5}{*}{\textbf{MNIST}} & \multirow{4}{*}{\textbf{$\epsilon$}}
\hline
\multirow{2}{*}{\textbf{$\epsilon$}} & \multicolumn{3}{c||}{\textbf{MNIST}} & \multicolumn{3}{c|}{\textbf{CIFAR-10}} \\ \cline{2-7}
% & \textbf{NFL}
& \textbf{NDP} & \textbf{CDP} & \textbf{LDP} 
% & \textbf{NFL} 
& \textbf{NDP} & \textbf{CDP} & \textbf{LDP} \\ \hline
% % \multicolumn{2}{c|}{\textbf{NFL}} & \multicolumn{2}{c|}{\textbf{NPFL}} & \multicolumn{2}{c|}{\textbf{Setup 1}} & \multicolumn{2}{c|}{\textbf{Setup 2}} & \multicolumn{2}{c}{\textbf{Setup 3}} \\ \cline{2-11}
% % & \textbf{MNIST} & \textbf{CIFAR} & \textbf{MNIST} & \textbf{CIFAR} & \textbf{MNIST} & \textbf{CIFAR} & \textbf{MNIST} & \textbf{CIFAR} & \textbf{MNIST} & \textbf{CIFAR} \\ 
% \midrule

% 2  & 0.86 & 0.82 & 0.45 & 0.65 & 0.96 & 0.96 & 0.41 & 0.47 \\ \hline
4  & 0.86 & 0.76 & 0.67 & 0.96 & 0.88 & 0.61 \\ \hline
6  & 0.86 & 0.82 & 0.68 & 0.96 & 0.90 & 0.68 \\ \hline
8  & 0.86 & 0.83 & 0.68 & 0.96 & 0.90 & 0.72 \\ \hline
10 & 0.86 & 0.84 & 0.68 & 0.96 & 0.90 & 0.74 \\ \hline
12 & 0.86 & 0.84 & 0.68 & 0.96 & 0.90 & 0.75  \\ \hline

% \bottomrule[1.5pt]
\end{tabular}
% }
\end{table}


% \renewcommand{\arraystretch}{1.2}
% \begin{table*}[ht]
% \centering
% \caption{Results of Differential Privacy Accuracy (with MNIST~\cite{xiao2017fashion} and CIFAR-10~\cite{krizhevsky2009learning}).}
% \label{table:dp_acc}
% \begin{tabular}{c|c|c|c|c|c|c|c|c|c|c}
% \toprule[1.5pt]
% \multirow{2}{*}{\textbf{Round}} & \multicolumn{5}{c|}{\textbf{MNIST}} & \multicolumn{5}{c}{\textbf{CIFAR}} \\ \cline{2-11}
% & \textbf{NFL} & \textbf{NDP} & \textbf{ODP} & \textbf{CDP} & \textbf{LDP} & \textbf{NFL} & \textbf{NDP} & \textbf{ODP} & \textbf{CDP} & \textbf{LDP} \\ 
% % \multicolumn{2}{c|}{\textbf{NFL}} & \multicolumn{2}{c|}{\textbf{NPFL}} & \multicolumn{2}{c|}{\textbf{Setup 1}} & \multicolumn{2}{c|}{\textbf{Setup 2}} & \multicolumn{2}{c}{\textbf{Setup 3}} \\ \cline{2-11}
% % & \textbf{MNIST} & \textbf{CIFAR} & \textbf{MNIST} & \textbf{CIFAR} & \textbf{MNIST} & \textbf{CIFAR} & \textbf{MNIST} & \textbf{CIFAR} & \textbf{MNIST} & \textbf{CIFAR} \\ 
% \midrule

% 1   & 0.72 & 0.25 & 0.12 & 0.12 & 0.10 
%     & 0.83 & 0.11 & 0.12 & 0.11 & 0.10 \\ \hline
% 20  & 0.98 & 0.85 & 0.66 & 0.56 & 0.36 
%     & 0.99 & 0.47 & 0.45 & 0.67 & 0.35 \\ \hline
% 40  & 0.99 & 0.85 & 0.69 & 0.64 & 0.50 
%     & 1.00 & 0.61 & 0.58 & 0.76 & 0.41 \\ \hline
% 60  & 1.00 & 0.91 & 0.67 & 0.78 & 0.60 
%     & 1.00 & 0.70 & 0.67 & 0.79 & 0.39 \\ \hline
% 80  & 1.00 & 0.93 & 0.81 & 0.94 & 0.65 
%     & 1.00 & 0.76 & 0.72 & 0.81 & 0.44 \\ \hline
% 100 & 1.00 & 0.93 & 0.77 & 0.96 & 0.67 
%     & 1.00 & 0.79 & 0.76 & 0.81 & 0.47 \\

% \bottomrule[1.5pt]
% \end{tabular}
% \end{table*}



\section{Evaluation}

In this section, we present the experimental results evaluating the efficiency and performance of \sys. Our findings address the following key research questions:

% \reza {We systematically evaluate our proposed \sys in two dimensions: efficiency  and performance. Our efficiency evaluation experiments include empirical time complexity of Setup phase and Aggregation phase and their corresponding bandwidths, respectively. Our performance evaluation assesses \sys's accuracy on two widely-used machine learning benchmark, MNIST and CIFAR10.}\\
% \yiwei{Can this be moved to previous subsection?}

% \reza{Dear Yiwei, please consider removing "RQ1" and "RQ2" and have each section as a numbered section instead.}\\
% \yiwei{Done.}

% \reza {We need to include Figures 3, 4, 5, and 6 in their corresponding numbered subsection provided in the paragraph above.}\\

% \reza{Yiwei, once these structural changes are done, I can do another pass and revise the writing. Thanks!}

\begin{itemize}

\item \textbf{Section~\ref{sec:eval:eff} (Efficiency Measurement)}: How efficient is post-quantum enhanced secure aggregation in FL? What gains in efficiency does \sys achieve through the use of pre-computation?
% How does the efficiency of \sys improve by the introduction of pre-computation?
\item \textbf{Section~\ref{sec:eval:perf} (Model Performance Measurement)}: How does \sys’s differential privacy module perform under different threat models? What is the impact of DP-enhanced methods on FL performance across different training datasets?
% How does the differential privacy module in \sys perform under different threat models? What is the performance of the DP-enhanced method in FL across different training datasets?
\end{itemize}

\subsection{Efficiency Measurement}~\label{sec:eval:eff}

\reza{For this and next section, I suggest we refer to figures at 3.a, 3.b, and 3.c in the text, instead of generally referring by Figure 3. Same applies to Figure 4 and Figure 5.}

\subsubsection{Computational Cost}
We systematically compare the computational cost of \sys in the Setup phase and Aggregation phase with four state-of-the-art approaches, i.e., \flamingo, \pqsa, \eseafl, and \micro.
% The results are listed in Table~\ref{table:sa_time}.

% \input{tables/sa_time}


\begin{figure*}[htbp]
    \centering
    \begin{minipage}{0.32\textwidth}
        \centering
        \includegraphics[width=\textwidth]{figures/sa_setup_time/sa_time_setup_server.pdf}
        \caption*{(a) Server}
    \end{minipage}
    \hfill
    \begin{minipage}{0.32\textwidth}
        \centering
        \includegraphics[width=\textwidth]{figures/sa_setup_time/sa_time_setup_client.pdf}
        \caption*{(b) Client}
    \end{minipage}
    \hfill
    \begin{minipage}{0.32\textwidth}
        \centering
        \includegraphics[width=\textwidth]{figures/sa_setup_time/sa_time_setup_node.pdf}
        \caption*{(c) Assisting node}
    \end{minipage}
    \caption{Computation Time of the Setup phase (The dimension of the weight list is set to 16K.)}
    \label{fig:sa_setup_time}
\end{figure*}


\vspace{5pt}
\noindent
\textbf{Setup Phase.}
Figure~\ref{fig:sa_setup_time} illustrates the computation costs of each method during the Setup phase.
Generally, for \sys, the computation time on the server (Figure~\ref{fig:sa_setup_time} (a)) and client (Figure~\ref{fig:sa_setup_time} (b)) side remains nearly constant, whereas it increases for assisting nodes as the number of clients grows (Figure~\ref{fig:sa_setup_time} (c)).
This is because the operations \sys performs on the client side are primarily dependent on the number of assisting nodes, which typically remains constant in general FL settings, and the fact that server-side operations have a constant computational cost.
In contrast, assisting nodes perform tasks, such as shared secret generation, that scale with the number of clients, leading to increased computation time as the client count rises.
% {\color{red}
% \reza{It is not clear to me what is meant by "directly related to the number of clients."}
% In contrast, the tasks performed by assisting nodes, such as shared secret generation, are related to the number of clients. 
% That is, the computation time is increasing with the increased number of clients.

Our results also show that, in the Setup phase, \sys incurs higher computation times compared to \flamingo, \eseafl and \micro across all entities.
The is due to \sys incorporating an additional precomputation step in the Setup phase, where several digital signature parameters are precomputed for subsequent runtime signing (see Section~\ref{sec:pqfl:sign}).

Additionally, \pqsa is excluded from this comparison as it only distributes several public parameters without performing significant computations. It's also worth noting that \flamingo does not involve any client-side operations, as it relies on a trusted third party to generate and distribute signing keys for each entity.


% \begin{itemize}
% \item Server and Assisting Node: \sys takes less time than \flamingo and \micro during the Setup phase. 
% The reason is that during the setup phase, the server and assisting nodes of \sys only need to generate their key pair and send their public key to the clients. 
% In contrast, 
% % Except generating and sending the public key, 
% the server and decryptors of \flamingo have to perform a distributed key generation (DKG) protocol to generate and distribute secret key shares for the asymmetric encryption scheme among the decryptors, without revealing the key to any single entity. 
% For \micro, the server must receive the client encryption keys, verify the signatures, manage client mask sharing, and ensure an adequate number of online clients.
%  % if the online users are enough.
% \elisa{In figure 3, I would change "User" with "Client" as in the text here we use "client".}
% \item Client: \sys takes less time than \flamingo and \microfirst but more time than \microsecond. The reason is that the clients of \sys perform key generation and key exchange to generate shared secret with each assisting node, and then send the public key to the server.
% The clients involved in \flamingo have to receive public keys from decryptors and verify their signatures.
% The client computation time for both \sys and \flamingo is proportional to the number of assisting nodes/decryptors but constant to the number of users. 
% For \microfirst, clients have to perform mask sharing with other clients, which is more computationally intensive than the secret sharing between users and assisting nodes in \sys.
% % the computation of which is larger than secret sharing between the users and assisting nodes in \sys.
% For \microsecond, clients only distribute shares among other users within the same group.
% \end{itemize}



\begin{figure*}[htbp]
    \centering
    \begin{minipage}{0.32\textwidth}
        \centering
        \includegraphics[width=\textwidth]{figures/sa_agg_time/sa_time_agg_server.pdf}
        \caption*{(a) Server}
    \end{minipage}
    \hfill
    \begin{minipage}{0.32\textwidth}
        \centering
        \includegraphics[width=\textwidth]{figures/sa_agg_time/sa_time_agg_client.pdf}
        \caption*{(b) Client}
    \end{minipage}
    \hfill
    \begin{minipage}{0.32\textwidth}
        \centering
        \includegraphics[width=\textwidth]{figures/sa_agg_time/sa_time_agg_node.pdf}
        \caption*{(c) Assisting node}
    \end{minipage}
    \caption{Computation Time of the Aggregation phase (The dimension of the weight list is set to 16K.)}
    \label{fig:sa_agg_time}
\end{figure*}


\vspace{5pt}
\noindent
\textbf{Aggregation Phase.}
Figure~\ref{fig:sa_agg_time} shows the computation time of \sys in the Aggregation phase compared with that of \flamingo, \pqsa, \eseafl, and \micro.
In \sys, the computation time for clients remains constant (Figure~\ref{fig:sa_agg_time} (b)), while it increases for the server (Figure~\ref{fig:sa_agg_time} (a)) and assisting nodes (Figure~\ref{fig:sa_agg_time} (c)) as the number of clients grows.
This increase is due to the need for assisting nodes and the server to verify the signatures of messages sent by clients, making computation time proportional to the number of clients.

The results demonstrate that all entities in \sys incur minimal computational overhead, with computation times significantly lower than those in \flamingo, \pqsa, and \micro, with the exception of \eseafl.
% regarding users, assisting nodes, and the server.
Specifically, \sys demonstrates a similar computation time to \eseafl on the client side, but a higher computation time on the assisting nodes and server.
This difference arises because both \sys and \eseafl clients perform similar operations, including gradient masking and a few signing operations. However, the assisting nodes and server in \sys must conduct a large number of signature verifications, which scale with the number of clients. The post-quantum signing algorithm (i.e., Dilithium) used by \sys is originally slower than the traditional algorithm (i.e., ECDSA) used in \eseafl, leading to higher computation times as the number of clients increases.

\sys outperforms \flamingo, \pqsa, and \micro in terms of computation time across clients, assisting nodes, and the server. 
\flamingo requires additional steps to remove masks for dropout clients, necessitating extra \yiwei{information} (e.g., \yiwei{shares of secrets used to generate the masks}) from clients and decryptors to allow the server to recover the gradient vectors of those offline clients.
\pqsa uses SHPRG-based encryption for gradient masking, which involves an extra step between clients and the server to decrypt and recover the masks and calculate the aggregated result.
In \micro, each client must additionally compute $H(k)^{X_i}$ and $H(k)^{R_i}$, and the server has to recover the gradient vector by calculating the discrete logarithm of $H(k)^{X_i} - H(k)^{R_i}$. Such discrete logarithm calculation is computationally very intensive, especially as the vector dimensions increase.

Overall, compared with the existing works, \sys employs a straightforward strategy for dropout clients by ignoring the masked vectors of dropped clients and it utilizes a post-quantum algorithm with precomputation for optimization. 
This approach reduces the number of messages, eliminates unnecessary calculations, and significantly reduces time overhead while maintaining quantum security.

% Generally, \sys employs a straightforward strategy that simply removes and ignores the masked vectors of dropout clients, and constructs a post-quantum algorithm protected communications with a precomputation for optimization.
% Thus it requires a smaller number of messages, eliminating unnecessary calculations and significantly reducing time overhead while keeping quantum-secure.

% \begin{itemize}
% \item \micro incurs the highest cost because each client has to calculate $H(k)^{X_i}$ and $H(k)^{R_i}$ and the server must recover the vector by calculating the discrete logarithm of $H(k)^{X_i} - H(k)^{R_i}$. This discrete logarithm calculation is computationally very intensive, especially as the vector dimensions increase.
% \item \flamingo takes more time than \sys because it involves removing the masks for those dropout clients. Consequently, the clients and decryptors have to provide additional materials (e.g., secret shares) for the server to recover the local vector. 
% \sys, however, employs a straightforward strategy that simply removes and ignores the masked vectors of dropout clients.
% % \elisa{The wording "message utilization" is not very good. Do you mean that "it requires a smaller number of messages"?}
% % While \sys may reduce message utilization, it eliminates unnecessary calculations, significantly reducing time overhead.
% Thus it requires a smaller number of messages, eliminating unnecessary calculations and significantly reducing time overhead.
% \end{itemize}

% The results show that \sys generally has a better performance than \flamingo and \micro in terms of the computation cost in Setup phase, as the computation time of \sys on server and assisting node sides is greatly lower than that of \flamingo and \micro though the computation time of \sys is slightly higher than \micro on the client side.
% \todo{This is because \micro does not generate a signature for its masked input.
% Although it generates a signature for the online set, but the signing algorithm is simple without taking too much time but achieving low security.}




\subsubsection{Communication Cost}
We analyze the communication cost, specifically the outbound bandwidth, of \sys during the Setup and Aggregation phases in comparison to existing approaches.

% \input{tables/sa_size}


\begin{figure*}[htbp]
    \centering
    \begin{minipage}{0.32\textwidth}
        \centering
        \includegraphics[width=\textwidth]{figures/sa_setup_size/sa_size_setup_server.pdf}
        \caption*{(a) Server}
    \end{minipage}
    \hfill
    \begin{minipage}{0.32\textwidth}
        \centering
        \includegraphics[width=\textwidth]{figures/sa_setup_size/sa_size_setup_client.pdf}
        \caption*{(b) Client}
    \end{minipage}
    \hfill
    \begin{minipage}{0.32\textwidth}
        \centering
        \includegraphics[width=\textwidth]{figures/sa_setup_size/sa_size_setup_node.pdf}
        \caption*{(c) Assisting node}
    \end{minipage}
    \caption{Bandwidth in the Setup Phase (The dimension of the weight list is set to 16K.)}
    \label{fig:sa_setup_bw}
\end{figure*}

\vspace{5pt}
\noindent
\textbf{Setup Phase.}
Figure~\ref{fig:sa_setup_bw} presents the outbound bandwidth costs of all entities in \sys during the Setup phase. 
In general, the outbound bandwidth of \sys remains constant on the server (Figure~\ref{fig:sa_setup_bw} (a)) and client (Figure~\ref{fig:sa_setup_bw} (b)) sides while increases on the assisting nodes (Figure~\ref{fig:sa_setup_bw} (c)) as the number of clients grows.
This is due to the fact that during the Setup phase, the server only needs to broadcast its public key for signing, and each client sends the public keys for key exchange and signing to the assisting nodes, whose number keeps constant in our experimental setting.
However, each assisting node must send these public keys to all clients, making its outbound bandwidth dependent on the number of clients.


\sys incurs less outbound bandwidth than \flamingo and \micro but is generally comparable to \eseafl across all three entities.
Specifically, during the Setup phase, \sys and \eseafl perform the same public key exchange operations, resulting in similar outbound bandwidths, both of which depend on the size of the public keys.
In contrast, in \flamingo, the server and decryptors participate in DKG protocols, where their outbound bandwidth depends on the number and size of the messages in DKG protocols and is proportional to the number of decryptors, but constant relative to the number of clients. This results in greater outbound bandwidth for the server and decryptors in \flamingo compared to \sys, which only involves public key exchanges.
As for \micro, the server has to forward all the communications, i.e., the public keys and \yiwei{secret shares generated by Shamir’s secret sharing scheme}, from one client to the other, making its bandwidth proportional to the number of clients and higher than that of \sys. Each client in \micro should send its public key and $N-1$ mask shares to all other clients, making its bandwidth increase proportional to the number of clients, which is significantly higher than that of \sys.


Additionally, \pqsa and the clients of \flamingo are excluded from this comparison for the same reasons previously mentioned.

% \begin{itemize}
% \item Server: The server in \sys broadcasts its public key to clients, thus its bandwidth depends on the public key size. The server in \flamingo participates in the DKG protocols, where the bandwidth depends
% %\elisa{do you mean depends on "the number of messages" or on the "size of the messages" or on both?} \yiwei{both}
% on the number and size of
% the messages of DKG protocols and is proportional to the number of decryptors, but constant relative to the number of clients. 
% In \micro, the server forwards all the communications, i.e., the public keys and secret shares, from one client to the others, making its bandwidth proportional to the number of clients.
% % all the communications such as the distribution of the DH keys and encrypted shares need to be communicated via the aggregation server, which incurs a significant communication overhead.
% \item Client: In \sys, each client should send its public key and the encrypted secret to each assisting node, thus its bandwidth is constant relative to the number of clients. In \micro, each client should send its public key and (N-1) mask shares to all the other clients, making its bandwidth proportional to the number of clients, thus higher than that of \sys. \flamingo is excluded here as its clients do not send any messages during this phase.
% \item Assisting Node: During the setup phase, each assisting node in \sys sends its public key to each client, thus its bandwidth is proportional to the number of clients. 
% In \flamingo, the decryptors involved in DKG protocols have a bandwidth dependent on DKG messages and proportional to the number of decryptors but constant relative to the number of clients.
% \end{itemize}


\begin{figure*}[htbp]
    \centering
    \begin{minipage}{0.32\textwidth}
        \centering
        \includegraphics[width=\textwidth]{figures/sa_agg_size/sa_size_agg_server.pdf}
        \caption*{(a) Server}
    \end{minipage}
    \hfill
    \begin{minipage}{0.32\textwidth}
        \centering
        \includegraphics[width=\textwidth]{figures/sa_agg_size/sa_size_agg_client.pdf}
        \caption*{(b) Client}
    \end{minipage}
    \hfill
    \begin{minipage}{0.32\textwidth}
        \centering
        \includegraphics[width=\textwidth]{figures/sa_agg_size/sa_size_agg_node.pdf}
        \caption*{(c) Assisting node}
    \end{minipage}
    \caption{Bandwidth in the Aggregation phase (The dimension of the weight list is set to 16K.)}
    \label{fig:sa_agg_bw}
\end{figure*}


\noindent
\textbf{Aggregation Phase.}
We present the outbound bandwidth cost of all entities in \sys during the runtime Aggregation phase in Figure~\ref{fig:sa_agg_bw}. 
Generally, the outbound bandwidth of \sys remains constant across all three entities, i.e., the server (Figure~\ref{fig:sa_agg_bw} (a)), the clients (Figure~\ref{fig:sa_agg_bw} (b)), and the assisting nodes (Figure~\ref{fig:sa_agg_bw} (c)) as the number of clients increases.
This stability occurs because the outbound messages for each entity do not depend on the number of clients. Specifically, each client's outbound messages depend only on the number of assisting nodes and the server, which remain constant in our experimental setup. Assisting nodes send a single message (containing the sum of partial masks) to the server, and the server broadcasts the aggregated results, keeping their outbound bandwidth unchanged.

When compared with existing works, \sys demonstrates lower outbound bandwidth costs across all entities compared to \flamingo, \pqsa, \eseafl, and \micro.
Specifically, in \flamingo, the server is involved in forwarding the messages between the clients and decryptors, leading to a higher outbound bandwidth that is roughly proportional to the number of clients.
Clients have to send {\color{red}secret shares} to decryptors and \yiwei{neighbors (i.e., clients in the same group)}, in addition to masked updates to the server, which increases their outbound bandwidth proportional to the number of decryptors and clients (i.e., neighbors), which is significantly higher than \sys.
Decryptors also transmit decrypted secret shares of each client to the server, resulting in higher bandwidth proportional to the number of clients, compared to \sys.
For \pqsa, the server performs an additional communication step with clients to decrypt and recover the masks, resulting in a higher bandwidth that is proportional to the number of clients.
Similarly, clients have to additionally send the decrypted secrets, except for the masked updates, leading to a higher bandwidth, which is proportional to the number of clients.
While \eseafl performs the similar operations to \sys across all entities, the difference in outbound bandwidth is primarily due to the size of each message, especially the size of signatures.
As for \micro, similar to \flamingo, the server has to forward the signature of each client to other clients, incurring a higher outbound bandwidth than \sys, which is proportional to the number of clients. 
Moreover, clients in \micro send masks of online clients along with the masked updates to the server, resulting in bandwidth higher than in \sys.

% \begin{itemize}
% \item Server: In \sys, the server only broadcasts the final update during the aggregation phase, thus its outbound bandwidth is the size of the final update and constant to the number of clients. Servers in \flamingo, \pqsa and \micro have to get involved in forwarding the client message to the decryptors or other clients to assist in recovering the masks of dropout clients and managing secret sharing among clients, thus their bandwidth is higher than that of \sys and roughly proportional to the number of clients. 
% % The server of \micro has to report the online client set to each client and forwards the signature of each client to other clients, as well as distribute the final update, thus its bandwidth is more than \sys and \flamingo and proportional to the number of clients.
% \item Client: Clients in \sys send masked updates and iteration numbers to the server and assisting nodes separately, with the bandwidth being dependent on the update vector size and proportional to the number of assisting nodes but constant relative to the number of clients.
% In \flamingo, clients send masked updates to the server and secret shares to decryptors and neighbors, making their bandwidth proportional to the number of decryptors and clients (i.e., neighbors).
% Clients in \micro send masked updates and masks of online clients to the server, resulting in bandwidth higher than \sys but lower than \flamingo. 
% Clients in \pqsa have to additionally send the split secrets of each other client, except to the masked update, leading to the highest bandwidth proportional to the number of clients.
% \item Assisting Node: Each assisting node in \sys should send the sum of masks of online clients to the server, thus its bandwidth is the size of the update and constant to the number of clients.
% In \flamingo, decryptors send decrypted secret shares of each client to the server, resulting in higher bandwidth proportional to the number of clients compared to \sys.
% \end{itemize}



\subsubsection{Precomputation Improvement}


\input{tables/precomputed}

To assess the impact of precomputation strategies on \sys, we conducted a comparative experiment implementing \sys without precomputation in the Dilithium signing algorithms and mask generation. The results, shown in Table~\ref{table:precomputed}, indicate that precomputation significantly enhances efficiency for both assisting nodes and clients as the number of clients increases.

Without precomputation, an assisting node must perform additional mask generation operations for $N$ clients and one signing operation, while a client must perform additional mask generation for $M$ assisting nodes and $M+1$ signing operations. Consequently, precomputation notably reduces the computational burden on these entities.

On the server side, the benefits of precomputation are less pronounced. The reason is that the server performs relatively fewer computational operations, limited to only one signing operation, compared to the assisting nodes and clients.


% To evaluate how precomputation strategies enhance \sys, e conducted a comparative experiment, in which we implemented \sys without precomputations, i.e., in Dilithium signing algorithms and mask generation.
% The results are listed in Table~\ref{table:precomputed}.
% We can see that precomputation could greatly improve the efficiency on assisting nodes and clients with the increasing number of clients.
% This is because without precomputation, one assisting node has to perform additional N mask generation for N clients and one signing operation, and one client has to perform additional M mask generation and M+1 signing operations. 
% Moreover, precomputations did not improve a lot on the server side, as the server perform much less computational operations (i.e., only one signing operation) than the assisting nodes and clients.

% \yiwei{Precomputation could greatly improve the efficiency on assisting nodes with the increasing number of clients.}


% \subsubsection{Number of Clients}
% We explore how different number of clients (ranging from 200 to 1000) affects the performance of secure aggregation in \sys.
% xxx and xxx show the computation time and outbound bandwidth of \sys when the number of clients varies.
% We observe that \sys consistently outperforms xxx and xxx in both time and bandwidth, especially when the system has more clients.
% For instance, the xxx gap between \sys and xxx increases from xxx\% with 200 clients to xxx\% with 1000 clients.




\subsection{Model Performance}~\label{sec:eval:perf}


% \subsubsection{DP Performance with MNIST and CIFAR-10}
% \reza{performance on MNIST should be generally higher than CIFAR10 as it is a much easier dataset. Can we double check to see why we get better performance with CIFAR10?}

% \reza{have we introduced LDP and CDP before?}

We evaluated the accuracy of machine learning models trained by \sys on the MNIST and CIFAR-10 datasets using two differential privacy (DP) methods, CDP and LDP, and compared them to a No-Differential Privacy (NDP) baseline. 
Table~\ref{tab:dp_acc} presents the best testing accuracy for federated learning (FL) models under these DP methods, with varying privacy budgets ($\epsilon$).

\input{tables/dp_acc}

As expected, the NDP method, which does not introduce noise, achieved the highest accuracy. On average, the accuracy reductions for CDP, and LDP were approximately 10\%, and 28\%, respectively. 
% Notably, ODP demonstrated superior accuracy compared to CDP and LDP. This can be attributed to ODP's addition of noise only at the final iteration, unlike CDP and LDP, which introduce noise at every iteration. 
CDP generally outperformed LDP, particularly at larger $\epsilon$ values, consistent with findings in~\cite{yang2023privatefl}. This is because CDP adds noise to aggregated results, allowing the model to better capture global patterns despite the noise. In contrast, LDP's noise application to individual client data at each iteration can diminish the model's ability to leverage data correlations and global information effectively.
% \elisa{I think that the above results is consistent with previous work as it is well known that LDP results in much less accuracy as one has to add a lot of noise to the data. Could we perhaps mention some references here?}
% \yiwei{Done.}


% \reza {I think we need to only keep the first 8 rows of Table VII. The relationship between the noise and accuracy becomes questionable when we change many other parameters at the same time. Please consider removing all the rows other than the first 8 numbers to make the table simple and accurate. Please also adjust the description of the table to match this change. Also, column such as sample rate that are always 1 in our case, can be removed from the table and mentioned in the text.}
% \yiwei{Done.}

\yiwei{Additionally, we observed that accuracy improved with increasing $\epsilon$ across all DP methods. This trend is due to smaller $\epsilon$ values—corresponding to stronger privacy protection—introducing more noise, thus increasing data heterogeneity. 
CDP's accuracy gains with larger $\epsilon$ values were more pronounced than those of LDP. The noise addition during intermediate model aggregation in CDP allows for more effective training, whereas LDP's {\color{red}dispersed} noise results in less impact on overall model performance.
Moreover, the increasing rate is slower when large $\epsilon$. This is due to the noise multiplier is non-linear decreasing with $\epsilon$ in opcaus DP library. When $\epsilon$ becomes larger, the change rate of noise multiplier is slower. 


In conclusion, while there is a trade-off between privacy and accuracy, our DP methods effectively maintain high accuracy levels, closely approximating that of the NDP baseline, while a ensuring robust data privacy.}


% % To evaluate the performance of our DP methods in FL, we conducted experiments using two benchmark datasets: MNIST and CIFAR-10. 
% % The goal was to assess the impact of different DP methods on the accuracy of the models while preserving privacy, under different threat models. 

% We assessed the accuracy of models trained using the MNIST and CIFAR-10 datasets across three differential privacy (DP) methods, i.e., ODP, CDP, LDP, and the Non-Differential Privacy (NDP) method as a baseline. Table~\ref{tab:dp_acc} presents the testing accuracy results (i.e., the best accuracy) for FL models under these DP methods, for varying privacy budget $\epsilon$.

% Generally, the NDP method, which does not add noise, achieves the highest accuracy. On average, ODP, CDP, and LDP methods result in accuracy reductions of approximately 5\%, 13\%, and 20\%, respectively. Notably, ODP exhibits superior accuracy compared to CDP and LDP. This is attributed to the fact that ODP only adds one-time noise at the final iteration, whereas CDP and LDP introduce noise at each iteration.
% % on the aggregated model, and LDP applies noise to individual client data transformations at every iteration.
% The reason why CDP generally achieves higher accuracy than LDP, particularly at larger $\epsilon$ values, is that CDP adds noise to the aggregated results, allowing the model to learn global patterns despite the presence of noise, whereas LDP applies noise to individual client data transformations, diminishing the model's ability to utilize data correlations and global information effectively.


% Furthermore, we observed that the accuracy improves with increasing $\epsilon$ across all three DP methods. This trend occurs because smaller $\epsilon$ values, which corresponds to stronger privacy protection, introduce more noise, increasing data heterogeneity. The accuracy improvement in CDP with larger $\epsilon$ values surpasses that of ODP and LDP, as CDP's noise addition during intermediate model aggregation allows for more effective training. In contrast, either the one-iteration noise in ODP or the dispersed impact of noise in LDP results in a smaller overall influence on the model. 

% % A higher $\epsilon$ value, which corresponds to weaker privacy protection, generally enhances the accuracy of both CDP and LDP, with improvements up to 1.09 and 1.03 times, respectively. This occurs because less noise is required for privacy preservation, leading to less distortion in the aggregated results and better model performance.


% In summary, although applying differential privacy does introduce a trade-off between privacy and accuracy, our DP methods effectively maintain a high level of accuracy, closely approximating that of the NDP baseline, while still ensuring data privacy.




% \begin{tcolorbox}[colback=gray!10,colframe=black,boxrule=1pt]
% \textbf{Takeaway:} Although applying differential privacy does introduce a trade-off between privacy and accuracy, our DP methods effectively maintained a high level of accuracy, closely approximating that of the NDP baseline, while still ensuring data privacy.
% \end{tcolorbox}

% Consequently, CDP generally achieves higher accuracy than LDP, particularly at larger $\epsilon$ values, as CDP allows the model to learn global patterns despite the presence of noise, whereas LDP's per-data-point noise diminishes the model's ability to utilize data correlations and global information effectively.



% \begin{figure}[!ht]
%   \centering
%   \includegraphics[width=1\linewidth]{figures/dp_acc.pdf}
%   \caption{The Accuracy of Different Privacy Module (MNIST)}
%   \label{fig:dp_acc}
% \end{figure}

% \subsection{RQ3: DP+FL Performance under different parameters}

% \subsubsection{DP Performance with different DP guarantees}
% \input{tables/dp_params}

% % overlap, one data in one client but not in another client


% To understand the trade-offs in our DP methods, we examined the effects of varying parameters. Our investigation, based on previous findings~\cite{opacus}, focused on how these parameters impact the accuracy of FL models. The four key parameters considered were 
% % the number of clients and
% three noise parameters, i.e., the privacy budget $\epsilon$, the number of training iterations, and the sample rate of clients. 
% The results are listed in Table~\ref{tab:dp_param}.


% % \noindent
% % \textbf{Number of Clients.}
% % % With the increasing number of clients, the accuracy of CDP is increasing, up to x1.43, as having more data from more clients or training with more iterations can help in better generalization, improving the model's performance, while keeping the same noise.
% % % But LDP, the more clients there are, the worse the accuracy is.
% % % This could be due to the fact that adding more noise at the local level for a larger number of clients aggregates to a higher total noise, degrading the overall model accuracy.
% % Increasing the number of clients generally improves the accuracy of CDP, with a reported increase of up to 1.43 times. 
% % This improvement is likely due to the greater data diversity and better generalization achieved with more clients, even when noise levels remain constant. In contrast, LDP shows a decrease in accuracy with more clients. This reduction is attributed to the cumulative effect of adding more noise at the local level, which deteriorates the overall model accuracy.


% \noindent
% \textbf{$\epsilon$.}
% % As $\epsilon$ increases, the accuracy of CDP and LDP generally improves, up to x1.09 and x1.03.
% % This is because a higher $\epsilon$, which corresponds to weaker privacy guarantees, allows for less added noise to reduce the distortion in the aggregated results, thus improving model performance.
% A higher $\epsilon$ value, which corresponds to weaker privacy protection, generally enhances the accuracy of both CDP and LDP, with improvements up to 1.09 and 1.03 times, respectively. This occurs because less noise is required for privacy preservation, leading to less distortion in the aggregated results and better model performance.


% \noindent
% \textbf{Number of Iterations.}
% % With the increasing number of iterations, the accuracy of CDP and LDP is increasing, even though the added noise is becoming larger.
% % This may result from the basic principle of FL training, that is, the more clients are involved and the more iterations are conducted, the better performance will be achieved.
% The accuracy of both CDP and LDP models improves with more training iterations, despite an increase in added noise. Because longer training with more iterations of computation, generally leads to better performance, as models have more opportunity to converge~\cite{yang2019federated}.
% % This result can be explained by the common observations of FL: more iterations and greater client involvement generally lead to better model performance.

% \noindent
% \textbf{Sample Rate.}
% An increase in sample rate leads to a slight improvement in the accuracy of both CDP and LDP. The sample rate impacts both the number of clients involved in the training and the amount of noise added for privacy. A larger sample rate allows for more client data to be used, which generally enhances model accuracy. However, it also necessitates more noise addition to preserve privacy, which can negatively impact accuracy. As a result, the opposing effects of increased data and added noise tend to balance each other out, leading to a marginal net gain in accuracy.

% \vspace{5pt}
% To achieve the best performance, a careful balance between model accuracy and noise levels for privacy protection is essential. The noise parameters should be optimized to meet specific privacy requirements while minimizing the impact on model performance.













% Our results show that the accuracy of CDP and LDP is slightly increasing when the sample rate is becoming larger, due to its double side impact.
% The sample rate of clients, on the one hand, affects the number of involved clients, and a larger sample rate will lead to better accuracy as more client data is used for training.
% On the other hand, it can also decide the added noise for privacy protection.
% With the increase of the sample rate, its two impacts are offset.


% \begin{tcolorbox}[colback=gray!10,colframe=black,boxrule=1pt]
% \textbf{Takeaway:} 
% % While higher noise levels provide stronger privacy guarantees, they also reduce model accuracy. 
% A careful balance between model accuracy and noise levels for privacy protection is essential. The noise parameters should be optimized to meet specific privacy requirements while minimizing the impact on model performance.
% \end{tcolorbox}

% In summary, our results indicate that while higher noise levels provide stronger privacy guarantees, they also reduce model accuracy. This necessitates a careful balance, where the noise parameters are optimized to provide adequate privacy without unduly compromising the model's performance. The choice of noise parameters can also be influenced by the sensitivity of the training data and the specific privacy requirements of the application.

% Moreover, the accuracy improves with the increasing number of iterations and client sample rate, even though the added noise is becoming larger.
% This may result from the basic principle of FL training, that is, the more clients are involved and the more iterations are conducted, the better performance will be achieved.
% In addition, with the increasing number of clients and same noise, the best accuracy is increasing, up to x1.43, as having more data from more clients or training with more iterations can help in better generalization, improving the model's performance.


% Things are similar for $\epsilon$, the number of iterations and the sample rate in LDP settings, as the more $\epsilon$ and the less iterations and sample rate are, the less noise will be added to the model training to protect privacy.
% But for the number of clients, the more clients there are, the worse the accuracy is.
% This could be due to the fact that adding more noise at the local level for a larger number of clients aggregates to a higher total noise, degrading the overall model accuracy.
% the more noise will be added in total, as LDP adopts DP (i.e., adding noise) at each client side.





% This a higher ε, which corresponds to weaker privacy guarantees, allows for better accuracy. The noise added to the data decreases with increasing ε (from 9.04 to 5.21), reducing the distortion in the aggregated results and thus improving model performance.
% LDP: Accuracy remains relatively flat at 0.68 regardless of ε. This suggests that LDP might be more resistant to changes in ε in terms of performance, potentially due to more noise being added at the local level, which might not reduce as significantly with increasing ε.

% Our analysis revealed that increasing the noise parameter generally leads to a decrease in accuracy, as the injected noise becomes more significant relative to the signal in the data. However, different DP methods responded differently to changes in noise levels. For instance, LDP, which applies noise at the local client level, showed a more pronounced decrease in accuracy compared to CDP, which aggregates the noise at the central server.

% The results indicate that while higher noise levels provide stronger privacy guarantees, they also reduce model accuracy. This necessitates a careful balance, where the noise parameters are optimized to provide adequate privacy without unduly compromising the model's performance. The choice of noise parameters can also be influenced by the sensitivity of the training data and the specific privacy requirements of the application.

% \yiwei{The performance of DP mainly depends on three parameters: epsilon, the number of iterations, and sample rate.
% The larger epsilon is, the less noise is added, the higher accuracy is.
% The less iterations are, the less noise is added, the higher accuracy is.
% The less sample rate is, the less noise is added, the higher accuracy is.}


% MNIST and CiFAR-10

==> sections/related.tex <==
\section{Related Works}
\todo{user or client or party?}
\todo{iterations or steps or rounds?}

\elisa{The related work is not well organized. First of all, I would replace subsection A with a subsection titled "Secure Aggregation for Federated Learning" which cover the crypto based approaches (including the ones using MPC), while subsection B can be titled "Differential Privacy for FL" or "Differentially Private FL". Also I would not repeat what FL means as you have already said this in the intro.}
\subsection{Federated Learning (FL)}
Federated Learning (FL)~\cite{mcmahan2017communication} is a technique that enables a group of users to jointly train a machine learning (ML) model without the data ever leaving the respective users’ devices. FL involves a server that coordinates the training in an iterative process. In each round, the server selects a subset of users to contribute to the learning round. Each user then selects a subsample of their training data, called a mini-batch, computes the gradients of an objective function for these samples, and sends these gradients, known as local updates, to the server. The server updates the shared model by aggregating the received gradients, adjusting them by a learning-rate parameter, and applying the changes to the shared model, which is then sent back to the users.

While the FL paradigm appears to offer privacy assurances, the exchange of model updates still poses potential risks. 
Prior works~\cite{boenisch2023curious, fowl2021robbing, wen2022fishing} have demonstrated that an untrusted server can directly extract user data from the model gradients by inserting a fully connected model layer as an extraction module, allowing direct extraction of individual data points. 
Wen et al.\cite{wen2022fishing} describe how the server can modify model parameters to extract single data points by increasing their gradient contributions.
Some researchers~\cite{fan2023blockchain, wang2021secure, tramer2016stealing, fung2020limitations, yang2023privatefl} have also revealed that untrusted clients (i.e., endpoint users) in FL can compromise model training. 
On the one hand, clients may be honest but curious, following the aggregation protocol but attempting to retrieve private training data from the received global models. 
On the other hand, compromised or malicious clients may upload poisoned local model parameters to the server, leading to inaccurate global model aggregation and distorting local model updates. 
Additionally, some works~\cite{yao2021secure, wang2021secure} discuss that external attackers can eavesdrop on server-client communications to intercept and analyze the uploaded parameters or replace the parameters with poisoned ones during the FL training process.


\subsection{Secure Aggregation in FL}
Secure aggregation enables federated learning (FL) by allowing collaborative training of clients using local gradient updates without exposing raw data, thereby preserving participant privacy. 
Numerous secure aggregation protocols applied in FL scenarios have been proposed.
Several works, including \cite{liu2024bfl, bonawitz2017practical, bell2020secure, so2021turbo}, utilize pairwise masks to conceal individual inputs. These pairwise masks are calculated based on a secret key agreed upon with other clients, which automatically cancel out each other when the server accumulates the received gradients.
Protocols such as \texttt{FastSecAgg}~\cite{kadhe2020fastsecagg}, \texttt{Turbo-Aggregate}~\cite{so2021turbo}, and \texttt{Lightsecagg}~\cite{so2022lightsecagg} use a secret-sharing-based Multi-Party Computation (MPC) to compute sums. MPC facilitates secure aggregation by allowing multiple parties to collectively train a model without sharing raw data.
Additionally, some works employ threshold additive homomorphic encryption~\cite{dasu2022prov, elahi2014privex, truex2019hybrid} for secure aggregation. In this approach, gradient aggregation is performed on ciphertexts without decryption, ensuring that sensitive data remains encrypted throughout the collaborative learning process.



\subsection{Differential Privacy in FL}
Some researchers~\cite{dwork2006differential, dwork2006calibrating} consider applying Differential Privacy (DP) approaches to safeguard users' sensitive data from disclosure during training. 
DP ensures that the participation of any specific client does not noticeably increase the likelihood of the observed messages (e.g., individual updates or trained models) by adding noise.
Differential Privacy techniques can be applied to FL in various ways. 
One approach is the central DP scheme (i.e., CDP), where the server adds DP-compliant noise to the aggregate update~\cite{kairouz2021advances, balle2020privacy, kairouz2021practical, ramaswamy2020training}. This method requires trusting the server, as it has access to the unprotected aggregate update.
However, when the server is untrusted or susceptible to compromise by attackers (e.g., via side-channel attacks~\cite{chen2021voltpillager, van2018foreshadow, chamikara2022local, truex2020ldp}), an alternative approach is the local DP scheme (i.e., LDP). 
In this scheme, each sampled client adds DP noise to perturb its local update. As long as the noise added by each client is sufficient to guarantee DP on its own, the client’s privacy is preserved regardless of the behavior of other clients or the server.


% \subsection{Our Method}
% In this paper, we propose \sys, a novel privacy-preserving federated learning protocol.
% Specifically, \sys has three features:
% \begin{enumerate}
% \item \textbf{Introducing post-quantum algorithms to support stronger adversary models.} 
% Existing works~\cite{} do not adequately consider the potential threats posed by quantum computing. As a result, they are limited by their reliance on classical cryptographic algorithms, which are vulnerable to attacks by quantum adversaries.
% In contrast, \sys integrates post-quantum algorithms (i.e., \todo{\texttt{ASCON} as PRF}, \texttt{Kyber} for secret agreement, and \texttt{Dilithium} for digital signatures), which ensures robust security even in the face of potential quantum attacks, thereby significantly enhancing security against sophisticated adversary models and surpassing the protection offered by existing solutions.

% \item \textbf{Integrating both secure aggregation and differential privacy to protect user private training data.}
% \yiwei{protecting training data and protecting final model privacy-preserving.}
% The current approaches~\cite{} are limited by their focus on either secure aggregation or differential privacy, failing to leverage the synergistic benefits of combining both techniques and provide comprehensive protection against a wide range of threats.
% On the one hand, secure aggregation does not protect against inference attacks once the aggregated data is available. Even though the data is protected during transmission, the aggregated results could still reveal patterns or trends that compromise the privacy of individuals.
% On the other hand, differential privacy techniques can ensure that the released data does not compromise individual privacy, but without secure aggregation, the data is vulnerable to interception and tampering during transmission. This will cause a risk of data breaches before the privacy guarantees of differential privacy are applied.
% Hence, \sys combines both secure aggregation and differential privacy to enhance data protection. Moreover, considering different threat models, we explore the best practice of such a combination, investigating performance and security trade-off.

% \item \textbf{Enhancing security while keeping efficiency and effectiveness.}
% Post-quantum cryptographic algorithms provide enhanced security by safeguarding against quantum attacks. However, they suffer from low efficiency due to increased computational complexity and larger key sizes. Additionally, the implementation of these algorithms introduces significant performance overheads, especially impacting processing time in FL environment.
% To tackle the challenge, \sys adopts a pre-computed post-quantum algorithms, in which an additional pre-computation step to calculate offline parameters will be performed before the main algorithms.
% This will save a lot of runtime processing time especially for digital signatures required by every messages during model update transmission.
% Moreover, inspired by~\cite{behnia2023efficient}, \sys introduce the assisting nodes into the FL procedure, which share secrets with users and assist the in unmasking the final gradients.
% This can not only reduce the communication overhead but also be greatly tolerate to dropout users. 

% \end{enumerate}


==> tables/dp_params.tex <==
\renewcommand{\arraystretch}{1.2}
\begin{table}[ht]
\centering
\caption{Results of Differential Privacy Accuracy among Different Parameters (with MNIST).}
\label{tab:dp_param}
\begin{tabular}{c|c|c|c|c|c|c}
\toprule[1.5pt]
\textbf{DP} & \textbf{N} & \textbf{$\epsilon$} & \textbf{Iters} & \textbf{SR} & \textbf{Noise} & \textbf{Best Acc} \\

\midrule

\multirow{3}{*}{CDP} & 100 & 4 & 100 & 1 & 9.04 & 0.76  \\ \cline{2-7}
 & 100 & 6 & 100 & 1 & 6.52 & 0.82  \\ \cline{2-7}
 & 100 & 8 & 100 & 1 & 5.21 & 0.83  \\ \cline{2-7}
 & 100 & 10 & 100 & 1 & 4.38 & 0.84  \\ \hline
\multirow{3}{*}{LDP} & 100 & 4 & 100 & 1 & 2.84-3.13 & 0.66  \\ \cline{2-7}
 & 100 & 6 & 100 & 1 & 2.10-2.31& 0.68 \\ \cline{2-7}
 & 100 & 8 & 100 & 1 & 1.73-1.89 & 0.68 \\ \cline{2-7}
 & 100 & 10 & 100 & 1 & 1.50-1.63 & 0.68 \\
\midrule
\multirow{3}{*}{CDP} & 100 & 6 & 60 & 1 & 5.05  & 0.78  \\ \cline{2-7}
 & 100 & 6 & 100 & 1 & 6.52 & 0.82 \\ \cline{2-7}
 & 100 & 6 & 150 & 1 & 7.99 & 0.82 \\ \hline
\multirow{3}{*}{LDP} & 100 & 6 & 60 & 1 & 1.70-1.85 & 0.58 \\ \cline{2-7}
 & 100 & 6 & 100 & 1 & 2.10-2.31 & 0.68 \\ \cline{2-7}
 & 100 & 6 & 150 & 1 & 2.51-2.77 & 0.69 \\ 
\midrule
\multirow{3}{*}{CDP} & 100 & 6 & 100 & 0.5 & 3.36 & 0.81  \\ \cline{2-7}
 & 100 & 6 & 100 & 0.7 & 4.62 & 0.82 \\ \cline{2-7}
 & 100 & 6 & 100 & 1 & 6.52 & 0.83 \\ \hline
\multirow{3}{*}{LDP} & 100 & 6 & 100 & 0.5 & 1.58-1.72 & 0.62  \\ \cline{2-7}
 & 100 & 6 & 100 & 0.7 & 1.81-1.98 & 0.66 \\ \cline{2-7}
 & 100 & 6 & 100 & 1 & 2.10-2.31 & 0.68 \\ 
% \midrule
% \multirow{3}{*}{CDP} & 50 & 6 & 100 & 1 & 6.52 & 0.58 \\ \cline{2-7}
%  & 100 & 6 & 100 & 1 & 6.52 & 0.82 \\ \cline{2-7}
%  & 150 & 6 & 100 & 1 & 6.52 & 0.83 \\ \hline
% \multirow{3}{*}{LDP} & 50 & 6 & 100 & 1 & 1.63-1.70 & 0.69 \\ \cline{2-7}
%  & 100 & 6 & 100 & 1 & 2.10-2.31 & 0.68 \\ \cline{2-7}
%  & 150 & 6 & 100 & 1 & 2.59-2.78 & 0.57 \\ 

\bottomrule[1.5pt]
\end{tabular}
\end{table}

==> tables/sa_size.tex <==
\renewcommand{\arraystretch}{1.2}
\begin{table*}[ht]
\centering
\caption{Outbound Bandwidth of Secure Aggregation (KB): B - \sys, F - \flamingo, P - \pqsa, M$_1$ - \microfirst, M$_2$ - \microsecond.}
\label{table:sa_size}
 \resizebox{2\columnwidth}{!}{
\begin{tabular}{c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c}
\toprule[1.5pt]
\multirow{3}{*}{\textbf{N}} & \multicolumn{8}{c|}{\textbf{Client}} & \multicolumn{3}{c|}{\textbf{Assisting Node}} & \multicolumn{9}{c}{\textbf{Server}} \\ \cline{2-21}
& \multicolumn{3}{c|}{\textbf{Setup}} & \multicolumn{5}{c|}{\textbf{Aggregation}} & \multicolumn{1}{c|}{\textbf{Setup}} & \multicolumn{2}{c|}{\textbf{Aggregation}} & \multicolumn{4}{c|}{\textbf{Setup}} & \multicolumn{5}{c}{\textbf{Aggregation}} \\ \cline{2-21}
& \textbf{B} & \textbf{M$_1$} & \textbf{M$_2$} & \textbf{B} & \textbf{F} & \textbf{P} & \textbf{M$_1$} & \textbf{M$_2$} & \textbf{B} & \textbf{B} & \textbf{F} & \textbf{B} & \textbf{F} & \textbf{M$_1$} & \textbf{M$_2$} & \textbf{B} & \textbf{F} & \textbf{P} & \textbf{M$_1$} & \textbf{M$_2$} \\ \midrule
% & \textbf{\sys} & \textbf{\flamingo} & \textbf{\micro} & \textbf{\sys} & \textbf{\flamingo} & \textbf{\micro} & \textbf{\sys} & \textbf{\flamingo} & \textbf{\micro} & \textbf{\sys} & \textbf{\flamingo} & \textbf{\micro} & \textbf{\sys} & \textbf{\flamingo} & \textbf{\micro} & \textbf{\sys} & \textbf{\flamingo} & \textbf{\micro} \\ \hline


200  & \textbf{6} & 180 & 15 & \textbf{130} & 107 & 337696 &  9625 & 9625 & \textbf{360}  & \textbf{128} & 64  & \textbf{0.2}  & 27 & 41786   & 4084  & \textbf{128} & 9840  & 506128 & 101573  & 101573  \\ \hline
400  & \textbf{6} & 359 & 30 & \textbf{130} & 116 & 546904 & 9625 & 9625 & \textbf{719}  & \textbf{128} & 147  & \textbf{0.2}  & 27 & 167016  & 15866 & \textbf{128} & 23185 & 884936 & 206272  & 206272  \\ \hline
600  & \textbf{6} & 529 & 44 & \textbf{130} & 115 & 746904 & 9625 & 9625 & \textbf{1078} & \textbf{128} & 206  & \textbf{0.2} & 27 & 364898  & 35564 & \textbf{128} & 29294 & 1255112 & 314095  & 314095  \\ \hline
800  & \textbf{6} & 718 & 58 & \textbf{130} & 116 & 965344 & 9625 & 9625 & \textbf{1438} & \textbf{128} & 298  & \textbf{0.2} & 27 & 667844  & 62650 & \textbf{128} & 46345 & 1643056 & 425044 & 425044 \\ \hline
1000 & \textbf{6} & 888 & 71 & \textbf{130} & 120 & 1165344 & 9625 & 9625 & \textbf{1797} & \textbf{128} & 447 & \textbf{0.2} & 27 & 1025430 & 96281 & \textbf{128} & 73194 & 2012976 & 539117 & 539117 \\ 
\bottomrule[1.5pt]
\end{tabular}
}


\end{table*}





% \renewcommand{\arraystretch}{1.2}
% \begin{table*}[ht]
% \centering
% \caption{Outbound Bandwidth of Secure Aggregation (KB): P - \sys, F - \flamingo, M1 - \microfirst, M2 - \microsecond.}
% \label{table:sa_size}
%  \resizebox{2\columnwidth}{!}{
% \begin{tabular}{c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c}
% \toprule[1.5pt]
% \multirow{3}{*}{\textbf{N}} & \multicolumn{7}{c|}{\textbf{User}} & \multicolumn{3}{c|}{\textbf{Assisting Node / Decryptor}} & \multicolumn{8}{c}{\textbf{Server}} \\ \cline{2-19}
% & \multicolumn{3}{c|}{\textbf{Setup}} & \multicolumn{4}{c|}{\textbf{Aggregation}} & \multicolumn{1}{c|}{\textbf{Setup}} & \multicolumn{2}{c|}{\textbf{Aggregation}} & \multicolumn{4}{c|}{\textbf{Setup}} & \multicolumn{4}{c}{\textbf{Aggregation}} \\ \cline{2-19}
% & \textbf{B} & \textbf{M$_1$} & \textbf{M$_2$} & \textbf{B} & \textbf{F} & \textbf{M$_1$} & \textbf{M$_2$} & \textbf{B} & \textbf{B} & \textbf{F} & \textbf{B} & \textbf{F} & \textbf{M$_1$} & \textbf{M$_2$} & \textbf{B} & \textbf{F} & \textbf{M$_1$} & \textbf{M$_2$} \\ \midrule
% % & \textbf{\sys} & \textbf{\flamingo} & \textbf{\micro} & \textbf{\sys} & \textbf{\flamingo} & \textbf{\micro} & \textbf{\sys} & \textbf{\flamingo} & \textbf{\micro} & \textbf{\sys} & \textbf{\flamingo} & \textbf{\micro} & \textbf{\sys} & \textbf{\flamingo} & \textbf{\micro} & \textbf{\sys} & \textbf{\flamingo} & \textbf{\micro} \\ \hline


% 200  & \textbf{10576} & 183904 & 15760 & \textbf{210384} & 18133480 & 922 & 922 & \textbf{368232}  & \textbf{117536} & 2033120  & \textbf{46400}  & 25920 & 42788800   & 4182400  & \textbf{231096} & 5718528  & 1617600  & 1617600  \\ \hline
% 400  & \textbf{10576} & 367512 & 30224 & \textbf{210384} & 37127920 & 922 & 922 & \textbf{736232}  & \textbf{117536} & 5321576  & \textbf{92800}  & 25920 & 171024000  & 16246400 & \textbf{247096} & 12665568 & 6435200  & 6435200  \\ \hline
% 600  & \textbf{10576} & 541912 & 45296 & \textbf{210384} & 55685200 & 922 & 922 & \textbf{1104232} & \textbf{117536} & 6777784  & \textbf{139200} & 25920 & 373656000  & 36417600 & \textbf{247096} & 15779808 & 14452800  & 14452800  \\ \hline
% 800  & \textbf{10576} & 734752 & 59248 & \textbf{210384} & 76161264 & 922 & 922 & \textbf{1472232} & \textbf{117536} & 9693296  & \textbf{185600} & 25920 & 683872000  & 64153600 & \textbf{247096} & 22649088 & 25670400 & 25670400 \\ \hline
% 1000 & \textbf{10576} & 909152 & 73200 & \textbf{210384} & 97702272 & 922 & 922 & \textbf{1840232} & \textbf{117536} & 14781544 & \textbf{232000} & 25920 & 1050040000 & 98592000 & \textbf{247096} & 32233728 & 40088000 & 40088000 \\ 
% \bottomrule[1.5pt]
% \end{tabular}
% }


% \end{table*}




==> tables/sa_time.tex <==
\renewcommand{\arraystretch}{1.2}
\begin{table*}[ht]
\centering
\caption{Computation Overhead Results of Secure Aggregation (ms): B - \sys, F - \flamingo, P - \pqsa, E - \eseafl, M$_1$ - \microfirst, M$_2$ - \microsecond.}
\label{table:sa_time}
 \resizebox{2\columnwidth}{!}{
\begin{tabular}{|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|}
% \toprule[1.5pt]
\hline
\multirow{3}{*}{\textbf{N}} & \multicolumn{11}{c|}{\textbf{Client}} & \multicolumn{6}{c|}{\textbf{Assisting Node}} & \multicolumn{11}{c|}{\textbf{Server}} \\ \cline{2-29}
& \multicolumn{5}{c|}{\textbf{Setup}} & \multicolumn{6}{c|}{\textbf{Aggregation}} & \multicolumn{3}{c|}{\textbf{Setup}} & \multicolumn{3}{c|}{\textbf{Aggregation}} & \multicolumn{5}{c|}{\textbf{Setup}} & \multicolumn{6}{c|}{\textbf{Aggregation}} \\ \cline{2-29}
& \textbf{B} & \textbf{F} & \textbf{E} & \textbf{M$_1$} & \textbf{M$_2$} & \textbf{B} & \textbf{F} & \textbf{P} & \textbf{E} & \textbf{M$_1$} & \textbf{M$_2$} & \textbf{B} & \textbf{F} & \textbf{E} & \textbf{B} & \textbf{F} & \textbf{E} & \textbf{B} & \textbf{F} & \textbf{E} & \textbf{M$_1$} & \textbf{M$_2$} & \textbf{B} & \textbf{F} & \textbf{P} & \textbf{E} & \textbf{M$_1$} & \textbf{M$_2$} \\ \hline
% & \textbf{\sys} & \textbf{\flamingo} & \textbf{\micro} & \textbf{\sys} & \textbf{\flamingo} & \textbf{\micro} & \textbf{\sys} & \textbf{\flamingo} & \textbf{\micro} & \textbf{\sys} & \textbf{\flamingo} & \textbf{\micro} & \textbf{\sys} & \textbf{\flamingo} & \textbf{\micro} & \textbf{\sys} & \textbf{\flamingo} & \textbf{\micro} \\ \hline


200  & \textbf{313} & 88 & 1 & 39 & 1 & \textbf{1} & 193 & 3390 & 1 & 131763 & 131821 & \textbf{13153} & 296 & 10 & \textbf{7} & 289 & 7 & \textbf{135} & 25 & 1 & 6  & 4  & \textbf{76}    & 10586  & 489 & 26 & 30730289  & 31511168  \\ \hline
400  & \textbf{312} & 88 & 1 & 183  & 2 & \textbf{1} & 215 & 6802 & 1 & 131787 & 131876 & \textbf{26186} & 591 & 20 & \textbf{14} & 591 & 11 & \textbf{135} & 24 & 1 & 28  & 9  & \textbf{151}  & 26134 & 1795 & 37 & 62393938  & 61894338  \\ \hline
600  & \textbf{315} & 87 & 1 & 441  & 3 & \textbf{1} & 221 & 10387 & 1 & 131787 & 13200 & \textbf{38865} & 909 & 26 & \textbf{21} & 810 & 15 & \textbf{143} & 26 & 1 & 65  & 16 & \textbf{225}  & 36099 & 3941 & 47 & 95284372  & 95113588  \\ \hline
800  & \textbf{314} & 87 & 1 & 823  & 4 & \textbf{1} & 220 & 14139 & 1 & 131797 & 131876 & \textbf{52143} & 1167 & 35 & \textbf{28} & 1122 & 20 & \textbf{146} & 24 & 1 & 122 & 25 & \textbf{323}  & 55836 & 6964 & 58 & 133114693 & 125088773 \\ \hline
1000 & \textbf{313} & 87 & 1 & 1326 & 5 & \textbf{2} & 236 & 18319 & 1 & 131842 & 131882 & \textbf{65347} & 1465 & 42 & \textbf{35} & 1708 & 24 & \textbf{215} & 24 & 1 & 189 & 38 & \textbf{417} & 87207 & 10818 & 69 & 175829383 & 158195623 \\ 
% \bottomrule[1.5pt]
\hline
\end{tabular}
}


% \begin{tabular}{c|c|c|c|c|c|c}
% \toprule[1.5pt]
% \multirow{2}{*}{\textbf{N}} & \multicolumn{2}{c|}{\textbf{User}} & \multicolumn{2}{c|}{\textbf{Assisting Node / Decryptor}} & \multicolumn{2}{c}{\textbf{Server}} \\ \cline{2-7}
% & \textbf{PQFL} & \textbf{Flamingo} & \textbf{PQFL} & \textbf{Flamingo} & \textbf{PQFL} & \textbf{Flamingo} \\ \midrule
% 200 & \textbf{18.46} & 154.98 & \textbf{20.74} & 164.87 & \textbf{123.29} & 4513.78 \\ \hline
% 400 & \textbf{18.55} & 162.62 & \textbf{28.10} & 280.73 & \textbf{245.65} & 10660.50 \\ \hline
% 600 & \textbf{20.89} & 162.46 & \textbf{34.11} & 363.73 & \textbf{366.45} & 15765.36 \\ \hline
% 800 & \textbf{18.88} & 171.72 & \textbf{42.00} & 531.70 & \textbf{487.66} & 23966.09 \\ \hline
% 1000 & \textbf{18.94}  & 181.66 & \textbf{51.08} & 721.59 & \textbf{619.86} & 33090.42 \\
% \bottomrule[1.5pt]
% \end{tabular}
\end{table*}



